FLACK: Counterexample-Guided Fault Localization for Alloy Models

Fault localization is a practical research topic that helps developers identify code locations that might cause bugs in a program. Most existing fault localization techniques are designed for imperative programs (e.g., C and Java) and rely on analyzing correct and incorrect executions of the program to identify suspicious statements. In this work, we introduce a fault localization approach for models written in a declarative language, where the models are not "executed," but rather converted into a logical formula and solved using backend constraint solvers. We present FLACK, a tool that takes as input an Alloy model consisting of some violated assertion and returns a ranked list of suspicious expressions contributing to the assertion violation. The key idea is to analyze the differences between counterexamples, i.e., instances of the model that do not satisfy the assertion, and instances that do satisfy the assertion to find suspicious expressions in the input model. The experimental results show that FLACK is efficient (can handle complex, real-world Alloy models with thousand lines of code within 5 seconds), accurate (can consistently rank buggy expressions in the top 1.9\% of the suspicious list), and useful (can often narrow down the error to the exact location within the suspicious expressions).

==> background.tex <==
\section{Background}

==> discuss.tex <==
\section{Discussion}
For \textit{arr1.als}, no counter example or passing instance generated due to the following sentence is a false statement and no valid instance: $ all i:Int |i>=0 and i<Array.length $.

For overconstraint specification where there no counterexample generated for assert, we change the fact to pred1, then we insert a correct pred called pred2,  then we add an assert to check if pred1 equals to pred2 by saying that $pred1<=>pred2$.

We use assertion and predicate to fully automate the procedure for fault localization, this part can be modified to involve user in the loop. For example, the user may write a predicate and run Alloy to generate some instance. Then he spot some relationship or signature that should be removed(or added), he could select such relationship and our tool will point him to the possible bug locations.

==> pldi21/algorithm.tex <==
\section{Approach}
\label{sec:approach}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwData{pairs}{pairs}
\SetKwData{maxpairs}{max\_instance\_pairs}
\SetKwData{cex}{c}
\SetKwData{sin}{s}
\SetKwData{diffs}{diffs}
\SetKwData{diff}{diff}
\SetKwData{nil}{nil}
\SetKwData{diff}{diff}
\SetKwData{expr}{expr}
\SetKwData{sexpr}{sexpr}
\SetKwData{exprs}{exprs}
\SetKwData{sexprs}{sexprs}
\SetKwData{conflicts}{conflicts}
\SetKwData{false}{false}
\SetKwData{rel}{rel}
\SetKwData{relates}{relates}
\SetKwData{infers}{infers}
\SetKwData{name}{name}
\SetKwData{tuples}{tuples}
\SetKwData{tuple}{tuple}
\SetKwData{atom}{atom}
\SetKwData{crel}{crel}
\SetKwData{srel}{srel}
\SetKwData{rank}{rank}
\SetKwData{sus}{suspicious}
\SetKwData{suspexprs}{susp\_exprs}
\SetKwData{keywords}{keywords}
\SetKwData{subs}{subs}
\SetKwData{sub}{sub}
\SetKwData{esubs}{epxr\_subs}
\SetKwData{node}{node}
\SetKwData{score}{score}
\SetKwData{relscore}{relscore}
\SetKwData{results}{results}
\SetKwData{instexpr}{isexpr}
\SetKwData{vals}{vals}
\SetKwData{cvals}{cvals}
\SetKwData{svals}{svals}
\SetKwData{instscore}{instscore}
\SetKwData{pexpr}{pexpr}
\SetKwData{child}{child}

\SetKwFunction{getchildren}{getchildren}
\SetKwFunction{AlloyAnalyzer}{AlloyAnalyzer}
\SetKwFunction{Pardinus}{Pardinus}  
\SetKwFunction{PMaxSolver}{PMaxSolver}
\SetKwFunction{AlloySolver}{AlloySolver}
\SetKwFunction{block}{blockcex}
\SetKwFunction{comparator}{comparator}
\SetKwFunction{gen}{gencex}
\SetKwFunction{unsat}{get\_unsatcore}
\SetKwFunction{unsatanalyzer}{unsat\_analyzer}
\SetKwFunction{diffsanalyzer}{diffs\_analyzer}
\SetKwFunction{getdiffs}{get\_diffs}
\SetKwFunction{getdiff}{get\_diff}
\SetKwFunction{slice}{slice}
\SetKwFunction{eval}{eval}
\SetKwFunction{collect}{collect\_exprs}
\SetKwFunction{infer}{infer}
\SetKwFunction{extract}{extract\_keywords}
\SetKwFunction{sort}{sort}
\SetKwFunction{inst}{instantiate}
\SetKwFunction{isbool}{isbool}
\SetKwFunction{getrelsubs}{get\_rel\_subs}
\SetKwFunction{getsuspexprs}{get\_susp\_exprs}
\SetKwFunction{collectsexprs}{collect\_exprs}
\SetKwFunction{compute}{computescore}
\SetKwFunction{isleaf}{isleaf}

\SetKwProg{Func}{Function}{:}{}

%The fault localization technique used by {\tool} heavily relies on the built-in Alloy Analyzer. More specifically, we use the Alloy Analyzer to check for assertion violations and obtain counterexamples and unsat cores to identify expressions in the input model causing these violations. Below we briefly introduce the Alloy Analyzer and present the {\tool} algorithm.


Figure~\ref{fig:workflow} gives an overview of {\tool}, which takes as input an Alloy model with some violated assertion and returns a ranked list of suspicious expressions contributing to the assertion violation.
The insight guiding our research is that the differences between counterexamples that do not satisfy the assertion and closely related satisfying instances can drive localization of suspicious expressions in the input model.
To achieve this, {\tool} uses the \emph{Alloy analyzer} to find counterexamples showing the violation of the assertion.
It then uses a PMAX-SAT solver to find satisfying instances that are \emph{as close as possible} to the cex's.
Next, {\tool} analyzes the differences between the cex's and satisfying instances to find expressions in the model that likely cause the errors.
Finally, {\tool} computes and returns a ranked list of suspicious expressions.


\begin{figure}[t!]
    \centering
    %\includegraphics[width=0.6\linewidth]{arch}
    \includegraphics[width=\linewidth]{arch.png}
    \caption{Overview of {\tool}.}
    \label{fig:workflow}
\end{figure}

%The rest of this section first overviews the formal underpinnings of our approach based on Alloy's relational logic and its associated analyzer, then presents our contributions to support fault localization for models written in Alloy's declarative language.

\begin{comment}
%Comment: The following paragraphs are confusing.
%We already provide an overview of the approach in II.A, which can potentially move here.

Following the human intuition looking for errors, the first heuristic is to find the expressions contains the relation in the difference. For example, in the motivating example, the relation \texttt{transition} and \texttt{FSM.start} are two most relevant relations.

After finding the most relevant expressions, we then try to assign a score to each expression based on their impact on the difference. This is based on the number of different values contained in the evaluation of each expression. For example, in the motivating example, for expression \texttt{FSM.start !in s.transition}, FSM.start evaluates to \texttt{State1} and s.transitioon evaluates to \texttt{State1, State0, State2}. It constraints out State1 from the set of values {State1, State0}. And none of these values affects the difference between cex and sat. By analyzing the ratio of how many different values are included in the expression, we can get an estimate of how close the expression related to the difference.  
\end{comment}


%We may want to use "Formal Underpinnings" as the title of this subsection
\subsection{The Alloy Analyzer}
%\subsection{Formal Underpinnings}

An Alloy specification or \emph{model} consists of three components: (i) Type signatures (\texttt{sig}) define essential \emph{data types} and their \emph{fields} capture relationships among such data types, (ii) \texttt{fact}s, predicates (\texttt{pred}), and assertions (\texttt{assert}) are formulae defining constraints over data types, and (iii) \texttt{run} and \texttt{check} are commands to invoke the Alloy Analyzer. The \texttt{check} command is used to find counterexamples  violating some asserted property, and \texttt{run} finds %instances satisfying some property defined by a predicate (\emph{sat instances})).
satisfying model instances (\emph{sat instances}).
For a model $M$ and a property $p$, a cex is an instance of $M$ that satisfies $M \wedge \neg p$, and a sat instance is one that satisfies $M \wedge p$.
The specification in Figure~\ref{fig:ex} defines two signatures (\texttt{FSM, State}), three fields (\texttt{start, stop, transition}), three facts (\texttt{OneStartStop, ValidStart, ValidStop}) and one assertion (\texttt{NoStopTransition}).

%In Alloy, an instance of $M$ is a set of relations for the sigs and fields defined in $M$. Moreover, each relation is a set of tuples and each tuple is a set of atoms. Table~\ref{fig:textrepr} shows the Alloy representation of the cex in Fig~\ref{fig:cex1}. For example, the second row lists the relation for the field \texttt{start}, and it contains one tuple \texttt{FSM00 -> State0} with two atoms \texttt{FSM0, State0} (graphically, this tuple is represented by the edge from \texttt{FSM} to \texttt{State0} in Figure~\ref{fig:cex1}).




%Given an model $M$ consisting of constraints $\{c_1, c_2, \dots, c_n\}$, a property $p$ is valid in $M$ if every instance of $M$ satisfies $p$, i.e., $\forall x. (\bigwedge c_i \implies x) \implies SAT(x,P)$, and $p$ is invalid if there exists a counterexample, which is  an instance of $M$ that does not satisfy $P$, i.e., $\exists x. (\bigwedge c_i \implies x) \wedge \neg SAT(x,P)$.

Analysis of specifications written in Alloy is entirely automated, yet bounded up to user-specified scopes on the size of type signatures.
More precisely, to check that  $p$ is satisfied by \emph{all} instances of $M$ (i.e., $p$ is valid) up to a certain scope, the Alloy developer encodes $p$ as an \emph{assertion} and uses the \texttt{check} command to validate the assertion, i.e., showing that no cex exists within the specified scope (a cex is an instance $I$ such that $I \vDash M \land \neg p$).
To check that $p$ is satisfied by \emph{some} instances of $M$, the Alloy developer encodes $p$ as a predicate and uses the \texttt{run} command to analyze the predicate, i.e., searching for a sat instance $I$ such that $I \vDash M \land p$.
In our running example, the \texttt{check} command examines the \texttt{NoStopTransition} property and returns a cex in Figure~\ref{fig:cex1}.


Internally, Alloy converts these tasks of searching for instances into boolean formulae and uses a SAT solver to check the satisfiability of the formulae. Each value of each relation is translated to a distinct variable in the boolean formula. For example, given a scope of 5 in the FSM model in Figure~\ref{fig:ex}, the relation \texttt{State} contains 5 values and is translated to 5 distinct variables in the boolean formula, and the \texttt{transition} is translated to 25 values representing 25 values of combinations of $\|State\| \times \|State\|$. An instance is an assignment for all variables that makes the formula True. For example, \emph{cex} in Figure~\ref{fig:cex1} is an assignment where all variables corresponding to values in Table~\ref{table:model1} are assigned True and others are False.
%Alloy is a bounded analyzer
%For efficiency, Alloy allows the user to run the SAT solver up to certain bounds, e.g., checking that $p$ holds up to certain bounds.
Finally, Alloy translates the result from the SAT solver, e.g., an assignment that makes the boolean formula True, back to an instance of $M$.




%Alloy then converts this formula's solution to an instance. Due to the randomness of SAT solver, the instances is also generated randonly. Alloy only ensures current relation is not the same as the next instance, and these two may differentiate from each.


% \begin{comment}
%   \begin{figure}[t]
    
%   \begin{subfigure}{0.24\linewidth}
%     \centering
%     \includegraphics[width=0.7\linewidth]{res/algo/ncne.png}
%     \caption{}
%     \label{fig:nocexnoexp}
%   \end{subfigure}
%   \begin{subfigure}{0.24\linewidth}
%     \centering
%     \includegraphics[width=0.7\linewidth]{res/algo/nce.png}
%     \caption{}
%     \label{fig:nocexexp}
%   \end{subfigure}
%   \begin{subfigure}{0.24\linewidth}
%     \centering
%     \includegraphics[width=0.7\linewidth]{res/algo/cne.png}
%     \caption{}
%     \label{fig:cexnoexp}
%   \end{subfigure}
%   \caption{Four cases when checking a property: (a) No Cex, No Sat; (b) Sat, No Cex; (c) Cex, No Sat; (d) Cex, Sat} 
%   \label{fig:4cases}
% \end{figure}


% \textcolor{cyan}{HB: The following subsection should move to the BFA algorithm as it is the observation underlying the approach. We also need to add a brief introduction explaining the in our approach for each assertion we systematically synthesize its predicate counterpart.}
% \paragraph{Possible Results in Alloy}
% The process of checking a property $p$ in a model $M$ typically results in the four cases shown in Figure~\ref{fig:4cases}.
% The circle represents the state space consisting of all instances of $M$.% {\tool} is only applicable to cases when we can obtain cex's representing  instances of $M$ that do not satisfy $p$.

% Figure~\ref{fig:nocexnoexp} shows the case, where we cannot obtain any instances of $M$ that do or do not satisfy $p$ (i.e., no cex's or sat instances).
% This could occur when $M$ contains conflicting constraints, e.g., they evaluate to \texttt{false} and thus there are no instances at all.
% {\tool} cannot be applied to this case as the Alloy Analyzer cannot generate any cex indicating the violation of $p$.
% Figure~\ref{fig:nocexexp} shows the case, where every instance of $M$ satisfies $p$ (i.e., no cex's).
% {\tool} is not applicable in this case as there is no assertion violation.

% Figure~\ref{fig:cexnoexp} shows the case, where we can only obtain cex's, but no sat instances, i.e., every instance of $M$ violates $p$.
% In this case {\tool} analyzes the unsat core to localize expressions in $M$ that do not satisfy $p$ (Section~\ref{sec:unsat}).
% Finally, Figure~\ref{fig:cexexp} shows the case where we can obtain both cex's and sat instances.
% This is the typical assertion violation situation that {\tool} is designed to effectively handle (Section~\ref{sec:alg}).

%% Given an Alloy model with fixed sigs and fields declaration and a scope, the full state space is represented as rectangle in the figure, the state space of expected model(or perfect model) is represented by the blue circle annotated with E, implemented model(concrete model) by the yellow circle with I and property expressed by assertion by red circle with A. The intersection of I and E are expected instances and the intersection of I and A are cexs. Each situation is explained below:

%% \begin{itemize}
%%   \item Fig ~\ref{fig:nocexnoexp}, No cex and no expected instance: The implemented model doesn't intersect with expceted model or assertion, thus no couterexample generated when checking the assert, and no expecting instance could be found. The implemented model is too overconstraint to generate anything. \tool couldn't work on this situation as there is no instance to compare.
%%   \item Fig ~\ref{fig:cexnoexp}, Cex and no expected instance: The implemented model intersect with assertion but not with the expected model, thus there are some couterexamples but no expected instance generated. The implemented model is overconstrainted to generate any expected instance and \tool uses UNSAT core analyzer to solve this kind of bug.
%%   \item Fig ~\ref{fig:cexexp}, Cex and expected instance: The implemented model intersect with both assertion and expected model, thus there are cexs and expected instances genereated. \tool uses comparator and locator to locate this kind of bugs.
%%   \item Fig ~\ref{fig:nocexexp}, No cex and expected instance: The implemented model itersect with the expected model and disjunct with the assertion. \tool assumes there is no error in this kind of situation. To check the correctness, either some manual inspection needed or write an other assertion to capture any over or under constraint problem of the implemented model with respect to the expected model.
%% \end{itemize}




\subsection{The {\tool} Algorithm}
\label{sec:alg}

\begin{algorithm}[t!]
%\hline
%\hline
  \small
  \DontPrintSemicolon
  
  \SetAlgoLined
  \Input{Alloy model $M$, property $p$ not satisfied by $M$}
  \Output{Ranked list of suspicious expressions in $M$}
%  \BlankLine
%\hline
  $\AlloySolver \leftarrow \AlloyAnalyzer(M, p)$\;
  $\pairs \leftarrow \emptyset$\;
  \While{$|\pairs| <  \maxpairs$}{
    $\cex \leftarrow \AlloySolver.\gen()$\;
    $\AlloySolver.\block(\cex)$\;
    $\sin \leftarrow \PMaxSolver(M, \cex)$\;
    \uIf{$\sin = \nil$}{
       $U \leftarrow \AlloySolver.\unsat()$\;
       \Return $\unsatanalyzer(M, U, \cex)$\;
     } 
      
    $\pairs \leftarrow \pairs \cup (\cex, \sin)$\;
  }
  $\diffs \leftarrow \comparator(\pairs)$\;
  \Return $\diffsanalyzer(\diffs)$\;
%\hline
%\hline
  \caption{{\tool} fault localization process}
  \label{algo:overview}
\end{algorithm}

Figure~\ref{algo:overview} shows the algorithm of {\tool}, which takes as input an Alloy model $M$ and a property $p$ that is not satisfied by $M$ (as an assertion violation) and returns a ranked list of expressions that likely contribute to the assertion violation.
{\tool} first uses the Alloy Analyzer and the Pardinus PMAX-SAT solver to generate pairs of cex and closely similar sat instances. %(the current implementation uses 5 pairs).
{\tool} then analyzes the differences between the cex and sat instances to locate the error.
If {\tool} cannot generate any sat instance, {\tool} inspects the \emph{unsat core} returned by the Alloy Analyzer to locate the error.



\subsubsection{Generating Instances}
\label{sec:geninsts}
To understand why $M$ does not satisfy $p$, {\tool} obtains differences between cexs and relevant  sat instances.
These differences can lead to the cause of the error.
One option is to use the Alloy Analyzer to generate a sat instance directly (e.g., by checking a \emph{predicate} consisting of $p$).
However, such an instance generated by Alloy is often predominantly different from the cex, and thus does not help identify the main difference.
For example, the cex, shown in Figure~\ref{fig:cex1}, that violates the assertion \texttt{NoStopTransition} is quite different from the two Alloy-generated satisfying instances, shown in Figure~\ref{fig:sat_inst_alloy}.


%After generating a cex\footnote{If there is no cex, we are done as Alloy cannot find any instance that violate the assertion as explained in Section~\ref{sec:4cases}.}, we attempt to find a sat instance and compare them. We could ask the Alloy Analyzer to directly generate a sat instance (e.g., by checking a \emph{predicate} consisting of $p$). However, such an instance generated by Alloy is often different from the cex and thus does not help identify the main difference. For example, the cex in Figure~\ref{fig:cex1} that violates the assertion \texttt{NoStopTransition} in Figure~\ref{fig:ex} is quite different from the two Alloy-generated satisfying instances, shown in Figure~\ref{fig:sat_inst_alloy}. Even if we keep asking Alloy to generating new sat instances, we would not likely get one that is similar to the cex.


%% To locate a bug for a cex, a general approach is to manually identify which relations are missing or need to be deleted. When the cex is simple, contains 5 or 10 relations, manually doing this is reasonable. But when the number of relations grows, it becomes much more difficult to identify such relations. The instance generator will automatically identify these relations.

%However, because of the randomness nature of Alloy search, the generated expected instance would be very different from the cex, including many unnecessary information. To address this problem, we would like to get an expected instance as same as the cex such that the difference between these two only contains necessary information. 

To generate a sat instance closely similar to the cex, we reduce the problem to a PMAX-SAT (partial maximum satisfiability) problem.

\begin{definition}[Finding a Similar Sat Instance from a Cex]
Given a set of \emph{hard} clauses, collectively specified by model $M$ and property $p$, and a set of \emph{soft} clauses, specified by a counterexample $cex$, find a solution that satisfies \emph{all} hard clauses and satisfies \emph{as many soft clauses as possible}. 
\end{definition}


\begin{figure}[h]
  \centering
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=1\linewidth]{res/images/random1.png}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=1\linewidth]{res/images/random2.png}
  \end{subfigure}
  \caption{Model instances generated by the Alloy Analyzer.}
  \label{fig:sat_inst_alloy}
\end{figure}


More specifically, %{\tool} converts the input model $M$ and the property $p$ into a set of hard clauses and the cex into a set of soft clauses. For instance, to generate the sat instance similar as the \emph{cex}, 
the hard clauses are generated by constraints in the Alloy model, %and the predicate converted from the assertion, 
and the soft clauses are the assignment represented by \emph{cex} where all presenting variables are True and other variables are False. Because the relations and scope of the Alloy model stay the same, the variables in the transformed boolean formula would also remain the same, and just the values assigned to them would differ between various model instances. Thus, this encoding can apply to general instances regardless of their structures.

{\tool} then uses an existing PMAX-SAT solver (Pardinus) to find an instance that has the property $p$ and is as similar to the cex as possible\footnote{Based on our experiment, the first solution returned by the PMAX-SAT solver is similar enough for {\tool} to locate bugs.}.
For example, the instance in Figure~\ref{fig:expected1} generated by Pardinus is similar to the cex in Figure~\ref{fig:cex1}, but has an extra edge from  \texttt{State3} to \texttt{State1}.
%Figure~\ref{fig:expected1} shows a PMAX-SAT instance that Pardinus generates from the cex in Figure~\ref{fig:cex1}.
The idea is that such (minimal) differences can help {\tool} identify the error.

%In case that the MAXSAT solver returns multiple similar instances, we run the MAXSAT solver 5 times and pick the instance with the minimum differences, with the purpose of reducing irrelevant differences. 

%% {\tool} then analyzes and maps the differences between the cex and the resulting instance to relations in the input model $M$.
%% Intuitively, these relations capture the minimal differences between instances that do and do not satisfy $p$.

%% {{\tool}} encodes $M \land P$ as hard clauses and cex C as soft clauses, to generate an instance that has property P while is as similar as C to ensure the difference between these two contains only necessary relations that differentiate having property P and not having property P.

%In addition, another advantage of using PMAX-SAT is that the generated pair have a unified names, which avoids mapping names by the comparator when comparing for differences.


%% There are two possible situations when generating instance pairs: (1) generate couterexample and couldn't generate expected instance; (2) generate couterexample and expected instance. For the first situation, this means an over-constraint bug that prevents any instance to have property stated in the expected instance, and {{\tool}} uses the UNSAT core analyzer discussed in ~\ref{sec:unsat} to locate the bug. For the second situation, {{\tool}} use Comparator in section ~\ref{sec:comparator} and Locator to locate the bug.

%Comparator is then able to find out which relation should be deleted or added by comparing the cex and the expected instance.

\subsubsection{Comparator}
\label{sec:comparator}

{\tool} compares the generated cex's and sat instances to obtain their differences, which involve atoms, tuples, and relations.
First, it obtains tuples and their atoms that are different between the cex and sat instance, e.g., in Figure~\ref{fig:pair1}, the tuple \texttt{State3->State1}, which has the atoms \texttt{State1} and \texttt{State3}, is in the cex but not in the satisfying instance. Next, it obtains relations with different tuples between the cex and sat instance, e.g., the \texttt{transition} relation involves the tuple \texttt{State3->State1} in the cex but not in the sat instance. Third, it obtains relations that can be inferred from the tuples and atoms derived in the previous steps, e.g., the relation \texttt{FSM.stop} involves tuples having the \texttt{State3} atom. %and the relation \texttt{transition}, which is already identified, that involves both atoms \texttt{State1} and \texttt{State3}.
%\tvn{Make sure I cover all the main ideas correctly}

In summary, for the pair of cex and sat instance in Figure~\ref{fig:pair1}, {\tool} obtains the suspicious relations \texttt{transitions} and \texttt{stop} and the atoms \texttt{State1, State3}. {\tool} applies these comparison steps for all pairs of instances and cex's and uses the common results.





%Within a relation, different tuples are those that are different between cex and sat instance, e.g., the tuple \texttt{State3->State1} in the \texttt{transition} relation is in cex but not in the sat instance.
%Related relations are those directly affecting the cex and sat instance, e.g. the ones that have different tuples between cex and sat instance, e.g., the relation \texttt{transition} in Figure~\ref{fig:pair1} has the tuple \texttt{State3->State1} in cex but not in the sat instance.
%Inferred relations are those inferred from the difference that possible affects cex and sat instance, e.g., the \texttt{FSM.stop} relation in Figure~\ref{fig:pair1} is inferred from \texttt{State3}.

%Algorithm~\ref{algo:compare} shows the algorithm for comparator, which takes as input a set of pairs of cex and sat instance generated from Section~\ref{subsec:geninst}, and a summary of difference between all pairs. 
%We first compare the tuples for each relation between each pair of cex and sat instance.
%If we find any different tuples for a relation, we save the tuples to different values and the relation to related relation.
%We then try to infer other possible relations that may affect the difference using the \emph{infer}. For each atom in the difference, \emph{infer} finds relations which contains exactly one tuple and the tuple's last atom equals this atom.
%For example, in Table~\ref{fig:textrepr}, \texttt{State3} appears as last atom of \texttt{stop} which only contains one tupe \texttt{FSM0->State3}.

% \begin{algorithm}[t]
%   \small
%   \DontPrintSemicolon

%   \SetAlgoLined
%   \Input{\pairs: pairs of counterexamples and sat instances}
%   \Output{\diff: summary of difference}

%   \ForEach{$(\cex,\sin) \in \pairs$}{
%     \ForEach{$\crel(\name,\tuples) \in \cex$}{
%       $\srel \leftarrow \sin.get(\crel.\name)$\;
%       \uIf{$\crel.\tuples \neq \srel.\tuples$}{
%         $\diffs.\diff \leftarrow \getdiff(\crel.\tuples,\srel.\tuples)$\;
%         $\diffs.\relates \leftarrow \relates \cup \crel.\name$\;
%         $\diffs.\infers \leftarrow \infers \cap \infer(\diff)$\;
%       }
%     }
%   }
%   \Return $\diffs$ \;
%   \Func{$\infer(\diff)$}{
%     \ForEach{$\tuple \in \diff$}{
%       \ForEach{$\crel(\name,\tuples) \in \cex \cup \sin$}{
%         \uIf{$|\tuples| = 1 \land \atom = \tuples[0].last\_atom$}{
%           $\infers \leftarrow \infers \cup \crel.\name$\;
%         }
%       }
%     }
%   }
%   \Return \infers\;
 
%  \caption{Comparator\tvn{Candidate to cut if out of space. The text already gave a good description of this}}
%  \label{algo:compare}
% \end{algorithm}

\subsubsection{Diff Analyzer}
After obtaining the differences consisting of relations and atoms between cex's and sat instances, {\tool} analyzes them to obtain a ranked list of expressions based on their suspicious levels.
{\tool} assigns higher suspicious scores to expressions whose evaluations depend on these differences (and lower scores to those not depending on these differences).


Algorithm~\ref{algo:diff} shows the Diff Analyzer algorithm, which takes as input a model $M$, the differences $\diffs$ obtained in Sect~\ref{sec:comparator}, and pairs of cex and sat instances obtained in Sect~\ref{sec:geninsts}, and outputs a ranked list of suspicious expressions in $M$.
It first identifies expressions in $M$ that involve relations in $\diffs$.
These expressions are likely related to the difference between cex and sat instance.
For example, consider the model in Figure~\ref{fig:ex}. {\tool} identifies two expressions: \\ \texttt{all s: State | FSM.stop in s.*transition} on line~\ref{line:sexp1} and \texttt{all s: State | s.transition = none => s in FSM.stop} on line~\ref{line:bug}, as they involve the relations \texttt{transition} and \texttt{stop} in $\diffs$.


\begin{algorithm}[t]
    \small
    \DontPrintSemicolon
%\hline
%\hline
    \SetAlgoLined
    \Input{Alloy model $M$, differences $\diffs$, pairs of cex's and sat instances $\pairs$ }
    \Output{Ranked list of suspicious expressions in $M$}
%    \BlankLine
%\hline
    $\exprs \leftarrow \getsuspexprs(M, \diffs)$\;
    $\results \leftarrow \{\}$\;
    \ForEach{$\expr \in \exprs$}{
      $\compute{\expr, \results}$\;
    }
    \Return $\sort{\results}$\;

    \BlankLine

    \Func{\compute{$\expr, \results$}}{
      $\score = 0$\;
      \uIf{\isleaf($\expr$)}{
        $\instexpr \leftarrow \inst(\expr,\diff)$\;
        \ForEach{$(\cex,\sin) \in \pairs$}{
          $\cvals \leftarrow \eval(\cex,\instexpr)$\;
          $\svals \leftarrow \eval(\sin,\instexpr)$\;
          $\instscore \leftarrow 0$\;
          \uIf{$\diff \subset \cvals$}{
            $\instscore \leftarrow \instscore + \frac{|\diff|}{|\cvals|}$\;
          }
          \uIf{$\diff \subset \svals$}{
            $\instscore \leftarrow \instscore + \frac{|\diff|}{|\svals|}$\;
          }
          $\score \leftarrow \score + \frac{\instscore}{2}$)\;
        }
        $\score \leftarrow \frac{\score}{|\pairs|}$\;
      }
      \Else{
        \uIf{$\isbool(\expr)$}{
          $\instexpr \leftarrow \inst(\expr,\diff)$\;
          \ForEach{$(\cex,\sin) \in \pairs$}{
            \uIf{$\eval(\cex,\instexpr) \neq \eval(\sin,\instexpr)$}{
              $\score \leftarrow \score + 1$\;
            }
          }
        }
        \ForEach{$\child \in \getchildren(\expr)$}{
          $\score \leftarrow \score + \compute(\child, \results)$\;
        }
      }
      $\results \leftarrow \results \cup (\expr, \score)$\;
      \Return $\score$\;
    }
%\hline
%\hline
  \caption{Diff Analyzer}
  \label{algo:diff}
\end{algorithm}

{\tool} then recursively computes the suspicious score for each collected expression $e$, represented as an AST tree.
If $e$ is a leaf (e.g., a relational expression), {\tool} instantiates $e$ with atoms from $\diffs$.
{\tool} then evaluates the instantiated expression for each pair of cex and sat instance.
If the evaluated result for an instantiated expression contains \textit{all} atoms involved in $\diffs$, {\tool} computes the score as ``\textit{size of $\diffs$ / size of evaluated results};'' otherwise, the score is 0. For a pair, the score is then the average score of cex and sat instance. At last, the score of $e$ is the average among all pairs.
Essentially, a higher suspicious score is assigned to a relational subexpression whose evaluation involves many atoms in $\diffs$.

If $e$ is not a leaf node, $e$'s score is the sum of boolean and relational scores. %two parts. %: the boolean and relational scores. %The boolean score is 0 if $e$ is not a boolean expression. 
If $e$ is a boolean expression (i.e., an expression that returns \texttt{true} or \texttt{false}), we instantiate $e$ with atoms from $\diffs$ and evaluate it on each cex and sat instance pair.
If it evaluates to different results between the cex and sat instance (e.g., one is \texttt{true} and the other is \texttt{false}), %{\tool} assigns the value 1 to $e$. 
{\tool} increases $e$'s score by 1.
Thus, a higher boolean score is assigned to the expressions whose evaluation does not match between pairs of the cex and sat instances.
%Note that $e$'s score is its average score across all pairs.
%Thus, a higher score is assigned to a boolean subpexression whose evaluation does not match between the cex and sat instance.
Then $e$'s relational score is calculated as the sum of $e$'s children. 
The final score assigned to each expression is the sum of the $e$'s boolean scores and the relational scores of $e$'s children.
In the end, {\tool} returns all expression ranked by their suspicious scores.
%\textcolor{red}{ \\\textbf{HB: These two sentences seem to be conflicting: "$e$'s score is its average score across all pairs." and "The final score assigned to each expression is the sum of the $e$'s scores and the scores of $e$'s children."}}

%Then for each suspicious expression, {\tool} collects a list of related expressions or nodes: the expression itself and all subexpressions of that expression.
%The subexpressions can be , or relational expressions (atomic formulae and return values).
%For example, for the expression \texttt{all s: State | s.transition = none => s in FSM.stop} on line ~\ref{line:bug} in Figure~\ref{fig:ex}, {\tool} collects 3 boolean expressions: \texttt{s.transition = none => s in FSM.stop}, \texttt{s.transition = none}, and \texttt{s in FSM.stop}, and 3 relational expressions: \texttt{s.transition}, \texttt{s} and, \texttt{FSM.stop}.

%% For example, for the cex and sat instance in Figure~\ref{fig:pair1}, the related relation is \texttt{transition} and the inferred relatiosn is \texttt{stop}. Two expressions are extracted as they mentions : 

%$\tool$ computes a score for each collected (sub)expression $e$ from each pair of cex and sat instance and then takes the average of these scores to be the final suspicious score for $e$.
 %{\tool} calculates the score of $e$ using a pair of cex and sat instance as follows: {\tool} first instantiates the expression with the different values between this pair of cex and sat instance. Then for each of the instantiated expression, {\tool} calculates its score as follows: If the expression is a boolean expression, its score and its parent's score are increased by 1 if any of its instantiated expression evaluates to different results, e.g. true or false, between cex and sat instance. Last, the expression gets a final score as the average score among all pairs.
%For each collected expression $e$, {\tool} compute a suspicious score as follows. The suspiciou score is sum of two scores: the score for boolean and the score for relation. 

%{\tool} first calculates the boolean score. If $e$ is a relational expression, then this score is 0. Otherwise, if $e$ is a boolean expression, {\tool} instantiate it with the atoms in $diffs$ and evaluates it with cex and sat instance. If the evaluated result is different between cex and sat instance, one false and the other true, then the socre for $e$ and $e$'s parent is increased by 1. 

%Then {\tool} calculates the relational score. To calculate relational score, {\tool} collects all sub relational expression for $e$. Then each sub relational expression is instantiated with atoms in $diffs$. {\tool} then evaluates each instantiated expression with both cex and sat instance. If the result doesn't contains all atoms in $diffs$, then the score is 0. If the result contains all atoms from $diffs$, a score is calculated as size of $diffs$ / size of $result$. The final relational score is then the average for all sub relations expression scores.

%% Subexpressions include the expression itself, all its sub boolean expressions and all its sub relational expressions. The sub boolean expressions are expressions that are connected by boolean Alloy operators and return true/false, for example, boolean operators like \texttt{=, in, =>} or unary boolean operators like \texttt{not, lone, some}. The sub relational expressions are expressions at 'atomic-level' which return a set of values and locates as a direct sub expression of a boolean operators. For example, for \texttt{all s: State | s.transition = none => s in FSM.stop} in Figure~\ref{fig:ex}, {\tool} collects 3 boolean expressions: \texttt{s.transtion = none => s in FSM.stop}, \texttt{s.transition = none} and \texttt{s in FSM.stop}, and 3 relational expressions: \texttt{s.transition}, \texttt{s} and \texttt{FSM.stop}.

%For each collected expression, {\tool} then calulate its scores as the average score among all pairs. {\tool} calculates the score of an expression in one pair as follows: {\tool} first instantiates the expression with the different values between this pair of cex and sat instance. Then for each of the instantiated expression, {\tool} calculates its score as follows: If the expression is a boolean expression, its score and its parent's score are increased by 1 if any of its instantiated expression evaluates to different results, e.g. true or false, between cex and sat instance. Last, the expression gets a final score as the average score among all pairs.

%For example, in Figure~\ref{fig:ex}, expression (b) 
To make the idea concrete, consider the expression
\texttt{s.transition = none} in Figure~\ref{fig:ex}. For the cex and sat instance pair in Figure~\ref{fig:pair1}, $\diffs$ contain two atoms \texttt{State1} and \texttt{State3}.
{\tool} first instantiates the expression under analysis with the atoms mentioned above into two concrete expressions: (1) \texttt{State1.transition = none} and (2) \texttt{State3.transition = none}. The concrete expression (1) evaluates to \texttt{false} in both cex and sat instance, while the concrete expression (2) evaluates to
\texttt{true} in cex and \texttt{false} in the sat instance.
Thus, the boolean score for the expression under analysis is 1 as the aggregation of the values obtained for the concrete expressions (1) and (2).


{\tool} then computes the relational score for the expression under analysis as the sum of the relational scores for its children: \texttt{s.transition} and \texttt{none}, both of which are leaves. 
%\texttt{s.transition} gets a score of 0.25 and \texttt{none} gets a score of 0.
To compute the score for \texttt{s.transtion}, it is instantiated to \texttt{State1.transition} and \texttt{State3.transtion}. \texttt{State1.transition} evaluates to \texttt{State2} in both cex and sat instance. Thus, it gets a score of 0.
For \texttt{State3.transition}, in cex, it evaluates to \texttt{State1} and gets a score of 1 as the size of different values \{\texttt{State3, State1}\} divided by the size of the instantiated values \{\texttt{State3}\} and the evaluated values \{\texttt{State1}\}. In sat instance, it evaluates to an empty set and gets a score of 0.
%Thus, \texttt{State3.transition} get a score of 0.5 as the average for cex and sat instance.
Overall, \texttt{s.transition} gets a relational score of 0.25 as the average of all its instantiated expressions: \texttt{State1.transition} (0) and \texttt{State3.transition} (0.5). Finally, the overall score of 1.25 is assigned to the expression \texttt{s.transition = none} as the aggregation of its boolean and relational scores. 
%Similarly, \texttt{none} gets a score of 0. Thus (b) gets a relational score of 0.25 as the sum of all its children's score. Overall, (b) get a score of 1.25. 
%\\\textbf{HB: The highlighted sentences are vague and hard to understand.}



\subsubsection{UNSAT Core Analyzer}
\label{sec:unsat}
It is possible that we can only generate cex's, but no sat instances, indicating that some constraints in the model have conflicts with the property we want to check.
To identify these constraints, {\tool} inspects the \emph{unsat core} returned by the Alloy Analyzer.
The unsat core explains why a set of constraints cannot be satisfied by giving a minimal subset of conflicting constraints.
Those conflicting constraints can help {\tool} identify suspicious expressions.

\begin{algorithm}[t]
  \small
  \DontPrintSemicolon
  \SetAlgoLined  
%\hline
%\hline
  \Input{Alloy model $M$, unsat core $U$, counterexample $c$}
  \Output{a set of expressions in $M$}
%  \BlankLine
%\hline
  $M' \leftarrow \slice(M, U)$\;
  $\sin \leftarrow \PMaxSolver(M', \cex)$\;
  $\diffs \leftarrow \comparator(\{(\cex, \sin)\})$\;
  $\exprs \leftarrow \collect(U)$\;
  $\conflicts \leftarrow \emptyset$\;
  \ForEach{$\expr \in \exprs$}{
    \ForEach{$\diff \in \diffs$}{
      \uIf{$\eval(\expr, \diff, M') = \false$}{
        $\conflicts \leftarrow \conflicts \cup \expr$\;
      }
    }
  }
  \Return $\conflicts$\;
%\hline
%\hline
  \caption{UNSAT Analyzer}
  \label{algo:unsatanalyzer}
\end{algorithm}
%There are two ways to identify conflicting constraints from unsat core.
%First is a ``delta-debugging'' approach where we attempt to remove the conflicting constraint 
%deleting each constraint one by one and re-run predicate to see if there is still unsat, if yes, then this constraint may not be the cause, else this constraint is definitely the cause. However, this method doesn't work when two constraints leads to the bug. Then we will have to check each two of the unsat core, then three til all constraints in unsat core. This leads to many calls to solvers.

Algorithm~\ref{algo:unsatanalyzer} outlines the process underlying our UNSAT core analyzer, 
which takes as input a model $M$, an unsat core $U$, and a cex $c$ showing $M$ does not satisfy a property $p$, and outputs a list of expressions in $M$ conflicting with $p$.
Recall that these values, $M$, $U$, and $c$, are earlier inferred by {\tool} as outlined in Algorithm~\ref{algo:overview}.

{\tool} starts by producing a sliced model $M'$, in which  all expressions in the unsat core are omitted from the original model $M$. Removing these conflicting expressions would allow us to obtain sat instances from the new model $M'$ to compare with the cex.
{\tool} now generates a minimal sat instance from $M'$ and compares it with the input cex to obtain the differences between the cex and the sat instance as shown in Section~\ref{sec:comparator}.
Then, {\tool} attempts to identify which of the removed expressions really conflict with $p$ by evaluating them on obtained differences.
The idea is that if an expression evaluates to true, then adding that expression back to the model would still allow the sat instance to be generated, i.e., that expression is not conflicting with $p$.
Thus, expressions that evaluate to \texttt{false} are ones conflicting with $p$ and are returned as suspicious expressions.
Note that we assign similar scores to these resulting expressions because they all contribute to the unsatisfiability of the original model and the intended property.

%Then for each boolean expression collected, {\tool} evaluates it using the value from the difference, if it is evaluated false, then {\tool} add it to the conflicts list. 

For example, if we change line~\ref{line:unsat1} in the model shown in Figure~\ref{fig:ex} to \texttt{all s: State | s.transition !in FSM.start}, Alloy would find counterexamples such as the one in Figure~\ref{fig:cex1}, but fail to generate any sat instances. This is because the modified line forces all states to have some transitions, which conflicts with the constraint requiring no transition for stop states. 

From the unsat core, %provided by the Alloy Analyzer, 
{\tool} identifies four expressions in the model: (a) \texttt{all start1, start2 : FSM.start | start1 = start2}, (b) \texttt{some FSM.stop}, (c) \texttt{FSM.start !in FSM.stop} and (d) \texttt{all s: State | s.transition !in FSM.start}. After removing these four expressions from the model, {\tool} can now generate the same sat instance in Figure~\ref{fig:expected1}.
As before, the main difference between the cex and sat instance involves two values:  \texttt{State1} and \texttt{State3}.
Then, {\tool} evaluates each expression using these values. Expressions (a), (b), and (c) are evaluated to \texttt{true} for both values, while expression (d) evaluates to \texttt{false} for \texttt{State3}. Thus, {\tool} correctly identifies (d) as the suspicious expression.


\begin{comment}
\subsection{Instance Satisfiability}
\label{sec:4cases}

\begin{figure}[t]
  \begin{subfigure}{0.24\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{res/algo/ncne.png}
    \caption{}
    \label{fig:nocexnoexp}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{res/algo/nce.png}
    \caption{}
    \label{fig:nocexexp}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{res/algo/cne.png}
    \caption{}
    \label{fig:cexnoexp}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{res/algo/ce.png}
    \caption{}
    \label{fig:cexexp}
  \end{subfigure}
  \caption{Four cases when checking a property: (a) No Cex, No Sat; (b) Sat, No Cex; (c) Cex, No Sat; (d) Cex, Sat} 
  \label{fig:4cases}
\end{figure}

Given an Alloy model $M$ and a property $p$, Figure~\ref{fig:4cases} shows four main cases about the  satisfiability of $M$'s instances with respect to $p$ .
%% The process of checking a property $p$ in a model $M$ typically results in the four cases shown in Figure~\ref{fig:4cases}.
The circle represents the state space consisting of all instances of $M$.% {\tool} is only applicable to cases when we can obtain cex's representing  
%instances of $M$ that do not satisfy $p$.

In Figure~\ref{fig:nocexnoexp}, we cannot obtain any instances of $M$ that do or do not satisfy $p$ (i.e., no cex's or sat instances).
This could occur when $M$ contains conflicting constraints, e.g., they evaluate to \texttt{false} and thus there are no instances at all.
{\tool} cannot be applied to this case as the Alloy Analyzer cannot generate any cex indicating the violation of $p$.
In Figure~\ref{fig:nocexexp}, every instance of $M$ satisfies $p$ (i.e., no cex's).
{\tool} is not applicable in this case as there is no assertion violation.

In Figure~\ref{fig:cexnoexp}, we can only obtain cex's, but no sat instances, i.e., every instance of $M$ violates $p$.
In this case {\tool} analyzes the unsat core to localize expressions in $M$ that do not satisfy $p$ (Section~\ref{sec:unsat}).
Finally, in Figure~\ref{fig:cexexp}, we can obtain both cex's and sat instances.
This is the typical assertion violation situation that {\tool} is designed to effectively handle (Section~\ref{sec:alg}).
\end{comment}




%% \subsubsection{Discussions}

%% \paragraph{When {\tool} doesn't Work Well} For situations in Fig ~\ref{fig:cexexp}, \tool works well when the error is caused by existing expression in the model and modifying the expression, like changing operators or deleting some subexpressions could repair the bug. But when the error is a completely missing expression, where a completely new expression needed to repair the bug, \tool would locate the error to some other exisiting correct expressions. For example, in the motivating example, if line 18 is deleted in the original model, given the same assertion, \tool will locate to line 17 instead.


%% \paragraph{Using Results from {\tool} to Repair Bugs}


==> pldi21/background.tex <==
\section{Background}

==> pldi21/discuss.tex <==
\section{Discussion}
For \textit{arr1.als}, no counter example or passing instance generated due to the following sentence is a false statement and no valid instance: $ all i:Int |i>=0 and i<Array.length $.

For overconstraint specification where there no counterexample generated for assert, we change the fact to pred1, then we insert a correct pred called pred2,  then we add an assert to check if pred1 equals to pred2 by saying that $pred1<=>pred2$.

We use assertion and predicate to fully automate the procedure for fault localization, this part can be modified to involve user in the loop. For example, the user may write a predicate and run Alloy to generate some instance. Then he spot some relationship or signature that should be removed(or added), he could select such relationship and our tool will point him to the possible bug locations.

==> pldi21/experiment.tex <==
\section{Evaluation}
\label{sec:eval}

{\tool} is implemented in Java and uses Alloy 4.2.
We extend the backend KodKod solver~\cite{kodkod} in Alloy to use the Pardinus solver~\cite{pardinus} to obtain sat instances similar to counterexamples.
We also modify the AST expression representation in Alloy to collect and assign suspicious scores to boolean and relational subexpressions. 

Our evaluation addresses the following research questions:
\begin{itemize}
\item \textbf{RQ1}: Can {\tool} effectively find suspicious expressions?
\item \textbf{RQ2}: How does {\tool} scale to large, complex models?
\item \textbf{RQ3}: How does {\tool} compare to AlloyFL? 
\end{itemize}

All experiments described below were performed on a Macbook with 2.2 GHZ i7 CPU and 16 GB of RAM.
%We note that {\tool} is deterministic because the Alloy analyzer and Pardinus produce the same output when running the same input on the same machine.
{\tool} and the experimental data are available at~\cite{BFA}.



\subsection{RQ1: Effectiveness}
\label{sec:arepair}

To investigate the effectiveness of {\tool}, we use the benchmark models from AlloyFL~\cite{alloyfl}.
Table~\ref{table:res1} shows 152 buggy models collected from 12 Alloy models in AlloyFL. 
These are real faults collected from Alloy release 4.1, Amalgam~\cite{whyandwhynot}, and Alloy homework solutions from graduate students.
Briefly, these models are \emph{addr} (address book) and \emph{farmer} (farmer cross-river puzzle) from Alloy; \emph{bempl} (bad employer), \emph{grade} (grade book) and \emph{other} (access-control specifications) are from Amalgam~\cite{whyandwhynot}; and \emph{arr} (array), \emph{bst} (balanced search tree), \emph{ctree} (colored tree), \emph{cd} (class diagram), \emph{dll} (doubly linked list), \emph{fsm} (finite state machine), and \emph{ssl} (sorted singly linked list) are homework from AlloyFL.


For models with assertions (e.g., from Amalgam~\cite{whyandwhynot}), we use those assertions for the experiments.
For models that do not have assertions (e.g., homework assignments), we manually create assertions and expected predicates by examining the correct versions or suggested fixes (provided by~\cite{alloyfl}).
Moreover, from the correct models or suggested fixes, we know which expressions contain errors and therefore use them as \emph{ground truths} to compare against {\tool}'s results.
{\tool} deals with models containing multiple violated assertions by analyzing them separately and returning a ranked list for each assertion.
For illustration purposes, we simulate this by simply splitting models with separate violations into separate models (e.g., \texttt{bst2} contains two assertion violations and thus are split into two models \texttt{bst2, bst2\_1}). Finally, {\tool} is highly automatic and has just one user-configurable option: the number of pairs of cex and satisfying instances (which by default is set to 5 based on our experiences).
% {\tool} can automatically find multiple faulty expressions within the same model (Section~\ref{sec:casestudies}).


%% in those benchmarks are already identified. To collect the result, we compare the output of {\tool} with the identified error locations. 


%% We use the assertions showing the errors in the faulty models if those assertions are available. Otherwise, we create assertions to show the existing of the bug.


%% Some of these faulty models come with their own assertions showing the violation; some do not.

%% if they come with their own assertions, we would use these assertions as oracle.
%% Otherwise, we will insert our own assertions trying to catch the error.\tvn{how many did came with their own assertions ?  how many you have to insert your own?  Give some examples how what assertions you have created? how do you know these have ``bugs'' to come up with these assertions?} \gz{add here} The 5 examples from Amalgam ~\cite{whyandwhynot} come with their own assertions and we directly use these assertions as oracle. The other 37 examples doesn't contain any assertions, we insert our own assertions to catch the error. The assertion is created by asserting that the buggy constraint equal to the correct constraint, in the format that \code{BuggyConstraint <=> CorrectConstraint}. For example, for a buggy predicate \code{pred ObjectNoExt\(\) \{all c: Class | Object !in c.ext\}} in cd1, we create the following assertion \code{assert \{ObjectNoExt <=>  all c: Class | Object !in c.~^ext\}}. The buggy version and correct version are obtained from ARepair's~\cite{arepair} annotation of buggy location and suggested fix. 


%\tvn{STOP here for now}

%% \paragraph{Implementation} Talk about your tool implementation (should also try to come up with a catchy name for it).  Written in Java (how many LoC's?),  use Alloy version X,  and other external tools.  

%% \paragraph{Benchmarks} Talk about the collected benchmarks here. General information such as what they are (what do they model),  how real are they (synthetic, real ?).  

%% Then talk about how "big" they are in term of AST node (because your fault localization works at this level).  

%% \paragraph{Setup}  Describe what you do the the benchmarks , e.g., do you insert your own assertion ?  do you randomly mutate the models ?  How do you mutate them ?  Refer to the numbers in the table when talking about this.  

%% \paragraph{Research questions}  Describe the questions your experiment want to answer.

% \begin{table}
%     \caption{Results for models collected from ARepair~\cite{arepair}.}
%     \label{table:res}
%    \small
%     \begin{tabular}{c c | c c c c}
%       \hline
%       \hline
%       model     & loc & \# rel   & \# val  & \# slice   &  r/t   \\
%       \hline      
%     addr1     &  21          &  1       & 3       &   10       &  1/74   \\ 
%     arr2      &  32          &  3       & 8       &   4        &  1/60       \\ 
%     bst1      &  50          &  5       & 4       &   104      &  $3*$/150     \\  
%     bst2\_1   &  48          &  3       & 2       &   52       &  1/125      \\  
%     bst2\_2   &  43          &  7       & 5       &   88       &  5/143   \\  
%     bst2\_3   &  46          &  5       & 3       &   65       &  $1^*$/129      \\    
%     bst3\_1   &  54          &  1       & 3       &   93       &  $1^*$/129      \\  
%     bst3\_2   &  53          &  5       & 3       &   60       &  1/133     \\  
%     cd1\_1    &  27          &  1       & 1       &   32       &  1/43      \\  
%     cd1\_2    &  26          &  1       & 2       &   30       &  1/43      \\  
%     cd2       &  28          &  1       & 2       &   25       &  1/35      \\  
%     dll1\_1   &  39          &  1       & 3       &   67       &  1/81      \\  
%     dll1\_2   &  39          &  2       & 1       &   52       &  3/81      \\  
%     dll2\_1   &  43          &  1       & 3       &   63       &  1/77      \\  
%     dll2\_2   &  43          &  2       & 1       &   52       &  2/77      \\  
%     dll3\_2   &  38          &  2       & 1       &   46       &  1/72      \\  
%     dll4      &  39          &  2       & 3       &   43       &  1/81      \\  
%     fsm1\_1   &  29          &  2       & 1       &   18       &  1/88      \\ 
%     fsm2      &  28          &  2       & 1       &   13       &  4/68      \\  
%     stu1      &  47          &  1       & 2       &   148      &  2/184      \\  
%     stu2\_1   &  44          &  1       & 2       &   127      &  1/163    \\    
%     stu3\_1   &  48          &  2       & 2       &   137      &  3/199      \\   
%     stu3\_2   &  50          &  1       & 1       &   138      &  1/199      \\  
%     stu4      &  44          &  1       & 2       &   122      &  1/158      \\   
%     stu5      &  46          &  1       & 2       &   164      &  2/200      \\   
%     stu6\_1   &  45          &  1       & 1       &   115      &  2/159      \\  
%     stu7\_1   &  45          &  1       & 1       &   110      &  1/143      \\  
%     stu7\_2   &  47          &  1       & 1       &   109      &  1/143      \\  
%     stu8      &  47          &  1       & 2       &   123      &  2/178      \\  
%     stu9      &  53          &  2       & 2       &   120      &  11/165    \\  
%     stu10     &  47          &  1       & 1       &   123      &  2/167      \\  
%     stu11     &  46          &  2       & 2       &   136      &  1/189      \\  
%     stu12\_1  &  45          &  2       & 1       &   127      &  1/173      \\       
%     stu13     &  49          &  2       & 2       &   120      &  $4^*$/186      \\  
%     stu14\_1  &  44          &  2       & 2       &   106      &  1/152      \\  
%     stu15     &  45          &  2       & 2       &   110      &  1/173      \\  
%     stu17\_1  &  45          &  2       & 2       &   105      &  1/158      \\  
%     stu18\_1  &  44          &  2       & 2       &   124      &  2/174      \\  
%     stu18\_2  &  46          &  2       & 1       &   126      &  3/174      \\  
%     stu18\_3  &  52          &  1       & 3       &   91       &  12/174   \\  
%     stu19\_1  &  45          &  2       & 2       &   137      &  1/182      \\  
%     stu19\_2  &  53          &  1       & 3       &   115      &  1/182       \\
%     \hline
%     fsm1\_2   &  29          &  2       & 1       &   54       &  1/88      \\    
%     \hline
%     bempl1    &  22          &  1       & 2       &   7        &  -/14      \\   
%     ctree     &  26          &  1       & 1       &   5        &  -/49     \\  
%     dll3\_3   &  38          &  2       & 1       &   64       &  -/72      \\  
%     grade1    &  22         &  2       & 3       &   15       &  -/22      \\
%     stu6\_2   &  47          &  3       & 3       &   100      &  -/159      \\  
%     stu14\_2  &  46          &  3       & 3       &   100      &  -/152   \\  
%     stu16     &  40          &  1       & 1       &   67       &  -/84      \\        
%     stu17\_2  &  47          &  3       & 3       &   100      &  -/158     \\      
%     \hline
%     other1    &  24          &  1       & 2       &   19       &  -/24      \\   
%     stu2\_2   &  55          &  0       & 0       &   198      &  -/198      \\
%     stu12\_2  &  52          &  1       & 2       &   89       &  -/173      \\          
%     \hline    
%     dll3\_1   &  36          &  -       & -       &   -        &  -/74      \\   
%     arr1      &  26          &  -       & -       &   -        &  -/45    \\
%     \hline
%     \hline
% \end{tabular}
% \end{table}

% \begin{table*}
%   \begin{tabular}{lrl}
%     metrics& time  & models \\
%     \hline
%     top1 &&addr,arr3,arr4,arr5,arr6,arr7,bst2,bst2\_1,bst3\_2,cd1,cd1\_1,cd2,cd3,cd3\_1,dll1,dll3,dll3\_1,dll4,dll5\_1,dll6,dll7\_1,dll8,dll9,dll11,dll12,dll13,dll14\_1,dll15,dll2,dll16,dll17\_1,dll18,dll18\_1,fsm1\_1,ssl10,ssl12,ssl14,ssl17,ssl17\_1,ssl18\_1,ssl18\_2,ssl19,ssl14\_2,dll20,ssl1,ssl4,ssl5,ssl6,ssl14\_3,fsm9\_4,grade,ssl14\_1,ssl6\_3,ssl3\_1,ssl6\_1,ssl6\_2,ssl3,ssl7,ssl7\_1,fsm7\_1,ssl8,ssl2\\
%     top5 &&arr7\_1,arr8,arr9,arr11,bst2\_2, bst2\_3, bst3,bst8,bst8\_1,bst10\_3\\
%     top10&&bst3\_1, bst3\_2, bst6\\
%     $>$10&&bst4\_2,bst\_11\\
%     -&&bst4\\
%     \hline
%   \end{tabular}
% \end{table*}

% \begin{table*}[]
%   \centering
%   \caption{Results for models violating assertions}
%   \label{table:res}
%   \begin{tabular}{c|ccccc|cc||c|ccccc|cc}
%     \hline
%     model    & loc & \#rel & \#val & sliced & total & flack & time & model    & loc & \#rel & \#val & sliced & total & flack & time \\ \hline
%     addr                    & 21  & 1      & 3      & 10     & 74    & 1 & 0.6  &     &     &        &        &        &       &   &       \\
%     arr3                    & 24  & 1      & 3      & 9      & 48    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     arr4                    & 24  & 0      & 0      & 61     & 64    & 1 & 0.2  &     &     &        &        &        &       &   &       \\
%     arr5                    & 24  & 0      & 0      & 59     & 62    & 1 & 0.2  &     &     &        &        &        &       &   &       \\
%     arr6                    & 25  & 1      & 3      & 30     & 56    & 1 & 0.3  &     &     &        &        &        &       &   &       \\
%     arr7                    & 25  & 0      & 0      & 50     & 63    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     bst2                    & 56  & 3      & 2      & 56     & 134   & 1 & 0.4  &     &     &        &        &        &       &   &       \\
%     bst2\_1                 & 56  & 1      & 3      & 95     & 134   & 1 & 0.3  &     &     &        &        &        &       &   &       \\
%     bst3\_2                 & 55  & 5      & 3      & 68     & 141   & 1 & 0.2  &     &     &        &        &        &       &   &       \\
%     cd1                     & 27  & 1      & 1      & 33     & 44    & 1 & 0.0  &     &     &        &        &        &       &   &       \\
%     cd1\_1                  & 27  & 1      & 2      & 31     & 44    & 1 & 0.0  &     &     &        &        &        &       &   &       \\
%     cd2                     & 27  & 1      & 1      & 25     & 35    & 1 & 0.0  &     &     &        &        &        &       &   &       \\
%     cd3                     & 26  & 1      & 1      & 32     & 43    & 1 & 0.0  &     &     &        &        &        &       &   &       \\ 
%     cd3\_1                  & 26  & 1      & 1      & 31     & 46    & 1 & 0.0  &     &     &        &        &        &       &   &       \\
%     dll1                    & 37  & 1      & 3      & 63     & 77    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll3                    & 37  & 5      & 4      & 59     & 80    & 1 & 0.0  &     &     &        &        &        &       &   &       \\
%     dll3\_1                 & 37  & 2      & 1      & 49     & 75    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll4                    & 37  & 1      & 3      & 67     & 81    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll5\_1                 & 39  & 1      & 3      & 80     & 102   & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll6                    & 36  & 1      & 3      & 94     & 113   & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll7\_1                 & 36  & 1      & 3      & 59     & 73    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll8                    & 36  & 1      & 3      & 76     & 96    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll9                    & 38  & 2      & 1      & 91     & 100   & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll11                   & 36  & 1      & 3      & 68     & 87    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll12                   & 36  & 1      & 3      & 63     & 77    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll13                   & 36  & 2      & 3      & 51     & 60    & 1 & 0.0  &     &     &        &        &        &       &   &       \\
%     dll14\_1                & 37  & 1      & 3      & 71     & 85    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll15                   & 40  & 1      & 3      & 107    & 126   & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll2                    & 42  & 1      & 3      & 63     & 77    & 1 & 0.1  &     &     &        &        &        &       &   &       \\
%     dll16    & 36  & 1      & 3      & 68     & 82    & 1 & 0.1 \\
%     dll17\_1 & 36  & 1      & 3      & 63     & 77    & 1 & 0.1 \\
%     dll18    & 36  & 3      & 2      & 84     & 102   & 1 & 0.0 \\
%     dll18\_1 & 36  & 2      & 3      & 67     & 101   & 1 & 0.1 \\    
%     fsm1\_1  & 30  & 2      & 1      & 19     & 90    & 1 & 0.0 \\
%     ssl10    & 43  & 2      & 1      & 110    & 155   & 1 & 0.1 \\
%     ssl12    & 40  & 2      & 2      & 114    & 157   & 1 & 0.1 \\
%     ssl14    & 44  & 0      & 0      & 149    & 158   & 1 & 0.5 \\
%     ssl17    & 41  & 2      & 1      & 119    & 152   & 1 & 0.0 \\
%     ssl17\_1 & 42  & 2      & 1      & 106    & 152   & 1 & 0.1 \\
%     ssl18\_1 & 40  & 2      & 2      & 118    & 160   & 1 & 0.1 \\
%     ssl18\_2 & 49  & 1      & 3      & 85     & 160   & 1 & 0.3 \\    
%     ssl19    & 40  & 1      & 2      & 141    & 169   & 1 & 0.1 \\
%     ssl14\_2 & 43  & 2      & 1      & 120    & 153   & 1 & 0.0 \\
%     dll20    & 36  & 4      & 4      & 64     & 90    & 1 & 0.0 \\
%     ssl1     & 40  & 2      & 2      & 126    & 168   & 1 & 0.1 \\  
%     ssl4     & 40  & 1      & 2      & 118    & 146   & 1 & 0.1 \\      
%     ssl5     & 42  & 1      & 2      & 160    & 188   & 1 & 0.6 \\  
%     ssl6     & 42  & 0      & 0      & 148    & 157   & 1 & 0.7 \\      
%     ssl14\_3 & 44  & 2      & 2      & 108    & 153   & 1 & 0.1 \\
%     fsm9\_4  & 30  & 0      & 0      & 78     & 91    & 1 & 0.1 \\
%     grade    & 33  & 2      & 3      & 7      & 22    & 1 & 0.0 \\    
%     ssl14\_1 & 44  & 0      & 0      & 149    & 158   & 1 & 0.5 \\    
%     ssl6\_3  & 42  & 2      & 1      & 107    & 152   & 1 & 0.1 \\
%     ssl3\_1  & 44  & 3      & 2      & 121    & 184   & 1 & 0.2 \\
%     ssl6\_1  & 42  & 0      & 0      & 148    & 157   & 1 & 0.5 \\
%     ssl6\_2  & 41  & 2      & 1      & 119    & 152   & 1 & 0.1 \\
%     ssl3     & 45  & 1      & 1      & 135    & 188   & 1 & 0.0 \\
%     ssl7     & 41  & 2      & 1      & 95     & 136   & 1 & 0.1 \\    
%     ssl7\_1  & 40  & 1      & 1      & 110    & 135   & 1 & 0.1 \\
%     fsm7\_1  & 29  & 2      & 2      & 14     & 59    & 1 & 0.0 \\
%     ssl8     & 43  & 1      & 1      & 119    & 166   & 1 & 0.1 \\
%     ssl2     & 40  & 1      & 2      & 122    & 150   & 1 & 0.1 &     &     &        &        &        &       &   &      \\
%     \multicolumn{8}{c||}{}&     &     &        &        &        &       &   &      \\
%     arr7\_1                 & 24  & 2      & 9      & 9      & 46    & 2 & 0.9  & 
%     arr9                    & 27  & 1      & 3      & 43     & 83    & 2 & 0.2  & 
%     bst2\_3                 & 52  & 5      & 3      & 68     & 133   & 2 & 0.1  & 
%     bst12                   & 47  & 5      & 3      & 94     & 146   & 2 & 0.2  & 
%     bst18                   & 51  & 3      & 2      & 115    & 187   & 2 & 1.4  & 
%     bst19                   & 47  & 5      & 3      & 112    & 158   & 2 & 0.1  & 
%     bst19\_1                & 52  & 6      & 3      & 112    & 175   & 2 & 0.1  & 
%     dll2\_1                 & 42  & 2      & 1      & 57     & 82    & 2 & 0.0  &
%     dll18\_3                & 36  & 2      & 1      & 78     & 103   & 2 & 0.0 \\
%     dll19    & 36  & 1      & 3      & 63     & 83    & 2 & 0.1 \\
%     dll20\_1 & 36  & 1      & 3      & 68     & 88    & 2 & 0.1 \\
%     fsm6     & 29  & 2      & 2      & 17     & 98    & 2 & 0.0 \\
%     fsm9\_2  & 29  & 2      & 2      & 18     & 90    & 2 & 0.1 \\
%     dll17\_2 & 36  & 2      & 1      & 57     & 82    & 2 & 0.0 \\
%     dll20\_2 & 36  & 2      & 1      & 47     & 88    & 2 & 0.0 \\
%     ssl11    & 42  & 2      & 1      & 127    & 177   & 2 & 0.1   \\
    
%     arr8                    & 25  & 2      & 6      & 15     & 80    & 4 & 0.5  & 
%     arr11                   & 24  & 2      & 3      & 41     & 83    & 5 & 0.1  & 
%     bst2\_2                 & 47  & 7      & 5      & 92     & 147   & 4 & 0.1  &     
%     bst3                    & 57  & 1      & 3      & 97     & 137   & 4 & 0.1  & 
%     bst8                    & 59  & 3      & 2      & 57     & 134   & 3 & 0.3  &     
%     bst8\_1                 & 59  & 3      & 2      & 57     & 134   & 3 & 0.2  & 
%     bst10\_3                & 55  & 7      & 5      & 75     & 162   & 5 & 0.3  & 
%     dll1\_1                 & 38  & 2      & 1      & 57     & 86    & 3 & 0.1  & 
%     bst22\_1                & 49  & 3      & 2      & 124    & 199   & 3 & 0.1  &
%     dll18\_2 & 36  & 1      & 3      & 71     & 107   & 3 & 0.6 \\
%     ssl18    & 40  & 1      & 2      & 131    & 162   & 3 & 0.0 \\
    
%     fsm5\_2  & 29  & 2      & 2      & 17     & 69    & 3 & 0.0 \\
%     fsm2     & 29  & 2      & 1      & 14     & 70    & 4 & 0.0 \\
%     fsm9\_1  & 29  & 2      & 1      & 18     & 91    & 5 & 0.1 \\
%     fsm8     & 29  & 3      & 1      & 14     & 71    & 4 & 0.1 \\
%     ssl2\_1  & 44  & 2      & 2      & 72     & 156   & 3 & 0.1 \\
%     ssl13    & 43  & 1      & 1      & 123    & 174   & 3 & 0.1   \\
%     ssl15    & 41  & 2      & 1      & 106    & 161   & 5 & 0.1   \\
%     fsm4     & 31  & 2      & 3      & 39     & 141   & 3 & 0.0 \\
    
%     bst3\_1                 & 57  & 3      & 2      & 58     & 137   & 6 & 0.2  & 
%     bst6                    & 51  & 7      & 5      & 61     & 140   & 8 & 0.2  & 
%     bst12\_1                & 56  & 5      & 3      & 68     & 164   & 8 & 0.2  & 
%     bst17\_2                & 55  & 7      & 5      & 79     & 177   & 9 & 0.2  & 
%     bst19\_2                & 55  & 5      & 3      & 86     & 154   & 8 & 0.2  & 
%     bst20\_1                & 55  & 7      & 5      & 61     & 152   & 6 & 0.2  & 
%     fsm7     & 29  & 2      & 2      & 14     & 64    & 6 & 0.1 \\
%     ssl19\_1 & 50  & 2      & 3      & 106    & 175   & 7 & 0.6   \\
%     ssl19\_2 & 44  & 1      & 3      & 81     & 174   & 8 & 0.3   \\
    
%     bst4\_2                 & 51  & 7      & 5      & 61     & 154   & 11& 0.3  & 
%     bst16                   & 64  & 7      & 5      & 79     & 181   & 12& 0.3  & 
%     bst17                   & 48  & 5      & 3      & 113    & 186   & 12& 0.2  & 
%     bst22\_2                & 54  & 6      & 3      & 118    & 209   & 10& 0.1  & 
%     bst22\_3                & 57  & 5      & 5      & 74     & 199   & 16& 0.5  & 
%     ssl12\_1 & 44  & 3      & 3      & 78     & 161   & 12& 0.4   \\
%     ssl9     & 44  & 2      & 2      & 72     & 153   & 13& 0.1   \\
    
%     bst4                    & 46  & 5      & 3      & 95     & 145   & - & 0.1  & 
%     bst11                   & 54  & 5      & 3      & 135    & 196   & - & 0.2  & 
%     bempl                   & 51  & 1      & 2      & 7      & 14    & - & 0.0  & 
%     ctree                   & 30  & 1      & 1      & 5      & 49    & - & 0.0  & 
%     dll3\_2                 & 36  & 2      & 1      & 67     & 75    & - & 0.0  &
%     ssl16\_1 & 39  & 2      & 2      & 115    & 133   & - & 0.0   \\
%     other    & 34  & 1      & 2      & 19     & 26    & - & 0.0 \\
%     ssl16    & 39  & 2      & 2      & 119    & 137   & - & 0.0   \\    
%     ssl16\_2 & 47  & 2      & 4      & 74     & 136   & - & 0.3   \\
%     ssl16\_3 & 43  & 2      & 2      & 71     & 133   & - & 0.2   \\


%     \hline
%   \end{tabular}
% \end{table*}
\begin{table*}[]
  \centering
  \caption{Results of {\tool} on 152 Alloy models.  Results are sorted based on ranking accuracy. Times are in seconds.}
  \label{table:res1}
  \begin{tabular}{c|ccc@{\;\;}c@{\;\;}c||c|ccc@{\;\;}c@{\;\;}c||c|ccc@{\;\;}c@{\;\;}c}
    \textbf{model}    & \textbf{loc} & \textbf{total} & \textbf{sliced} & \textbf{rank} & \textbf{time} & \textbf{model}    & \textbf{loc} &  \textbf{total} & \textbf{sliced} & \textbf{rank} & \textbf{time} & \textbf{model} & \textbf{loc} & \textbf{total} & \textbf{sliced} & \textbf{rank} & \textbf{time} \\
    \midrule
    \cellcolor[gray]{.75}\textbf{top 1 (91)} & \cellcolor[gray]{.75}\textbf{41} & \cellcolor[gray]{.75}\textbf{120} & \cellcolor[gray]{.75}\textbf{95} & \cellcolor[gray]{.75}\textbf{1} & \cellcolor[gray]{.75}\textbf{0.2} & ssl10                 & 43          & 155          & 110         & 1            & 0.1          & dll20\_2                      & 36          & 88           & 47          & 2             & 0.0          \\ \cline{1-6}
    addr                & 21          & 74           & 10          & 1          & 0.6          & ssl12                 & 40          & 157          & 114         & 1            & 0.1          & fsm6                          & 29          & 98           & 17          & 2             & 0.0          \\
    arr3                & 24          & 48           & 9           & 1          & 0.1          & ssl14                 & 44          & 158          & 149         & 1            & 0.5          & fsm9\_2                       & 29          & 90           & 18          & 2             & 0.1          \\
    arr4                & 24          & 64           & 61          & 1          & 0.2          & ssl14\_1              & 44          & 158          & 149         & 1            & 0.5          & ssl11                         & 42          & 177          & 127         & 2             & 0.1          \\
    arr5                & 24          & 62           & 59          & 1          & 0.2          & ssl14\_2              & 43          & 153          & 120         & 1            & 0.0          & bst8                          & 59          & 134          & 57          & 3             & 0.3          \\
    arr6                & 25          & 56           & 30          & 1          & 0.3          & ssl14\_3              & 44          & 153          & 108         & 1            & 0.1          & bst8\_1                       & 59          & 134          & 57          & 3             & 0.2          \\
    arr7                & 25          & 63           & 50          & 1          & 0.1          & ssl17                 & 41          & 152          & 119         & 1            & 0.0          & bst22\_1                      & 49          & 199          & 124         & 3             & 0.1          \\
    bst2                & 56          & 134          & 56          & 1          & 0.4          & ssl17\_1              & 42          & 152          & 106         & 1            & 0.1          & dll1\_1                       & 38          & 86           & 57          & 3             & 0.1          \\
    bst2\_1             & 56          & 134          & 95          & 1          & 0.3          & ssl18\_1              & 40          & 160          & 118         & 1            & 0.1          & dll18\_2                      & 36          & 107          & 71          & 3             & 0.6          \\
    bst3\_2             & 55          & 141          & 68          & 1          & 0.2          & ssl18\_2              & 49          & 160          & 85          & 1            & 0.3          & fsm4                          & 31          & 141          & 39          & 3             & 0.0          \\
    cd1                 & 27          & 44           & 33          & 1          & 0.0          & ssl19                 & 40          & 169          & 141         & 1            & 0.1          & fsm5\_2                       & 29          & 69           & 17          & 3             & 0.0          \\
    cd1\_1              & 27          & 44           & 31          & 1          & 0.0          & \textit{arr1}         & 24          & 45           & 31          & 1            & 0.1          & ssl2\_1                       & 44          & 156          & 72          & 3             & 0.1          \\
    cd2                 & 27          & 35           & 25          & 1          & 0.0          & \textit{arr2}         & 25          & 60           & 47          & 1            & 0.2          & ssl13                         & 43          & 174          & 123         & 3             & 0.1          \\
    cd3                 & 26          & 43           & 32          & 1          & 0.0          & \textit{arr10}        & 24          & 59           & 45          & 1            & 0.0          & ssl18                         & 40          & 162          & 131         & 3             & 0.0          \\
    cd3\_1              & 26          & 46           & 31          & 1          & 0.0          & \textit{bst1}         & 51          & 171          & 155         & 1            & 0.2          & arr8                          & 25          & 80           & 15          & 4             & 0.5          \\
    dll1                & 37          & 77           & 63          & 1          & 0.1          & \textit{bst4\_1}      & 52          & 163          & 147         & 1            & 0.1          & bst2\_2                       & 47          & 147          & 92          & 4             & 0.1          \\
    dll2                & 42          & 77           & 63          & 1          & 0.1          & \textit{bst5}         & 52          & 184          & 168         & 1            & 0.1          & bst3                          & 57          & 137          & 97          & 4             & 0.1          \\
    dll3                & 37          & 80           & 59          & 1          & 0.0          & \textit{bst7}         & 52          & 159          & 143         & 1            & 0.1          & fsm2                          & 29          & 70           & 14          & 4             & 0.0          \\
    dll3\_1             & 37          & 75           & 49          & 1          & 0.1          & \textit{bst8\_2}      & 54          & 156          & 140         & 1            & 0.1          & fsm8                          & 29          & 71           & 14          & 4             & 0.1          \\
    dll4                & 37          & 81           & 67          & 1          & 0.1          & \textit{bst9}         & 55          & 185          & 169         & 1            & 0.1          & arr11                         & 24          & 83           & 41          & 5             & 0.1          \\
    dll5\_1             & 39          & 102          & 80          & 1          & 0.1          & \textit{bst10}        & 47          & 157          & 140         & 1            & 0.6          & bst10\_3                      & 55          & 162          & 75          & 5             & 0.3          \\
    dll6                & 36          & 113          & 94          & 1          & 0.1          & \textit{bst10\_2}     & 52          & 172          & 156         & 1            & 0.1          & fsm9\_1                       & 29          & 91           & 18          & 5             & 0.1          \\
    dll7\_1             & 36          & 73           & 59          & 1          & 0.1          & \textit{bst11\_1}     & 60          & 214          & 198         & 1            & 0.1          & ssl15                         & 41          & 161          & 106         & 5             & 0.1          \\ \cline{13-18} 
    dll8                & 36          & 96           & 76          & 1          & 0.1          & \textit{bst13}        & 53          & 200          & 184         & 1            & 0.1          & \cellcolor[gray]{.75}\textbf{top 6-10 (10)}        & \cellcolor[gray]{.75}\textbf{51} & \cellcolor[gray]{.75}\textbf{155} & \cellcolor[gray]{.75}\textbf{73} & \cellcolor[gray]{.75}\textbf{7.6}  & \cellcolor[gray]{.75}\textbf{0.2} \\ \cline{13-18} 
    dll9                & 38          & 100          & 91          & 1          & 0.1          & \textit{bst14}        & 59          & 202          & 186         & 1            & 0.1          & bst3\_1                       & 57          & 137          & 58          & 6             & 0.2          \\
    dll11               & 36          & 87           & 68          & 1          & 0.1          & \textit{bst15}        & 53          & 197          & 181         & 1            & 0.1          & bst20\_1                      & 55          & 152          & 61          & 6             & 0.2          \\
    dll12               & 36          & 77           & 63          & 1          & 0.1          & \textit{bst17\_1}     & 52          & 201          & 185         & 1            & 0.1          & fsm7                          & 29          & 64           & 14          & 6             & 0.1          \\
    dll13               & 36          & 60           & 51          & 1          & 0.0          & \textit{bst18\_1}     & 56          & 204          & 188         & 1            & 0.1          & ssl19\_1                      & 50          & 175          & 106         & 7             & 0.6          \\
    dll14\_1            & 37          & 85           & 71          & 1          & 0.1          & \textit{bst20}        & 52          & 169          & 153         & 1            & 0.1          & bst6                          & 51          & 140          & 61          & 8             & 0.2          \\
    dll15               & 40          & 126          & 107         & 1          & 0.1          & \textit{bst21}        & 52          & 182          & 166         & 1            & 0.2          & bst12\_1                      & 56          & 164          & 68          & 8             & 0.2          \\
    dll16               & 36          & 82           & 68          & 1          & 0.1          & \textit{bst22}        & 50          & 213          & 158         & 1            & 0.6          & bst19\_2                      & 55          & 154          & 86          & 8             & 0.2          \\
    dll17\_1            & 36          & 77           & 63          & 1          & 0.1          & \textit{dll7}         & 38          & 90           & 79          & 1            & 0.1          & ssl19\_2                      & 44          & 174          & 81          & 8             & 0.3          \\
    dll18               & 36          & 102          & 84          & 1          & 0.0          & \textit{dll10}        & 40          & 91           & 85          & 1            & 0.2          & bst17\_2                      & 55          & 177          & 79          & 9             & 0.2          \\
    dll18\_1            & 36          & 101          & 67          & 1          & 0.1          & \textit{dll14}        & 39          & 102          & 91          & 1            & 0.1          & bst22\_2                      & 54          & 209          & 118         & 10            & 0.1          \\ \cline{13-18} 
    dll20               & 36          & 90           & 64          & 1          & 0.0          & \textit{dll17}        & 37          & 89           & 83          & 1            & 0.1          & \cellcolor[gray]{.75}\textbf{\textgreater{}10 (6)} & \cellcolor[gray]{.75}\textbf{51} & \cellcolor[gray]{.75}\textbf{172} & \cellcolor[gray]{.75}\textbf{80} & \cellcolor[gray]{.75}\textbf{12.7} & \cellcolor[gray]{.75}\textbf{0.3} \\ \cline{13-18} 
    farmer              & 99          & 124          & 30          & 1          & 1.6          & \textit{fsm1}         & 31          & 90           & 71          & 1            & 0.0          & bst4\_2                       & 51          & 154          & 61          & 11            & 0.3          \\
    fsm1\_1             & 30          & 90           & 19          & 1          & 0.0          & \textit{fsm3}         & 60          & 67           & 56          & 1            & 0.7          & bst16                         & 64          & 181          & 79          & 12            & 0.3          \\
    fsm7\_1             & 29          & 59           & 14          & 1          & 0.0          & \textit{fsm9}         & 30          & 91           & 79          & 1            & 0.5          & bst17                         & 48          & 186          & 113         & 12            & 0.2          \\
    fsm9\_4             & 30          & 91           & 78          & 1          & 0.1          & \textit{fsm9\_3}      & 32          & 91           & 78          & 1            & 0.1          & ssl12\_1                      & 44          & 161          & 78          & 12            & 0.4          \\ \cline{7-12}
    grade               & 33          & 22           & 7           & 1          & 0.0          & \cellcolor[gray]{.75}\textbf{top 2-5 (35)} & \cellcolor[gray]{.75}\textbf{40} & \cellcolor[gray]{.75}\textbf{120} & \cellcolor[gray]{.75}\textbf{66} & \cellcolor[gray]{.75}\textbf{2.9} & \cellcolor[gray]{.75}\textbf{0.2} & ssl9                          & 44          & 153          & 72          & 13            & 0.1          \\ \cline{7-12}
    ssl1                & 40          & 168          & 126         & 1          & 0.1          & arr7\_1               & 24          & 46           & 9           & 2            & 0.9          & bst22\_3                      & 57          & 199          & 74          & 16            & 0.5          \\ \cline{13-18} 
    ssl2                & 40          & 150          & 122         & 1          & 0.1          & arr9                  & 27          & 83           & 43          & 2            & 0.2          & \cellcolor[gray]{.75}\textbf{fail (10)}            & \cellcolor[gray]{.75}\textbf{42} & \cellcolor[gray]{.75}\textbf{104} & \cellcolor[gray]{.75}\textbf{71} & \cellcolor[gray]{.75}\textbf{-}    & \cellcolor[gray]{.75}\textbf{0.1} \\ \cline{13-18} 
    ssl3                & 45          & 188          & 135         & 1          & 0.0          & bst2\_3               & 52          & 133          & 68          & 2            & 0.1          & bst4                          & 46          & 145          & 95          & -             & 0.1          \\
    ssl3\_1             & 44          & 184          & 121         & 1          & 0.2          & bst12                 & 47          & 146          & 94          & 2            & 0.2          & bst11                         & 54          & 196          & 135         & -             & 0.2          \\
    ssl4                & 40          & 146          & 118         & 1          & 0.1          & bst18                 & 51          & 187          & 115         & 2            & 1.4          & bempl                         & 51          & 14           & 7           & -             & 0.0          \\
    ssl5                & 42          & 188          & 160         & 1          & 0.6          & bst19                 & 47          & 158          & 112         & 2            & 0.1          & ctree                         & 30          & 49           & 5           & -             & 0.0          \\
    ssl6                & 42          & 157          & 148         & 1          & 0.7          & bst19\_1              & 52          & 175          & 112         & 2            & 0.1          & dll3\_2                       & 36          & 75           & 67          & -             & 0.0          \\
    ssl6\_1             & 42          & 157          & 148         & 1          & 0.5          & dll2\_1               & 42          & 82           & 57          & 2            & 0.0          & other                         & 34          & 26           & 19          & -             & 0.0          \\
    ssl6\_2             & 41          & 152          & 119         & 1          & 0.1          & dll17\_2              & 36          & 82           & 57          & 2            & 0.0          & ssl16                         & 39          & 137          & 119         & -             & 0.0          \\
    ssl6\_3             & 42          & 152          & 107         & 1          & 0.1          & dll18\_3              & 36          & 103          & 78          & 2            & 0.0          & ssl16\_1                      & 39          & 133          & 115         & -             & 0.0          \\
    ssl7                & 41          & 136          & 95          & 1          & 0.1          & dll19                 & 36          & 83           & 63          & 2            & 0.1          & ssl16\_2                      & 47          & 136          & 74          & -             & 0.3          \\
    ssl7\_1             & 40          & 135          & 110         & 1          & 0.1          & dll20\_1              & 36          & 88           & 68          & 2            & 0.1          & ssl16\_3                      & 43          & 133          & 71          & -             & 0.2          \\
    ssl8                & 43          & 166          & 119         & 1          & 0.1          &                       &             &              &             &              &              &                               &             &              &             &               &             
    \\
    \bottomrule
  \end{tabular}
  \end{table*}



% \begin{table*}[]
%   \centering
%   \caption{Results for models violating assertions}
%   \label{table:res}
%   \begin{tabular}{c|ccccc|cc|cc||c|ccccc|cc|cc}
%   \hline
%   model    & loc & \#rel & \#val & sliced & total & flack & time & afl & at  & model    & loc & \#rel & \#val & sliced & total & flack & time & afl & at  \\ \hline
%   addr                    & 21  & 1      & 3      & 10     & 74    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.6}  & \cellcolor[HTML]{C0C0C0}1  & 9.2   & dll16    & 36  & 1      & 3      & 68     & 82    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 7.4   \\
%   arr3                    & 24  & 1      & 3      & 9      & 48    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 6.1   & dll17\_1 & 36  & 1      & 3      & 63     & 77    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 7.3   \\
%   arr4                    & 24  & 0      & 0      & 61     & 64    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.2}  & \cellcolor[HTML]{C0C0C0}1  & 8.7   & dll17\_2 & 36  & 2      & 1      & 57     & 82    & 2                         & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}1  & 7.8   \\
%   arr5                    & 24  & 0      & 0      & 59     & 62    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.2}  & \cellcolor[HTML]{C0C0C0}1  & 5.8   & dll18    & 36  & 3      & 2      & 84     & 102   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.0}  & 3                          & 14.2  \\
%   arr6                    & 25  & 1      & 3      & 30     & 56    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.3}  & 2                          & 4.4   & dll18\_1 & 36  & 2      & 3      & 67     & 101   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 103.8 \\
%   arr7                    & 25  & 0      & 0      & 50     & 63    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 6.9   & dll18\_2 & 36  & 1      & 3      & 71     & 107   & 3                         & \textbf{0.6}  & \cellcolor[HTML]{9B9B9B}1  & 44.2  \\
%   arr7\_1                 & 24  & 2      & 9      & 9      & 46    & 2                         & \textbf{0.9}  & \cellcolor[HTML]{9B9B9B}1  & 5.7   & dll18\_3 & 36  & 2      & 1      & 78     & 103   & 2                         & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}1  & 29.5  \\
%   arr8                    & 25  & 2      & 6      & 15     & 80    & 4                         & \textbf{0.5}  & \cellcolor[HTML]{9B9B9B}1  & 8.8   & dll19    & 36  & 1      & 3      & 63     & 83    & 2                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 7.7   \\
%   arr9                    & 27  & 1      & 3      & 43     & 83    & 2                         & \textbf{0.2}  & 2                          & 8     & dll20    & 36  & 4      & 4      & 64     & 90    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.0}  & 4                          & 8.3   \\
%   arr11                   & 24  & 2      & 3      & 41     & 83    & 5                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 7     & dll20\_1 & 36  & 1      & 3      & 68     & 88    & 2                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 8.3   \\
%   bst2                    & 56  & 3      & 2      & 56     & 134   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.4}  & 12                         & 68.3  & dll20\_2 & 36  & 2      & 1      & 47     & 88    & 2                         & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}1  & 7.6   \\
%   bst2\_1                 & 56  & 1      & 3      & 95     & 134   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.3}  & 13                         & 68.5  & fsm1\_1  & 30  & 2      & 1      & 19     & 90    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 2.9   \\
%   bst2\_2                 & 47  & 7      & 5      & 92     & 147   & 4                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}2  & 95.2  & fsm2     & 29  & 2      & 1      & 14     & 70    & 4                         & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}1  & 2.8   \\
%   bst2\_3                 & 52  & 5      & 3      & 68     & 133   & 2                         & \textbf{0.1}  & 2                          & 68.1  & fsm4     & 31  & 2      & 3      & 39     & 141   & 3                         & \textbf{0.0}  & 3                          & 4.7   \\
%   bst3                    & 57  & 1      & 3      & 97     & 137   & \cellcolor[HTML]{9B9B9B}4 & \textbf{0.1}  & 8                          & 70    & fsm5\_2  & 29  & 2      & 2      & 17     & 69    & \cellcolor[HTML]{9B9B9B}3 & \textbf{0.0}  & 9                          & 2.1   \\
%   bst3\_1                 & 57  & 3      & 2      & 58     & 137   & \cellcolor[HTML]{9B9B9B}6 & \textbf{0.2}  & 7                          & 71.2  & fsm6     & 29  & 2      & 2      & 17     & 98    & \cellcolor[HTML]{9B9B9B}2 & \textbf{0.0}  & 16                         & 3     \\
%   bst3\_2                 & 55  & 5      & 3      & 68     & 141   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.2}  & \cellcolor[HTML]{C0C0C0}1  & 68.6  & fsm7     & 29  & 2      & 2      & 14     & 64    & \cellcolor[HTML]{9B9B9B}6 & \textbf{0.1}  & 13                         & 2.6   \\
%   bst4                    & 46  & 5      & 3      & 95     & 145   & \textbf{-}                & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}4  & 70.4  & fsm7\_1  & 29  & 2      & 2      & 14     & 59    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.0}  & 9                          & 2.6   \\
%   bst4\_2                 & 51  & 7      & 5      & 61     & 154   & 11                        & \textbf{0.3}  & \cellcolor[HTML]{9B9B9B}1  & 84.8  & fsm8     & 29  & 3      & 1      & 14     & 71    & \cellcolor[HTML]{9B9B9B}4 & \textbf{0.1}  & 14                         & 2.7   \\
%   bst6                    & 51  & 7      & 5      & 61     & 140   & 8                         & \textbf{0.2}  & \cellcolor[HTML]{9B9B9B}1  & 69.4  & fsm9\_1  & 29  & 2      & 1      & 18     & 91    & 5                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 3.1   \\
%   bst8                    & 59  & 3      & 2      & 57     & 134   & \cellcolor[HTML]{9B9B9B}3 & \textbf{0.3}  & 8                          & 62.8  & fsm9\_2  & 29  & 2      & 2      & 18     & 90    & 2                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 2.9   \\
%   bst8\_1                 & 59  & 3      & 2      & 57     & 134   & \cellcolor[HTML]{9B9B9B}3 & \textbf{0.2}  & 8                          & 62.7  & fsm9\_4  & 30  & 0      & 0      & 78     & 91    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 1.5   \\
%   bst10\_3                & 55  & 7      & 5      & 75     & 162   & 5                         & \textbf{0.3}  & \cellcolor[HTML]{9B9B9B}4  & 9  & grade    & 33  & 2      & 3      & 7      & 22    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 4.1   \\
%   bst11                   & 54  & 5      & 3      & 135    & 196   & \textbf{-}                & \textbf{0.2}  & \cellcolor[HTML]{9B9B9B}31 & 77    & other    & 34  & 1      & 2      & 19     & 26    & \textbf{-}                & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}11 & 1.4   \\
%   bst12                   & 47  & 5      & 3      & 94     & 146   & \cellcolor[HTML]{9B9B9B}2 & \textbf{0.2}  & \textbf{-}                 & 0.6   & ssl1     & 40  & 2      & 2      & 126    & 168   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 25.7  \\
%   bst12\_1                & 56  & 5      & 3      & 68     & 164   & 8                         & \textbf{0.2}  & \cellcolor[HTML]{9B9B9B}6  & 62.9  & ssl2     & 40  & 1      & 2      & 122    & 150   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 26.5  \\
%   bst16                   & 64  & 7      & 5      & 79     & 181   & 12                        & \textbf{0.3}  & \cellcolor[HTML]{9B9B9B}3  & 76.9  & ssl2\_1  & 44  & 2      & 2      & 72     & 156   & 3                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}2  & 46.9  \\
%   bst17                   & 48  & 5      & 3      & 113    & 186   & 12                        & \textbf{0.2}  & \cellcolor[HTML]{9B9B9B}1  & 113.7 & ssl3     & 45  & 1      & 1      & 135    & 188   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 81.1  \\
%   bst17\_2                & 55  & 7      & 5      & 79     & 177   & 9                         & \textbf{0.2}  & \cellcolor[HTML]{9B9B9B}1  & 83.9  & ssl3\_1  & 44  & 3      & 2      & 121    & 184   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.2}  & \cellcolor[HTML]{C0C0C0}1  & 65.4  \\
%   bst18                   & 51  & 3      & 2      & 115    & 187   & \cellcolor[HTML]{9B9B9B}2 & \textbf{1.4}  & \textbf{-}                 & 0.7   & ssl4     & 40  & 1      & 2      & 118    & 146   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 25.8  \\
%   bst19                   & 47  & 5      & 3      & 112    & 158   & 2                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 93.6  & ssl5     & 42  & 1      & 2      & 160    & 188   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.6}  & 3                          & 26.5  \\
%   bst19\_1                & 52  & 6      & 3      & 112    & 175   & \cellcolor[HTML]{9B9B9B}2 & \textbf{0.1}  & 10                         & 88.7  & ssl6     & 42  & 0      & 0      & 148    & 157   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.7}  & \cellcolor[HTML]{C0C0C0}1  & 30.2  \\
%   bst19\_2                & 55  & 5      & 3      & 86     & 154   & 8                         & \textbf{0.2}  & \cellcolor[HTML]{9B9B9B}2  & 50.1  & ssl6\_1  & 42  & 0      & 0      & 148    & 157   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.5}  & \cellcolor[HTML]{C0C0C0}1  & 31.7  \\
%   bst20\_1                & 55  & 7      & 5      & 61     & 152   & 6                         & \textbf{0.2}  & \cellcolor[HTML]{9B9B9B}2  & 83.3  & ssl6\_2  & 41  & 2      & 1      & 119    & 152   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 29.1  \\
%   bst22\_1                & 49  & 3      & 2      & 124    & 199   & \cellcolor[HTML]{9B9B9B}3 & \textbf{0.1}  & 12                         & 47.1  & ssl6\_3  & 42  & 2      & 1      & 107    & 152   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 31.2  \\
%   bst22\_2                & 54  & 6      & 3      & 118    & 209   & 10                        & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 98    & ssl7     & 41  & 2      & 1      & 95     & 136   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 58.7  \\
%   bst22\_3                & 57  & 5      & 5      & 74     & 199   & 16                        & \textbf{0.5}  & \cellcolor[HTML]{9B9B9B}4  & 75.7  & ssl7\_1  & 40  & 1      & 1      & 110    & 135   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 34.1  \\
%   \textit{\textbf{bempl}} & 51  & 1      & 2      & 7      & 14    & \textbf{-}                & \textbf{0.0}  & \textbf{-}                 & 1.9   & ssl8     & 43  & 1      & 1      & 119    & 166   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 35    \\
%   cd1                     & 27  & 1      & 1      & 33     & 44    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.0}  & 2                          & 0.8   & ssl9     & 44  & 2      & 2      & 72     & 153   & 13                        & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 47.4  \\
%   cd1\_1                  & 27  & 1      & 2      & 31     & 44    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 1.8   & ssl10    & 43  & 2      & 1      & 110    & 155   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 31.2  \\
%   cd2                     & 27  & 1      & 1      & 25     & 35    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 0.5   & ssl11    & 42  & 2      & 1      & 127    & 177   & \cellcolor[HTML]{9B9B9B}2 & \textbf{0.1}  & 4                          & 33.5  \\
%   cd3                     & 26  & 1      & 1      & 32     & 43    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.0}  & 2                          & 0.7   & ssl12    & 40  & 2      & 2      & 114    & 157   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 70.2  \\
%   cd3\_1                  & 26  & 1      & 1      & 31     & 46    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.0}  & 4                          & 1     & ssl12\_1 & 44  & 3      & 3      & 78     & 161   & 12                        & \textbf{0.4}  & \cellcolor[HTML]{9B9B9B}1  & 53.5  \\
%   \textit{\textbf{ctree}} & 30  & 1      & 1      & 5      & 49    & \textbf{-}                & \textbf{0.0}  & \textbf{-}                 & 4.2   & ssl13    & 43  & 1      & 1      & 123    & 174   & 3                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}1  & 67.8  \\
%   dll1                    & 37  & 1      & 3      & 63     & 77    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 7.3   & ssl14    & 44  & 0      & 0      & 149    & 158   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.5}  & \cellcolor[HTML]{C0C0C0}1  & 31.3  \\
%   dll1\_1                 & 38  & 2      & 1      & 57     & 86    & \cellcolor[HTML]{9B9B9B}3 & \textbf{0.1}  & \textbf{-}                 & 0.2   & ssl14\_1 & 44  & 0      & 0      & 149    & 158   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.5}  & \cellcolor[HTML]{C0C0C0}1  & 32    \\
%   dll2                    & 42  & 1      & 3      & 63     & 77    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 7.3   & ssl14\_2 & 43  & 2      & 1      & 120    & 153   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 30.6  \\
%   dll2\_1                 & 42  & 2      & 1      & 57     & 82    & 2                         & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}1  & 7.8   & ssl14\_3 & 44  & 2      & 2      & 108    & 153   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 31.6  \\
%   dll3                    & 37  & 5      & 4      & 59     & 80    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 7.4   & ssl15    & 41  & 2      & 1      & 106    & 161   & 5                         & \textbf{0.1}  & \cellcolor[HTML]{9B9B9B}3  & 35.5  \\
%   dll3\_1                 & 37  & 2      & 1      & 49     & 75    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 14.9  & ssl16    & 39  & 2      & 2      & 119    & 137   & \textbf{-}                & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}1  & 53.1  \\
%   dll3\_2                 & 36  & 2      & 1      & 67     & 75    & \textbf{-}                & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}1  & 13.2  & ssl16\_1 & 39  & 2      & 2      & 115    & 133   & \textbf{-}                & \textbf{0.0}  & \cellcolor[HTML]{9B9B9B}1  & 16.3  \\
%   dll4                    & 37  & 1      & 3      & 67     & 81    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 8.3   & ssl16\_2 & 47  & 2      & 4      & 74     & 136   & \textbf{-}                & \textbf{0.3}  & \cellcolor[HTML]{9B9B9B}1  & 16.9  \\
%   dll5\_1                 & 39  & 1      & 3      & 80     & 102   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 9.2   & ssl16\_3 & 43  & 2      & 2      & 71     & 133   & \textbf{-}                & \textbf{0.2}  & \cellcolor[HTML]{9B9B9B}1  & 40.6  \\
%   dll6                    & 36  & 1      & 3      & 94     & 113   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 9.3   & ssl17    & 41  & 2      & 1      & 119    & 152   & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 29.5  \\
%   dll7\_1                 & 36  & 1      & 3      & 59     & 73    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 7.1   & ssl17\_1 & 42  & 2      & 1      & 106    & 152   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 32.2  \\
%   dll8                    & 36  & 1      & 3      & 76     & 96    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 9.8   & ssl18    & 40  & 1      & 2      & 131    & 162   & \cellcolor[HTML]{9B9B9B}3 & \textbf{0.0}  & \textbf{-}                 & 0.4   \\
%   dll9                    & 38  & 2      & 1      & 91     & 100   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 2                          & 10.8  & ssl18\_1 & 40  & 2      & 2      & 118    & 160   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 30.9  \\
%   dll11                   & 36  & 1      & 3      & 68     & 87    & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 8.9   & ssl18\_2 & 49  & 1      & 3      & 85     & 160   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.3}  & 2                          & 54.9  \\
%   dll12                   & 36  & 1      & 3      & 63     & 77    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 7.3   & ssl19    & 40  & 1      & 2      & 141    & 169   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 29.1  \\
%   dll13                   & 36  & 2      & 3      & 51     & 60    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.0}  & \cellcolor[HTML]{C0C0C0}1  & 11.6  & ssl19\_1 & 50  & 2      & 3      & 106    & 175   & 7                         & \textbf{0.6}  & \cellcolor[HTML]{9B9B9B}1  & 28    \\
%   dll14\_1                & 37  & 1      & 3      & 71     & 85    & \cellcolor[HTML]{C0C0C0}1 & \textbf{0.1}  & \cellcolor[HTML]{C0C0C0}1  & 7.3   & ssl19\_2 & 44  & 1      & 3      & 81     & 174   & \cellcolor[HTML]{9B9B9B}8 & \textbf{0.3}  & \textbf{-}                 & 0.5   \\
%   dll15                   & 40  & 1      & 3      & 107    & 126   & \cellcolor[HTML]{9B9B9B}1 & \textbf{0.1}  & 3                          & 13.6  &          &     &        &        &        &       &                           & \textbf{}     &                            &       \\
%  \hline
%   \end{tabular}
%   \end{table*}


  % \begin{table}[]
  %   \centering
  %   \caption{Results for models violating predicates}
  %   \label{table:unsatres}
  %   \begin{tabular}{c|ccc|cc|cc}
  %   \hline
  %   model            & loc & sliced & total & flack & time & afl & at \\ \hline
  %   arr1             & 24  & 31     & 45    & 1     & 0.1  & 1   & 1.6  \\
  %   arr2             & 25  & 47     & 60    & 1     & 0.2  & 1   & 7.4  \\
  %   arr10            & 24  & 45     & 59    & 1     & 0.0  & 1   & 1.3  \\
  %   balancedBST1     & 51  & 155    & 171   & \cellcolor[HTML]{9B9B9B}1     & 0.2  & 5   & 43.6 \\
  %   balancedBST4\_1  & 52  & 147    & 163   & 1     & 0.1  & 1   & 94   \\
  %   balancedBST5     & 52  & 168    & 184   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 5   & 67.6 \\
  %   balancedBST7     & 52  & 143    & 159   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 4   & 49   \\
  %   balancedBST8\_2  & 54  & 140    & 156   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 4   & 40.4 \\
  %   balancedBST9     & 55  & 169    & 185   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 4   & 59.2 \\
  %   balancedBST10    & 47  & 140    & 157   & \cellcolor[HTML]{9B9B9B}1     & 0.6  & 2   & 91   \\
  %   balancedBST10\_2 & 52  & 156    & 172   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 5   & 50.3 \\
  %   balancedBST11\_1 & 60  & 198    & 214   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 8   & 77.2 \\
  %   balancedBST13    & 53  & 184    & 200   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 5   & 66.1 \\
  %   balancedBST14    & 59  & 186    & 202   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 4   & 63.3 \\
  %   balancedBST15    & 53  & 181    & 197   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 5   & 68.5 \\
  %   balancedBST17\_1 & 52  & 185    & 201   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 5   & 70   \\
  %   balancedBST18\_1 & 56  & 188    & 204   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 5   & 68.4 \\
  %   balancedBST20    & 52  & 153    & 169   & \cellcolor[HTML]{9B9B9B}1     & 0.1  & 4   & 54   \\
  %   balancedBST21    & 52  & 166    & 182   & \cellcolor[HTML]{9B9B9B}1     & 0.2  & 4   & 57.3 \\
  %   balancedBST22    & 50  & 158    & 213   & \cellcolor[HTML]{9B9B9B}1     & 0.6  & 3   & 51.8 \\
  %   dll7             & 38  & 79     & 90    & 1     & 0.1  & 1   & 7.4  \\
  %   dll10            & 40  & 85     & 91    & 1     & 0.2  & 1   & 6    \\
  %   dll14            & 39  & 91     & 102   & 1     & 0.1  & 1   & 7.4  \\
  %   dll17            & 37  & 83     & 89    & 1     & 0.1  & 1   & 6.8  \\
  %   fsm1             & 31  & 71     & 90    & 1     & 0.0  & 1   & 1.6  \\
  %   fsm3             & 60  & 56     & 67    & 1     & 0.7  & 1   & 2.7  \\
  %   fsm9             & 30  & 79     & 91    & 1     & 0.5  & 1   & 2.9  \\
  %   fsm9\_3          & 32  & 78     & 91    & 1     & 0.1  & 1   & 1.8  \\ \hline
  %   \end{tabular}
  %   \end{table}
\paragraph{Results}

Table~\ref{table:res1} shows {\tool}'s results.
For each model, we list the name, lines of code, the number of nodes that {\tool} determined irrelevant and sliced out, and the number of total AST expression nodes. The last two columns show {\tool}'s resulting ranking of the correct node and its total run time in second.
The 28 italicized \emph{models} contain predicate violations, while the other 124 models contain assertion violations.
{\tool} automatically determines the violation type and switches to the appropriate technique (e.g., using comparator for assertion errors and the unsat analyzer for predicate violations (Section~\ref{sec:approach}).
% Table~\ref{table:res} lists 123 bugs that violate assertions and Table~\ref{table:res} lists 28 bugs that violate predicates.
% Note that {\tool} automatically determines the bug type and switch to appropriate technique.
Finally, the models are listed in sorted order based on their ranking results.

% Columns \textbf{afl} and \textbf{at} show AlloyFL's resulting ranking and analysis time in seconds taken by AlloyFL, respectively.
%(recall that nodes refer to expressions and their subexpressions)
% The first two columns list the model names and lines of code in the model\footnote{The LoC counter tool \texttt{sloccount}~\cite{sloccount} does not work with Alloy models so we create our own (and is released together with {\tool}), which essentially performs the same calculation, e.g., only count real code and ignore comments and blank spaces/lines.}. %and the types of bugs (i.e., the cases shown in Figure~\ref{fig:4cases}).
%The next two columns \textbf{\# rel, \# val} list the number of different relations and atoms between the cex and sat instances.
%Column \textbf{sliced} lists the number of expressions irrelevant to the differences and thus are sliced out, and Column \textbf{total} lists the number of total AST nodes.
%Columns \textbf{flack} and \textbf{time} show


In summary, {\tool} was able to rank the buggy expressions in the top 1 (e.g., the buggy expression is ranked first) for 91 (60\%), top 2 to 5 for 35 (23\%), top 6 to 10 for 10 (34\%), above top 10 for 6 (4\%) out of 152 models.
%For 141/152 models, {\tool} was able to loacate the correct buggy expressions within the top 1.9\% (average) or the top 1 (median) for each of these models.
%{\tool} correctly ranked the buggy expression within the top 1 of the ranking lists for 90/152 models, the top 5 for 125 models, and top 10 for 135 models.
For 10 models, {\tool} was not able to identify the cause of the errors (e.g., the buggy expression are not in the ranking list), many of which are beyond the reach of {\tool} (e.g., the assertion error is not due to any existing expressions in the model, but rather because the model is ``missing'' some constraints).
Finally, regardless of whether {\tool} succeeds or fails, the tool produces the results almost instantaneously (under a second).


\paragraph{Analysis}
{\tool} was able to locate and rank the buggy expressions in 142/152 models.
% For 123 models in Table~\ref{table:res}, {\tool} applies \
% \textbf{Comparator} to locate bugs and for the rest 28 models in Table~\ref{table:unsatres}, {\tool} uses UNSAT analyzer.
Many of these bugs are common errors in which the developer did not consider certain corner cases.
For example, \texttt{stu5} contains the buggy expression \texttt{all n : This.header.*link | n.elem <= n.link.elem} that does not allow any node without link (the fix is changing to 
\texttt{all n : This.header.*link | some n.link => n.elem <= n.link.elem}).
{\tool} successfully recognizes the difference that the last node of the list contains a link to itself in the cex but not in the sat instance, and ranks this expression second; more importantly, it ranks first the subexpression \texttt{n.elem <= n.link.elem}, where the fix is actually needed.
%based on the generated satisfying instance by deleting UNSAT cores. 
% For several cases, the buggy expressions have the same ranking as other expressions. The main reason is that the generated differences between the cex's and sat instances were not able to help {\tool} differentiate between these expresions.
% Nonetheless, for these models, the buggy expressions are still ranked very high on the suspicious lists (2 ranked 1st, 1 ranked 3rd, and one 4th).
{\tool} also performed especially well on 28 models with violated predicates by analyzing the unsat cores and correctly ranked the buggy expressions first. 

For six models \texttt{bst4\_2}, \texttt{bst16}, \texttt{bst17}, \texttt{bst22\_3}, \texttt{stu9}, and \texttt{stu12\_1}, {\tool} was not able to place the buggy expression within the top 10 (but still within the top 16).
For these models, {\tool} obtains differences that are not directly related to the error, but consistently appear in both the cex and stat instances and therefore confuse {\tool}. %For example, the bugs in \texttt{bst4\_2}, \texttt{bst16}, and \texttt{bst22\_3} are caused by the expression \texttt{a - b} which should be \texttt{minus[a,b]}, however {\tool} obtains differences in left and right structure of the tree thus locates other expressions on top of the list.


{\tool} was not able to identify the correct buggy expressions in 10 models, e.g., the resulting ranking list does not contain the buggy expressions.
Most of these bugs are beyond the scope of {\tool} (and fault localization techniques in general).
More specifically, the 9 models \texttt{bst4}, \texttt{bst11}, \texttt{bempl}, \texttt{ctree}, \texttt{dll3\_2}, \texttt{ssl16}, \texttt{ssl16\_1}, \texttt{ssl16\_2}, and \texttt{ssl16\_3} have assertion violations due to \emph{missing} constraints in predicates and thus do not contain buggy expressions to be localized.
% {\tool} always assign a suspicious score 0 for an empty predicate, thus other expressions related to the difference always get higher score and rank first.
% For example, the error in \texttt{bst4 and bst11} is an empty predicate \texttt{pred HasAtMostOneChild(n: Node) \{\}} where the fix is adding expression \texttt{no n.left || no n.right} to the body of the expression. {\tool} is able to capture the difference is caused by \texttt{no left or no right} and ranks first a fact expression \texttt{no n.left \& n.right}.
For \texttt{other}, {\tool} did not find the "ground truth" buggy expression (the buggy expression does not contain the different relation) but ranked first another expression that could also be modified to fix the error.


% For the 3 models \texttt{other1, stu2\_2, stu12\_2}, {\tool} fail to identify the buggy expression in its ranking list.
% In \texttt{stu2\_2}, the difference between the cex's and sat instances does not lead to the correct buggy expression.

% For \texttt{stu12\_2}, {\tool} did not find the buggy expession, but ranked a subexpression of the buggy expression fourth.

% For the 2 models \texttt{arr1} and \texttt{dll3\_1}, the error is trivial false and the Alloy Analyzer returns no cex's and thus there is no assertion violation for {\tool} to check.
% This can happen when the model contains conflicting constraints, e.g., they evaluate to \texttt{false} and thus there are no instances at all.
% For example, for the model \texttt{arr1}, we couldnot generate any cex's (or sat instances) because the model itself is \texttt{false} (it contains the false expression \texttt{all i:Int |i>=0 and i<Array.length}).


%For \texttt{grade1, stu6\_2, stu14\_2, stu17\_2}, {\tool} is able to locate to the predicate the needs to repair all at the top 2 location\tvn{Not clear, then why this has a - in the ranking ?}.\gz{the expression that need to fix is not in the ranking list, but its subexpression is presented. For example, if the fix is change \texttt{all n : Node | some n} to \texttt{no header or (all n:Node | some n)}. We output \texttt{some n}, but not \texttt{all n: Node | some n}}.

%is an integer input to the predicate called in the assertion and {\tool} couldn't capture this information\tvn{what does this mean ?  it doesn't capture integer input?}. \gz{That integer is in the Int relation, the Int relation in Alloy contains same integers, so there is no difference between cex and sat. This integer is just selected as an input to a predicate, no difference exists between Int relation in cex and sat, thus we can't capture this information.}

%% 2/56 models contains bugs that {\tool} doesn't support.  falls into (a) and (b) cases shown in Figure~\ref{fig:cexexp} recepectively. 
%%  \texttt{dll3\_1} is a case (b) model which generates no couterexample when running the assertion and is able to generate the sat instance, thus {\tool} assumes the model is correct. 


%\texttt{dll3\_3, stu16} use empty predicate in assertion which doesn't provide any useful information.


%% For 2 out of these 43 models, \texttt{stu9} and \texttt{stu18\_3}, we were not able to place the buggy expression within the top 5 (but still within the top 10) due to several reasons. Both have a similar kind of assertion, which contains a predicate call that not related to the error, and the difference between cex and sat instance are caused by the violation of this preciate and leads {\tool} locates to other expressions.

%The main reason happens is due to the counterexample and expected instance are not most similar. With manually selected couterexample and expected instance to ensure the difference are minimum, {\tool} is able to locate to correct buggy location. One possible solution is to generate more expected instances and select the most similar one as counterexample. \tvn{I don't understand. So why does this give problem to your alg?}


%% For the other 8/56 models (where the rank is listed as -), (\texttt{bempl1, ctree, dll3\_3, grade1, stu6\_2, stu14\_2, stu16, stu17\_2})we were \emph{not} able to identify the correct expression simply because the ``bug'' is due to missing constraints and is not caused by any expression in the model. \texttt{bempl1, ctree} is missing constraints in \texttt{fact}, thus any location will be a possible location to fix the problem. \texttt{dll3\_3, stu16} use empty predicate in assertion which doesn't provide any useful information. For \texttt{grade1, stu6\_2, stu14\_2, stu17\_2}, {\tool} is able to locate to the predicate the needs to repair all at the top 2 location.



%\tvn{Give some interesting examples that perform well here first. Then talk about those that do not perform well. The whole writing right now are very negative.  It completely talks about failures and not successes.}

%\tvn{For example. You can say several of these.  For program X that has some interesting bug Y,  {\tool} was able to localize the fault to the expression Z, which clearly shows the error.}

%\tvn{Some of these have ranking 2,3 ... talk about them.  Some of these have ranking 23,  specifically talk about them.}

%For 14 out of 48 examples (\tvn{How many, state the number, e.g., X/Y}) {\tool} are not performing well due to the following reasons. 

%The bug in \texttt{bst1} generate the same expected instance with only a single root node for all counterexamples generated. As all the expected instances are the same, we couldn't collect enough information from the expected instance.  One possible way to fix this problem is to manually write the expected predication, for example adding more constraint like \code{some left and some right} to force Alloy generate instance more than a single root node. \tvn{Give some hypothesis on what you can do (in future work) to address this. For example, it might be possible to do X ..}

%The bug of bst2\_bug3 and bst3\_bug2 locates involves Alloy self-defined functions: mul, minus and signum which are not supported by current implementation and fail to locate that bug. \tvn{Why not? what's tricky about these?  }\gz{todo: need to think how to explain this.}

%The counter examples generated in stu2\_bug2, stu9, stu12\_bug2 stu18\_bug3 and stu19\_bug2 are the same as the expected instances respectively. This is due to the difference is that in the counter example one of skolimized variable has a value false while in the expected instance it contains no skolim vairables, thus this difference is not captured by the tool.
%\tvn{rewrite this, ppl will not be able to understand what Skolem variables mean.}\gz{don't know how to replace this terms, will think about it}
%With human provided expected instances, this examples are able to achieve a better ranking.\tvn{give a concrete example}

%\tvn{I think it's better to put these bugs in a category of its own. May be put them at the end of the table and not interleaving with others}\gz{added a new table and described in 2nd paragraph}
%There are also some missing constraint bugs that the repair needs to add new constraints other than modifying existing constraints, as shown in Table ~\ref{table:missingres}. For these examples, we report the rank as 0 and exclude them from calculating the averages, as any located location would be wrong. For example, bempl1, ctree, dll3\_bug3, grade1, stu6\_bug2, stu14\_bug2 and stu17\_bug2.


%\gz{add new paragraph talking about difference between AlloyFL and \tool}

\subsection{RQ2: Real-world Case Studies}
\label{sec:casestudies}
The AlloyFL benchmark contains a wide variety of Alloy models and bugs, but they are relatively small ($\approx$50 LoC).
To investigate the scalability of {\tool}, we consider additional case studies on larger and more complex Alloy models.


\begin{table}
\vspace{0.2cm}
  \caption{{\tool}'s results on large complex models}
  \label{tab:realworld}
  \centering
  \begin{tabular}{lr|rrrr}
    \textbf{model}           &  \textbf{loc}           & \# \textbf{slice}   & \textbf{total} &  \textbf{rank}   & \textbf{time(s)}\\
    \midrule
    surgical robots &  200             &     278     & 293  & 2  & 2.3   \\
    % FiveDOFSolver   &  197             &  278     & 293  & 2  & 2.3   \\
    % FourDOF\_needle &  197             &  278     & 293  & 2 & 2.4    \\
    % FrankenVREP     &  197             &  278     & 293  & 2 &2.5     \\
    % SevenDOFSolver  &  197             &  278     & 293  & 2 &2.6     \\
    % TomBot          &  197             &  278     & 293  & 2 &2.7     \\
    \midrule
    android permissions        &  297         & 673 &  1138  & 2    & 5.2 \\
    \midrule
      % sll-contains-3  &  2634          &  3344      & 3396 &  3    \\
      % sll-contains-6  &  3942          &  4427      & 4479 &  3    \\
    sll-contains    &  5250             &  5510      & 5562 &  3  &3.0  \\
    count-nodes     &  3791           &  2861      & 5064 & 18  &188.7  \\
    remove-nth      &  5063           &  3306      & 6336 & 12 &1265.0   \\    
    \bottomrule
  \end{tabular}
\end{table}

% \begin{table}
%   \caption{{\tool}'s results on large complex models}
%   \label{table:robots}
%   \centering
%   \begin{tabular}{lr|rrrc}
%     \toprule
%     model           &  loc           & \# slice   & total &  rank   & time\\
%     \midrule
%     FiveDOFSolver   &  197             &  278     & 293  & 2  & 2.3   \\
%     FourDOF\_needle &  197             &  278     & 293  & 2 & 2.4    \\
%     FrankenVREP     &  197             &  278     & 293  & 2 &2.5    \\
%     SevenDOFSolver  &  197             &  278     & 293  & 2 &2.6    \\
%     TomBot          &  197             &  278     & 293  & 2 &2.7    \\
%     \midrule
%       % sll-contains-3  &  2634          &  3344      & 3396 &  3    \\
%       % sll-contains-6  &  3942          &  4427      & 4479 &  3    \\
%     sll-contains    &  5250             &  5510      & 5562 &  3  &3.0  \\
%     remove-nth      &  5063           &  3306      & 6336 & 12 &1265.0   \\
%     count-nodes     &  3791           &  2861      & 5064 & 18  &188.7  \\
%     \midrule
%     android         &  297         & 673 &  1138  & 2    & 5.2 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\paragraph{Surgical Robots} The study in~\cite{robots} uses Alloy to model highly-configurable surgical robots to verify a critical \emph{arm movement safety} property:
%as the surgeon moves the control device during the surgery procedure,
the position of the robot arm is in the same position that the surgeon articulates in the control workspace during the surgery procedure and the surgeon is notified if the arm is pushed outside of its physical range.
This property is formulated as an assertion and checked on 15 Alloy models representing 15 types of robot arms using different combinations of hardware and software features.
The study found that 5 models violate the property.

Table~\ref{tab:realworld}, which has the same format as Table~\ref{table:res1}, lists the results.
We use all 5 buggy models (each has about 200 LoC) but list them under one row because they are largely similar and share many common facts and predicates but with different configurable values (one model has a fact that has an AngleLmit set to 3 while another has value 6). The buggy expression is also similar and appears in the same fact.  
For each model, {\tool} ranked the correct buggy expressions in the second place in less than 3 seconds. {\tool} returned two suspicious expressions (1) \texttt{HapticsDisabled in UsedGeomagicTouch.force} and (2) \texttt{some notification : GeomagicTouch.force |  notification = HapticsEnabled}.
Modifying either expression would fix the issue, e.g., changing \texttt{Disable} to \texttt{Enabled} in (1) or \texttt{Enabled} to \texttt{Disabled} in (2).


\paragraph{Android Permissions}
The COVERT project~\cite{covert} uses compositional analysis to model the permissions of Android OS and apps to find inter-app communication vulnerabilities.
The generated Alloy model used in this work does not contain bugs violating assertions, thus we used the MuAlloy mutation tool~\cite{mualloy} to introduce 5 (random) bugs to various predicates in the model: 3 binary operator mutations, 1 unary operator mutation, and 1 variable declaration mutation.

Table~\ref{tab:realworld} shows the result.
{\tool} was able to locate 4 buggy expressions (the unary modification ranked 2nd, the binary operations ranked 3rd, 9th, and 11th), but could not identify the other mutated expression (the variable declaration mutation). However, after manual analysis, we realize that this mutated expression does not contribute to the assertion violation (i.e., {\tool} is \emph{correct} in not identifying it as a fault). 
%After fixing the 4 bugs found in the model, we find that the 5th mutation doesn't violate the assertion.




\paragraph{TACO}
The TACO (Translation of Annotated COde) project~\cite{tacoconf} uses Alloy to verify Java programs with specifications.
TACO automatically converts a Java program annotated with invariants to an Alloy model with an assertion.
If the Java program contains a bug that violates the annotated invariant, then checking the assertion in the Alloy model would provide a counterexample.
We use three different  Alloy models with violated assertions representing three real Java programs from TACO~\cite{tacoconf}:
\texttt{sll-contains} checks that a linked list containing a certain element;
\texttt{count-nodes} counts the number of a list's nodes; and \texttt{remove-nth} removes the nth element of a list.
These (machine-generated) models are much larger than typical Alloy models ($\approx$5000 to 6000 LoC each).
%We use TACO to translate these programs to Alloy models with assertions. The original Java program has a bug that violates this assertion and hence the corresponding Alloy model fails the asserted property. %The different types bugs are translated to different types of bugs that violate the Alloy assertions. 

Table~\ref{tab:realworld} shows the results.
For \texttt{ssl-contains}, {\tool} ranked the buggy expression third within 3 seconds.
This expression helps us locate an error in the original Java program that skips the list header.
% Moreover, the buggy expression found by {\tool} directly leads us to identify the bug in the original Java program
% Briefly, the \texttt{sll-contains} model contains 1 bug and {\tool} locates the buggy expression at 3th in the ranking list in 3.0 seconds, with 1.7 seconds to generate instances and 1.3 seconds to locates.
The faulty expressions of \texttt{remove-nth} and \texttt{count-nodes} are ranked 12th and 18th, respectively (which are still quite reasonable given the large, $>5000$, number of possible locations).
%This inaccuracy and the long run time are because 
Note that 
these buggy expressions consist of multiple errors (e.g., having 5 buggy nodes), causing {\tool} to instantiate and analyze combinations of a large number of subexpressions.

%{\tool} did not produce accurate results for the other two models (the buggy expressions are still ranked in the top 20 out of 5000+ candidates): 
%The multiple faulty expressions in complex models forced {\tool} to instantiate and analyze a large number of expression combinations to identify the suspicious expressions.
Manual analysis on the identified buggy expressions showed that the original Java programs consist of (single) bugs within loops. TACO performs loop unrolling and thus spreads it into multiple bugs in the corresponding Alloy models.

%The other two models take much longer to analyze because 

% and a more accurate location for the minimal buggy expression contains 1 bug appears at 67th in the ranking list. The analyze time is 1265 seconds, with 4 seconds to generate instances and 1261 seconds to evaluate and analyze more than 2.5 million instantiated expressions generated from the large number of expressions. 

%  and a more accurate location for the minimal buggy expression contains 1 bug appears at 36th in the ranking list. The analyze time is 189 seconds, with 2 seconds to generate instances and 187 seconds to evaluate and analyze 400 thousands instantiated expressions.


In summary, we found that {\tool} works well on large real-world Alloy models.
While coming up with correct fixes for these models remain nontrivial, {\tool} can help the developers (or automatic program repair tools) quickly locate buggy expressions, which in turn helps understand (and hopefully repair) the actual errors in original models.






% The \texttt{adnroid} model is collected fro COVERT~\cite{}, an Alloy model describing Android permissions. The original model doesn't contain any bugs that violates the assertion, and we randomly introduce 5 bugs to the model using a mutation tool. 


% %Table~\ref{table:robots}, which has the same format as Table~\ref{table:res}, shows the results (the first 5 rows) of applying {\tool} on these 5 models and the safety property.
% %These models are largely similar; they share many common facts and predicates, but use different values in definitions (e.g., \texttt{fourDofNeedle} has a fact that sets an AngleLimit to 3, while \texttt{fiveDofSolver} uses value 6).




% We then ran {\tool} on these Alloy models to identify the buggy expressions and understand the error in the original Java programs.
% Table~\ref{table:robots} shows the results (the last 5 rows).
% These three Alloy models are generated by TACO and contain around 5000 LoC.

\subsection{RQ3: Comparing to AlloyFL}
% As mentioned, the AlloyFL tool [48], which is also part of the ARe-
%  pair tool, also identifies buggy expressions in Alloy models. How-
%  ever, there are several main differences between AlloyFl and BFA’s
%  assumptions and techniques. BFA relies on assertions to indicate
%  errors while AlloyFL uses tests, expressed as predicates generated
%  from the AUnit test framework [45], to indicate errors. Moreover,
%  BFA relies on comparing and extracting differences from coun-
%  terexamples and satisfying instances, while BFA adopts existing
%  debugging techniques often used in imperative programs such as
%  mutation testing and spectrum-based fault localization. Thus, the
%  two tools, while serving a similar purpose, have different input
%  requirements and techniques to localize faults.
%  We have also attempted to directly compare BFA and AlloyFL,
%  but were not able to do it completely. The main reason is that
%  AlloyFL and its dataset, e.g., the tests used to indicate errors, are
%  not available (the paper [48] is being submitted and reviewed). Thus,
%  we were not able to reproduce AlloyFL’s results as described in [48].
%  However, we were able to find an unofficial AlloyFL version
%  within the ARepair tool, and were able to use the provided AUnit
%  tests to run AlloyFL on these ARepair models. For most of these
%  models, both AlloyFL and BFA performed similarly, e.g., consis-
%  tently ranked the correct buggy expressions at the top. For example,
%  for addr1, both AlloyFL and BFA were able to rank the buggy node
%  first, though AlloyFL used 62 test cases and ran in 2.5 seconds while
%  BFA used one assertion and finished in 0.8 seconds. For some mod-
%  els, BFA performed better, e.g., for balancedBST1, AlloyFL took 52
%  seconds and ranked the buggy expression fifth while BFA runs un-
%  der a second and rank the same expression third. For some models,
%  AlloyFL performed better, e.g., for stu9, AlloyFL used 58 seconds
%  but ranked the buggy expression first, while BFA took 1 second but

% ranked that same expression 11th. For some models, e.g., the models 987 bempl,stu16 with missing constraints, both tools fail because the 988 models do not contain any buggy expressions. 989
% For the larger Alloy models used in our case studies in Section 4.2, 990 we were not able to run AlloyFL as it crashed immediately when 991 reading these models and their Aunit tests (we have reported the 992 issue to the main author of AlloyFL). 993
% In general, while BFA appears to be faster, it is still difficult to 994 directly compare these tools as the inputs to the tools are different 995 and they use different approaches that produce complimentary 996 results (sometimes one tool is better than the other).


We compare {\tool} with AlloyFL~\cite{alloyfl}, which to the best of our knowledge, is the only Alloy fault localization technique currently available.
While both tools compute suspicious statements, they are very different in both assumptions and technical approaches.
As discussed in Section~\ref{sec:related}, AlloyFL requires \emph{AUnit tests}~\cite{aunit}, provided by the user or generated from the correct model, and adopts existing fault localization techniques in imperative programs, such as mutation testing and spectrum-based fault localization; in contrast, {\tool} uses violated assertions and relies on counterexamples.
% expressed as predicates generated
% % from the AUnit test framework [45]

To apply AlloyFL on the 152 benchmark models, we use the best performance configuration and testsuites described in~\cite{alloyfl}. Specifically, we use the AlloyFl$_{hybrid}$ algorithm with Ochiai formula and reuse tests in~\cite{alloyfl} (automatically generated by MuAlloy~\cite{mualloy} as described in~\cite{alloyfl}).

Table~\ref{table:compare} compares the results of {\tool} and AlloyFL.
The two approaches appear to perform similarly, with {\tool} being slightly more accurate. 
Overall, {\tool} outperforms AlloyFL, where on average the  buggy expressions ranked 2nd and 3rd by {\tool} and AlloyFL, respectively. Also, in top 1 ranking {\tool} performs much better compared to AlloyFL (91 over 76 models). %and on average (the correct buggy expressions ranked 2nd and 3rd by {\tool} and AlloyFL, respectively), but {\tool} is slightly accurate in the top 5 (128 over 126 models).
Moreover, {\tool} is much faster, where the average analysis time is far less than a second for {\tool}, it takes over 30 seconds for AlloyFL to analyze the same specifications.

We were not able to apply AlloyFL to the models in Section~\ref{sec:casestudies} because MuAlloy~\cite{mualloy}, which is used to generate AUnit tests for AlloyFL, does not work with these models (e.g., mostly caused by unhandled Alloy operators). %that would require extending MuAlloy).
This is not a weakness of AlloyFL, but it suggests that it is not trivial to generate tests from existing Alloy models automatically.

%In summary, while {\tool} runs much faster, it is difficult to directly compare the two tools they have different assumptions (tests versus assertions), employ different techniques, and produce complimentary results (for some models {\tool} is better but for other models AlloyFL is better).



% To obtain AlloyFL results, we use the test suites used in AlloyFL paper (most are automatically generated from correct models but some are manually generated as described in~\cite{alloyfl}) and choose the best performance configuration as described in~\cite{alloyfl} (e.g., using the AlloyFL$_{hy}$ algorithm with the Ochiai formula, 100\% tests and 0.4 weight). In Table~\ref{table:res} and Table~\ref{table:unsatres}, we highlight with light gray the 35 models that both tools rank the buggy expression at top 1, and dark gray the models that one tool outpus a better result. For 60 models, 44 models in Table~\ref{table:res} and 16 models in Table~\ref{table:unsatres}, {\tool} ranks higher than AlloyFL. For 40 models, all in Table~\ref{table:res}, AlloyFL ranks higher than {\tool}.   

% Table~\ref{table:compare} shows the summary of {\tool} and AlloyFL on the 152 models collected from AlloyFL. Overall, {\tool} and AlloyFL has a similar performance with a 2.4 and 3.1 average ranking. {\tool} has a higher number of top1 performance, while AlloyFL can find 3 more models where {\tool} couldn't. This is because AlloyFL could locates to the body for empty predicates like in \texttt{ssl16, ssl16\_1, ssl16\_2 and ssl16\_3}.

\begin{table}
  \centering
  \vspace{0.2cm}
  \caption{Comparision with AlloyFL.}
  \label{table:compare}
  \begin{tabular}{c | c c c c c | c c}
    \toprule
    &\multicolumn{4}{c}{\textbf{top}}&&\multicolumn{2}{c}{\textbf{avg}}\\
    \textbf{tool} & 1& 5 & 10 & $>$ 10 & \textbf{failed} & \textbf{rank}& \textbf{time(s)} \\
    \midrule
    {\tool}&91&126&136&6&10&2.4&0.2\\
    AlloyFL&76&128&137&8&7&3.1&32.4\\
    \bottomrule
  \end{tabular}
\end{table}

% \begin{table}
%   \centering
%   \caption{Comparision with AlloyFL}
%   \label{table:compare}
%   \begin{tabular}{c | c c}
%     \toprule
%     metrics & {\tool} & AlloyFL \\
%     \midrule
%     top1 & 91      & 75 \\
%     top5 & 125     & 127 \\
%     top10 & 135    & 136 \\
%   $>$ 10 & 6       & 8   \\
%     -    & 10      & 7   \\
%     \midrule
%     rank & 2.4     & 3.1 \\
%     time(s) & 0.2     & 32.4 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

%{\tool} has a much lower time overhead (0.2 seconds in average) than AlloyFL (32.4 seconds in average). AlloyFL calls the solver based on the number of mutations and test cases, while {\tool} only calls the solver 10 times for localization, 5 times for generating cex and 5 times for generating sat. 
% As mentioned, the AlloyFL tool~\cite{alloyfl}, which is also part of the ARepair tool, also identifies buggy expressions in Alloy models.
% However, there are several main differences between AlloyFl and {\tool}'s assumptions and techniques.
% {\tool} relies on assertions to indicate errors while AlloyFL uses tests, expressed as predicates generated from the AUnit test framework~\cite{aunit}, to indicate errors.
% Moreover, {\tool} relies on comparing and extracting differences from counterexamples and satisfying instances, while {\tool} adopts existing debugging techniques often used in imperative programs such as mutation testing and spectrum-based fault localization.
% Thus, the two tools, while serving a similar purpose, have different input requirements and techniques to localize faults.


% We have also attempted to directly compare {\tool} and AlloyFL, but were not able to do it completely.
% The main reason is that AlloyFL and its dataset, e.g., the tests used to indicate errors, are not available (the paper~\cite{alloyfl} is being submitted and reviewed).
% Thus, we were not able to reproduce AlloyFL's results as described in~\cite{alloyfl}.

% However, we were able to find an unofficial AlloyFL version within the ARepair tool, and were able to use the provided AUnit tests to run AlloyFL on these ARepair models.
% For most of these models, both AlloyFL and {\tool} performed similarly, e.g., consistently ranked the correct buggy expressions at the top.
% For example, for \texttt{addr1}, both AlloyFL and {\tool} were able to rank the buggy node first, though AlloyFL used 62 test cases and ran in 2.5 seconds while {\tool} used one assertion and finished in 0.8 seconds.
% For some models, {\tool} performed better, e.g., for \texttt{bst1}, AlloyFL took 52 seconds and ranked the buggy expression fifth while {\tool} runs under a second and rank the same expression third.
% For some models, AlloyFL performed better, e.g., for \texttt{stu9}, AlloyFL used 58 seconds but ranked the buggy expression first, while {\tool} took 1 second but ranked that same expression 11th.
% For some models, e.g., the models \texttt{bempl,stu16} with missing constraints, both tools fail because the models do not contain any buggy expressions.

% For the larger Alloy models used in our case studies in Section~\ref{sec:casestudies}, we were not able to run AlloyFL as it crashed immediately when reading these models and their Aunit tests (we have reported the issue to the main author of AlloyFL).

% In general, while {\tool} appears to be faster, it is still difficult to directly compare these tools as the inputs to the tools are different and they use different approaches that produce complimentary results (sometimes one tool is better than the other).



%% For each benchmark model in the ARepair benchmark, we create 5 AUnit tests and run AlloyFL
%% For this benchmark, both yield similar results: they both correctly rank suspicious statements within the top {\tvn ??} percent, do not work on the same programs (\tvn{Vu: mentioned which in Table}), and both yield results within seconds (AlloyFL runs within 5 secs while {\tool} runs in 1 second).






%% bst1 allfl locates to 5 using 52 seconds 
%%              bfa  locates to 3 using 1 sec
%% stu9: alloyfl locates to 1 using 58 seconds
%% 	  bfa     locates to 11 using 1 seconds 
%% bempl, stu16: both couldn't work






%\paragraph{Comparing to AlloyFL} Although we evaluate {\tool} using the same benchmark as AlloyFL ~\cite{arepair}, {\tool} applies different techniques and use the benchmark differently. AlloyFL uses on test suites getting from correct version of Alloy specification and mutation to locate bug, while {\tool} directly works on the buggy version and uses inserted assertion or assertion coming with specification to locate bug. 





%% First, we note that the tool AlloyFL and its data are not publicly available so we can only use the the version that came with ARepair, which is slightly modified for automatic program repair purpose.

%% \tvn{NOT DONE, waiting for results}

%% We also ran AlloyFL on the Alloy models used in the real-world studies descsribed in Section~\ref{}.
%% For these models, we manually create AUnit tests to give to AlloyFL.
%% However, AlloyFL fails to run on any of these models (it just crashes).



\subsection{Threats to Validity}
%There exist several threats to the validity of our results.
We assume no fault in data type (sig's) and field declarations, which may limit the usage of {\tool}.
However, none of the benchmark models we used has bugs at these locations.
Moreover, we could always translate constraints for sig and field to facts. For example, \texttt{one sig A} could be translated to \texttt{sig A; fact\{one A\}}.

The models in the AlloyFL benchmark are collected from graduate student's homework and relatively small.
Thus, they may not represent faulty Alloy models in the real world.
However, we also evaluate {\tool} with large Alloy models, written by experienced Alloy developer (the surgical robot models and Android permissions model) or generated by an automatic tool (TACO) and 
show that {\tool} performs well on these models (Section~\ref{sec:casestudies}).

We manually create assertions for models that do not have assertions. Thus, our assertions might be inaccurate and not as intended.
However, for other models with assertions (e.g., those in the AlloyFL benchmark and all the case studies), we use those assertions directly and {\tool} output similar results.

%Some the overconstraint bugs may not be captured by assertions. For this situation, {\tool} could try to use the cex and sat instance provided by user to locate the error.

%The real faulty models we use in the experiment are limited in the sense that most of them are written by graduate students.So the experiment results may not generalize to faulty models written by experienced developers.
% However, we collect our subject faulty models to the best of our ability.
% The AUnit tests (e.g., the test in Figure 1b) can require some manual effort to create.
% In this paper, all tests are automatically generated using MuAlloy [61] and the expected behavior (expect 0 or 1) of each test is automatically verified using the correct model.
% In practice, users need to manually specify the expected behavior but no manually effort is needed to write test predicates.
% We choose to use automatically generated test predicates to evaluate AlloyFL because we did not find real faulty models with enough tests.
% So our result may not generalize to manually written tests.
% Additionally, although our distance metrics simulate different ways users may inspect code highlighted by AlloyFL, our result may not generalize to new metrics.


==> pldi21/introduction.tex <==
\section{Introduction}
%Hamid: Alloy is not used much for model-driven development.
%Software is everywhere in our daily lives and provides variety of services. The complexity and size of the software increases as the growing requirement for more and more sophisticated functionality. 
%One promising technique for robust software development is model-driven engineering~\cite{modeldriven}, where model is used in the early stage of development. A modelling language is used to create and validate models in the design process to discover errors as early as possible. Most notably, Alloy~\cite{alloy} has received a lot of attention due to its expressiveness and simplicity.  

Declarative specification languages and the corresponding formally precise analysis engines have long been utilized to solve various software engineering problems. Most notably, the Alloy specification language~\cite{alloy}, that relies on first-order relational logic,
%Alloy is a declarative language for modelling the structure and behavior of complex hardware and software systems~\cite{alloy}.
%It 
has been used in a wide range of applications, such as program verification~\cite{tacoconf}, test case generation~\cite{testcase,ICSE2016}, network  security~\cite{network1,network2,network3}, security analysis of emerging platforms, such as IoT~\cite{iot_issta} and Android~\cite{android,android2}, and design tradeoff analysis~\cite{trademaker_ICSE,trademaker_TSE_2017}, to name a few. Cunha and Macedo, among others, use a recent extension of Alloy, called Electrum~\cite{DBLP:conf/kbse/BrunelCCM18}, to validate the European Rail Traffic Management System, a system of standards for management and inter-operation of signaling for the European railways~\cite{alloyuse3}. Kim~\cite{alloyuse7} proposes a  Secure Swarm Toolkit (SST), a platform for building an authorization service infrastructure for IoT systems, and uses Alloy to show that SST provides necessary security guarantees. 
 
% \gz{rewrite}
% Software has embedded itself in our daily lives, and is now essential for communication, healthcare, transportation, and even homecomfort. Yet at the same time, software continues to fail, and ma-licious users exploit weaknesses of systems [1]. Fifteen years ago the National Institutes of Standards reported that a poor softwarequality infrastructure was costing the US upwards of \$59 Billionannually [2], and an equally ominous report from Tricentis in 2017estimated the annual financial loss due to software failures world-wide at \$1.7 Trillion [3]. While many efforts have been made toimprove our software engineering techniques, and to develop bettersoftware validation methods, these problems still persist. Recenthighly publicized bugs like the Toyota acceleration problem andthe heartbleed bug as well as the explosion of Android exploits [4]show that we still lack sufficient techniques to verify and validateour software

% One class of techniques that have been used to tackle dependability are those which fall into the category of formal methods,with their strength residing in the mathematical concepts leveragedto prove the correctness of dependability properties. Most notably, Alloy, a lightweight formal verifier, such as those based on bounded veri-fication, have recently received a lot of attention due to their auto-mated, yet formally precise analysis capabilities, which reduce theburden on traditional formal verification techniques. This spans awide range of software engineering and security domains, includingsoftware design [5,6], code analysis [7], security analysis [4], testcase generation [8] and tradeoff synthesis and analysis [9,10]. \gz{end}

% Recent work: ~\cite{alloyuse1} apply   and   assessUseCase  Modeling  for  System-level,  Acceptance  Tests  Generation(UMTG), an approach that generates executable system testcases for acceptance testing by exploiting behavioral infor-mation in use case specifications and use Alloy to generate test input data for object constraint language constraints generated using NLP technique.
% ~\cite{alloyuse2} implements  transitive-closure-based model checking using Alloy.

% ~\cite{alloyuse4} presents a self-adaptation techniques, building on top of Alloy, to reduce the number of possible adaptations that need be considered for each run-time adaptation decision 
% ~\cite{alloyuse5} use Alloy to model and reason about thestructure and behavior of sparse matrices
% ~\cite{alloyuse6} extends Alloy to help simplifying the development of a full software product line(SPL) with many variants supporting different features


%Given a system specification written in the Alloy language, a developer can write an assertion or a predicate to check if the specification violates or satisfies some property. Alloy then translates the system specification along with the property specification to a SAT formula, and uses an off-the-shelf SAT solver to find a solution that violates the assertion or satisfies the predicate.  


%Similar to writing programs in an imperative language, such as C or Java, developers can make subtle mistakes when writing Alloy specifications, especially those that capture complex systems with non-trivial behaviors.
%Moreover, the user might not be familiar with the Alloy language's syntax and semantics and can make subtle mistakes, hard to detect by a novice developer.
Similar to developing programs in an imperative language, such as C or Java, developers can make subtle mistakes when using Alloy in modeling system specifications, especially those that capture complex systems with non-trivial behaviors, rendering debugging thereof even more arduous. 
%Moreover, developers can make subtle mistakes, rendering the debugging even more arduous.
These challenges call for debugging assistant mechanisms, such as fault localization techniques, that support declarative specification languages.
%Hence, debugging assistance mechanisms, such as fault localization techniques, can help the users write correct Alloy code and thus help increase the uses and adoption of Alloy and formal methods in general.


%Comparing to imperative languages, there are far less fault localization techniques developed for declarative languages. 
However, there is a dearth of fault localization techniques developed for Alloy. 
AlloyFL~\cite{alloyfl} is perhaps the only fault localization tool available for Alloy as of today.
The key idea of AlloyFL is to use ``unit tests," where a test is a predicate that describes an Alloy instance to encode expected behaviors, to compute suspicious expressions in an Alloy model that fails these tests.
To compute the suspicious expressions, AlloyFL uses mutation testing~\cite{mut1,mut2} and statistical debugging techniques~\cite{spfl1,spfl2,spfl3}, i.e., it mutates expressions, collects statistics on how each mutation affects the tests, then uses this information to assign suspicious scores to expressions.

%The submission presents an automated approach to repair faults in Alloy models. Faults in Alloy models are identified using AUnit tests [66]: a "unit test" framework for Alloy, where a test is a predicate that describes an Alloy instance.

%My problem with the failing AUnit tests is that it seems to me more difficult to create a correct AUnit test than to just repair the Alloy model it refers to. This is a serious threat to the applicability of the entire approach.

%I am bothered with the paper's implicit assumption of the availability of AUnit tests (because I believe that it is more difficult to manually create a correct AUnit test than to manually fix the bug). This is not the common case as in Java where failing tests are indeed available - without them, no one starts fault localization and repair - a bug does not exist if there is no test that demonstrates it. I don't think the challenge of writing AUnit tests is similar to the challenge of writing tests in other languages like Java. It is much more difficult and error prone; very difficult to know that the test itself is correct.

%% AlloyFL takes in a set of predicates as 'tests' for Alloy and outputs an ordered list of AST nodes based on their suspicious level. These predicates are labeled as should satisfy or not, as the passing test case or failing ones. .
  
%Not many work has focus on fault localization for Alloy. AlloyFL ~\cite{alloyfl}  is the first paper addressing the debugging problem for Alloy. 

While AlloyFL pioneered fault localization in the Alloy context and the obtained results thereof are promising, it relies on the assumption of the availability of AUnit tests~\cite{aunit}, which is not common in the Alloy setting. Indeed, instead of writing test cases, Alloy users write assertions to describe the desired property and let the Alloy Analyzer search for potential counterexamples (cex's) that violate the property.
%There are existing test generation works for Alloy (e.g., AlloyFL uses the AUnit framework to automatically generate tests from given correct models), however, 
Moreover, it is unclear how many test cases are needed or how good they must be for AlloyFL to be effective (e.g., in the AlloyFL evaluation~\cite{alloyfl}, the number of tests ranges from 30 to 120).
%Moreover, instead of writing tests describing a specific instance that should or should not be satisfied a property, Alloy users often write assertions or predicates to describe the desired property and let the Alloy Analyzer searches for specific instances that satisfies or violates the property.


%% that can help automatically generate such tests, 

%% It is tedious for developers to manually write these predicates, which is similar to creating ``corner case'' tests for imperative programs.
%% AlloyFL also presents AUnit ~\cite{aunit} to automatically generates these tests. However, AUnit generates tests based on the correct model, which is useful in many scenarios like homework grading or model rewriting. But this limits the usage of AlloyFL when the model is too complicated that developer is not able to write numbers of predicates or when there is no correct models. Another limitation is that to rather than writing tests as a specific instance, Alloy developers usually use assertion or predicate, which represents a set of instances shares same property, to check the correctness of a model. \tvn{Also say that requiring thse tests are NOT natural for Alloy developers, which often just write general assertions or predicates, not something as specific as a test}\gz{Do we need some support papers to say that tests are not natural for Alloy?}




%% Thus, automatic fault localization techniques, which help automatically identify buggy code, are useful in helping developers find, understand, and fix bugs in Alloy.
%% Fault localization in Alloy is different from imperative programming language like C or Java which consist of executable statements that behave differently depending on the inputs (e.g., some do not even get executed).
%% Many techniques have been developed based on this feature to locate bugs for imperative program.
%% For example, one of the most popular debugging technique, statistical debugging, locates bug by collecting statistical information of statements executed by passing and failing test cases. However, unlike imperative language, Alloy doesn't have statement or execution trace, all facts and called predicates or asserts are translated togother to one boolean formula. The techniques used for imperative programs couldn't directly apply to declarative domain
%% %\tvn{why not? AlloyFL uses mutation testing and statistical debugging in imperative domains.  Need to say something about orders do not matter in SAT formula}.
%% Bug localization in declarative language requires completely different fault localizaiton techniques.



%is gaining more attentions due to its expressiveness, effectiveness, and ease of use.%Alloy is used mainly for \emph{modeling}\tvn{expand a bit more about this}\gz{Probablly need some help from Hamid to expand this, I don't know any papers to support the usage of Alloy}.
%Alloy has been applied to a variety of software problems, such 

%When developer write Alloy models, they also make mistakes, e.g., in the models, which result in intended properties not being satisfied.


To address this state of affairs and improve the quality of Alloy development, %we present {\tool}, a technique and tool that finds faulty expressions causing an assertion violation in an Alloy model.
we present an automated approach and an accompanying tool-suite for \textbf{f}ault \textbf{l}ocalization in \textbf{A}lloy models using \textbf{c}ounterexamples, called {\tool}. %FLACK.
Given an Alloy model and a property that is not satisfied by the model, {\tool} first queries the underlying Alloy Analyzer for a counterexample, an instance of the model that does not satisfy the property.
Next, {\tool} uses a partial max sat (PMAXSAT) solver to find an instance that does satisfy the property and is as close as possible to the counterexample.
{\tool} then determines the relations and atoms that are different between the cex and sat instance.
Finally, {\tool} analyses these differences to compute suspicious scores for expressions in the original model.

%Thus instead of using many tests as in AlloyFL, 
Unlike AlloyFL that relies on unconventional unit tests,  %to the Alloy environment,
{\tool} uses well-established and widely-used assertions, %familiar to Alloy users.
naturally compatible with the development practices in Alloy.
Also, instead of using mutation testing or statically analyzing the effects of tests, {\tool} relies on counterexamples and satisfying instances generated by constraint solvers, which are the main underlying technology in Alloy. 


We evaluated {\tool} on a benchmark consisting of a suite of %56 
buggy models from AlloyFL~\cite{alloyfl}. The experimental results corroborate that {\tool} is able to consistently rank buggy expressions in the top 1.9\% of the suspicious list. We also evaluated {\tool} on three case studies consisting of larger Alloy models used in the real-world settings (e.g., Alloy model for surgical robots, Java programs and Android permissions), and {\tool} was able to identify the buggy expressions within the top 1\%.
The run time of {\tool} for most the %each of these 56 
models is under 5 seconds (under 1 second for the AlloyFL benchmarks).
%% We evaluates {\tool} on 55 examples adapted from ARepair ~\cite{arepair} which consists of examples from Alloy book and homework of Alloy models. We also evaluate for XX real and large examples from XX. {\tool} is able to rank to top 3 locations for 34 out of 55 bugs and able to tell related information for the rest 21 bugs. The result shows that {\tool} is able to accurately locate bug and the analysis time is under 5 seconds. We also classify these bugs based on its corresponding repair. {\tool} works well when the repair needs to modify existing constraints, but not when the repair needs to add completely new constraints.\tvn{We also classify these bugs,  {\tool} works well on 3 classes but not in 1 class ...}
%% The contributions of this paper are:
%% \begin{itemize}
%% \item We propose a novel automatic fault localization technique for Alloy based on counterexamples. \tvn{Guolong}
%% \item We propose a novel method to isolate relations in counterexample that cause the error by reducing it to a PMAXSAT problem. \tvn{Guolong}
%% \item We implement the fault localization technique in a prototype tool, {\tool}, and evaluates it on 56 Alloy models collected from ARepair~\cite{arepair} and 2 large Alloy models from real world problems of surgical robots~\cite{robots} and Java program verification~\cite{taco}.\tvn{Guolong}
%% \end{itemize}
The experimental results corroborate that
{\tool} has the potential to facilitate a non-trivial task of formal specification development significantly
%We believe that {\tool} takes an important step in finding bugs in Alloy and analysis of Alloy model 
and exposes opportunities for researchers to exploit new debugging techniques for Alloy. 
%We also note that while BFA is designed for Alloy, our technique can be generalized to other declarative languages that use constraint solvers to generate counterexamples and instances, e.g., the modeling languages Promela~\cite{spin} and NuSMV~\cite{nusmv}.
%\tvn{Guolong: cite these papers: NuSMV: An opensource tool for symbolic model checking, The model checker Spin, and The SPIN model checker}. \gz{cited NuSMV and SPIN}
%that do not have imperative notions of control flow or statements.

To summarize, this paper makes the following contributions:
\begin{itemize}
%\vspace{-0.2cm}
\item \textit{Fault localization approach for declarative models}:
We present a novel fault localization approach for declarative models specified in the Alloy language. The insight underlying our approach is that expressions in an Alloy model that likely cause an assertion violation can be identified by analyzing the counterexamples and closely related satisfying instances.


\item \textit{Tool implementation}: We develop a fully automated
technology, dubbed {\tool}, that effectively realizes our
fault localization approach. We make {\tool} publicly available to the research and education~community~\cite{BFA}.



\item \textit{Empirical evaluation}: We evaluate {\tool} in the context of faulty Alloy specifications found in prior work and specifications derived from real-world systems, corroborating {\tool}’s ability to  consistently rank buggy expressions high on the suspicious list, and analyze complex, real-world Alloy models with thousand lines of code.
%in the top 1.9\% no longer accurate
\end{itemize}
 
%tvn: temp comment for space
The rest of the paper is organized as follows. Section~\ref{Illustration} motivates our research through an illustrative example. Section~\ref{sec:approach} describes the details of our fault localization approach for Alloy models. Section~\ref{sec:eval} presents the implementation and evaluation of the research. The paper concludes with an outline of the related research and future work.

%% and a counterexample violates this assertion, {\tool} automatically locates bug to the boolean formula level. {\tool} first identifies which relation should be added or removed by comparing models. {\tool} converts the assertion to predicate to generate an expected instance. The difference between counterexample and expected instance indicates relations that cause violation of the assertion in counterexample. However, due to randomness in Alloy search, this difference may be very large and contains misleading informations. {\tool} reduce this problem to a partial Max Sat(PMAXSAT)\tvn{use another name, maxsat or something} problem to minimize the difference such that it only contains necessary information. {\tool} is then able to locate bug by mapping these differences to the causes in the model, the causes to the differences\tvn{clause?} are possible bug locations\tvn{there's no feedback or iterative loop here?}\gz{no feedback as we are not repairing}. We then rank these causes based on their suspicious level.   




%{\tool} takes as inputs an Alloy model and an assertion that is not satisfied by the model, and returns a set of suspicious expressions in the model that cause the assertion violation.
%{\tool} uses the backend Alloy Analyzer to generate counterexamples and satisfying instances, compute the the differences

%targets different scenarios than AlloyFL. Given a model and an assertion, Alloy verifies model's correctness by searching for a counterexample violates the assertion. The presence of a counterexample indicates an error in the model. {\tool} then automatically identifies tuples for each relations that should be removed or added in the counterexample such that the counterexample no longer violates the assertion. This modification is then utilized to locate bugs in the original model. This eliminate the requirements for tests or correct model in AlloyFL. 

%\tvn{what is the granularity level ?  Talk about that here}

%We evaluates {\tool} on 55 examples adapted from ARepair ~\cite{arepair} which consists of examples from Alloy book and homework of Alloy models. We also evaluate for XX real and large examples from XX. {\tool} is able to rank to top 3 locations for 34 out of 55 bugs and able to tell related information for the rest 21 bugs. The result shows that {\tool} is able to accurately locate bug and the analysis time is under 5 seconds. We also classify these bugs based on its corresponding repair. {\tool} works well when the repair needs to modify existing constraints, but not when the repair needs to add completely new constraints.\tvn{We also classify these bugs,  {\tool} works well on 3 classes but not in 1 class ...}





==> pldi21/motivating.tex <==
\section{Illustration}
\label{Illustration}
\begin{comment}
\begin{figure}[t]
\begin{lstlisting}[language=Alloy, escapechar=?, escapeinside={(*@}{@*)}]
one sig FSM { 
  start: set State
  stop: set State 
}
sig State { transition: set State } (*@\label{line:sig}@*)
fact OneStartAndStop {
  all start1,start2: FSM.start | start1 = start2
  all stop1,stop2: FSM.stop | stop1 = stop2
  some FSM.stop
}
fact ValidStart{
  FSM.start !in FSM.stop
  all s: State | FSM.start !in s.transition (*@\label{line:unsat1}@*)
  State = FSM.start.*transition
} 
fact ValidStop{
  all s:State | FSM.stop in s.*transition (*@\label{line:sexp1}@*)

  // error: should be <=> instead of =>
  all s:State |
    s.transition=none => s in FSM.stop (*@\label{line:bug}@*)
}
assert NoStopTransition{ (*@\label{assert}@*)
  no FSM.stop.transition
}
\end{lstlisting}
\caption{Buggy FSM model.}
\label{fig:ex}
\end{figure}
\end{comment}
\begin{figure}[t]
\begin{lstlisting}[language=Alloy, escapechar=?, escapeinside={(*@}{@*)}, basicstyle=\footnotesize\ttfamily]
one sig FSM {
  start: set State,
  stop: set State
}
sig State { transition: set State } (*@\label{line:sig}@*)
fact OneStartAndStop {
  // FSM only has one start state.
  all start1, start2 : FSM.start | start1 = start2
  // FSM only has one stop state.
  all stop1, stop2 : FSM.stop | stop1 = stop2
  some FSM.stop
}
fact ValidStartAndStop {
  // A state cannot be both a start and a stop state.
  FSM.start !in FSM.stop
  // No transition ends at the start state.
  all s : State | FSM.start !in s.transition (*@\label{line:unsat1}@*)
  // Error: should be "<=>" instead of "=>".
  all s: State | s.transition = none => s in FSM.stop (*@\label{line:bug}@*)
}
fact Reachability {
  // All states are reachable from the start state.
  State = FSM.start.*transition
  // The stop state is reachable from any state.
  all s: State | FSM.stop in s.*transition (*@\label{line:sexp1}@*)
}
assert NoStopTransition{
	no FSM.stop.transition
}
check NoStopTransition for 5
\end{lstlisting}
\caption{Buggy FSM model, adapted AlloyFL~\cite{alloyfl}.}
\label{fig:ex}
\end{figure}

To motivate the research and illustrate our approach, we provide an Alloy specification of a finite state machine (FSM), adapted from AlloyFL benchmarks~\cite{alloyfl}.
%We use the Alloy model in Figure~\ref{fig:ex} to motivate the use of {\tool}. This model specifies a simple type of finite state machine (FSM), adapted from ARepair benchmarks~\cite{arepair}, with the following constraints, expressed as fact paragraphs in Alloy.
The specification defines two type signatures, i.e., \texttt{State} and \texttt{FSM}, along with their fields (lines 1--5). The specification contains three fact paragraphs, expressing the constraints, detailed below:
The FSM consists of only one start and one stop state (fact \texttt{OneStartAndStop}).
A state cannot be both a start and a stop state; no transition terminates at the start state; and no transition leaves a stop state (fact \texttt{ValidStartAndStop}).
Finally, every state is reachable from the start state, and  the stop state is reachable from any state (fact \texttt{Reachability}).


Each \texttt{assertion} specifies a property that is expected to hold in all instances of the model.
%To check that our requirements are satisfied by the model, we express them as assertions and check them using the Alloy Analyzer.
For example, we use the assertion \texttt{NoStopTransition} to check that a stop state behaves as a sink.
However, the Alloy Analyzer disproves this assertion by producing a counterexample, shown in Figure~\ref{fig:cex1}, in which the stop state labeled \texttt{State3} transitions to \texttt{State1}.

Thus, there is a ``bug'' in the model causing the assertion violation.
Indeed, careful analysis of the model and the generated cex reveals that the problem is in the expression on line~\ref{line:bug}: instead of stating that a stop state does not have any transition to any state, the expression states that any state not having a transition to anywhere is a stop state---a subtle logical error that is difficult to realize\footnote{There are two potential fixes for this: (i) reverse the expression to: \texttt{s in FSM.stop => s.transition=none} %(since there is no \texttt{<=} operator in Alloy) 
or (ii) replace the implication operator (\texttt{=>}) to logical equivalence (\texttt{<=>}), which technically would strengthen the intended requirement.}.

\begin{table}[h]
  \caption{{\tool}'s results obtained for the model in Figure~\ref{fig:ex}.}
\label{table:model1}
  \small
  \centering
  \begin{tabular}{l  l }
    \hline  
    \hline
    Suspicious Expression & Score \\
     \hline     
     s.transition = none =$>$ s in FSM.stop (=$>$)  & 1.58 \\
     s.transtion = none & 1.25 \\
     FSM.stop in s.*transtion  &  0.5 \\
     s in FSM.stop  & 0.5  \\
     \hline
     \hline     
  \end{tabular}
\end{table}

The goal of {\tool} is to identify such buggy expressions automatically.
For this example, within a second, {\tool} identifies four suspicious expressions with the one on line~\ref{line:bug} ranked first. Table~\ref{table:model1} shows the results: expressions or nodes with higher scores are ranked higher.
Moreover, {\tool} suggests that the operator \texttt{=>} is likely the issue in the expression.
Such a level of granularity can significantly help the developer understand and fix the problem.
The results in Section~\ref{sec:eval} show that {\tool} can consistently rank the exact buggy expression within the top 5 suspicious ones and do so under a second.



%% Suppose that we want to model a simple type of finite state machine (FSM) and it should have the following properties. The FSM contains one start and stop state, the start and stop state are distinct, no incoming transition to the start state, all states are reachable from the start state and the stop state is reachabe by any state. In addition, a state that has no outgoing state is a stop state.


%% We then implement this model using Alloy specification as shown in Figure~\ref{fig:ex}.
%% First, we use \emph{sigs} to specify that the FSM has start and stop states and a state has a transition to a set of states.
%% The fact \texttt{OneStartAndStop} defines a constraint that there is only one start and one stop state and there must be some stop. The fact \texttt{ValidStart} defines that start is not a subset of stop, all state transition shouldn't point to start state, and all state are reachable from start state following relation transition.
%% The fact \texttt{ValidStop} stop are in the end of all transition, if a state has no transition then it is the stop state.
%% To check the requirement that this all stop states of this FSM contain no outgoing transitions, we use the assertion \texttt{NoStopTransition} at line~\ref{assert}.
%% \tvn{can you quickly define the terminologies used in Alloy that you will use throughout the paper? e.g., sentence, relation, atom, expression, etc and give examples of each from the figure.  Most people are not familiar with Alloy and might get confused.}

%% \tvn{I think in this particular example, we should just say here what the bug is,  e.g., this assert will fail because of the expression on line X.  Our goal is to be able to automatically identify this expression.  Also say why it is not easy to do this.  At this place, it might be a good time to reminder the user that finding Alloy bug is different than imperative bugs because no ordering in program execution.   Also mention here that normal Alloy approach on using unsat cores will not work directly,  because assertion violation means we do get satisfying model, i.e., cex's. }\gz{Add the following paragraphs:}
%% The bug locates at line 18 \code{all s : State | s.transition = none => s in FSM.stop}, which says that if a state has no transition, then it should be a stop state. Alloy produces a cex as shown in Fig ~\ref{fig:cex1} when running \code{check NoStopTransition}, indicating an error in this model. 

% TODO: use this later
%% From the cex, it is hard to tell which part of the algorithm is reponsible to the error. If this were an imperative language like C or Java, developer would write some tests and check statements exectuted differently in passing tests and failing tests. However, in Alloy, there is no such context of test cases and all 'statements' are translated togather to one boolean formula. A popular method to fault localization in Alloy is using UNSAT core, ~\cite{unsat1}, however, UNSAT core only exists when Alloy couldn't find any instances, in other words, no cex when checking an assert usually means no bug.


\begin{comment}
%moved to the approach section
\subsection{Overview}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{arch}
    \caption{{\tool} Work Flow}
    \label{fig:workflow}
\end{figure}

Figure~\ref{fig:workflow} gives an overview of {\tool}, which takes as input an Alloy model with some violated assertion and returns a ranked list of suspicious expressions contributing to the assertion violation.
The insight guiding our research is that the differences between counterexamples that do not satisfy the assertion and closely related satisfying instances can derive localization of suspicious expressions in the input model.
To achieve this, {\tool} uses the \emph{Alloy analyzer} to find counterexamples showing the violation of the assertion.
Then, it uses a PMAX-SAT solver to find satisfying instances that are \emph{as close as possible} to the cex's.
Next, {\tool} analyzes the differences between the cex's and satisfying instances to find expressions in the model that likely cause the errors.
Finally, {\tool} computes and returns a ranked list of suspicious expressions.

\end{comment}

%\textcolor{cyan}{HB: Double check the previous paragraph after finalizing the Intro to omit potential repetitive sentences.}
  
%% To check the correctness of an Alloy specification, Alloy developer usually write an assertion and check to see if there is any counterexample. The presence of a counterexample indicates the model contains bugs. We presents {\tool} to locate the bug.

%% Given an Alloy specification with assertion and a corresponding predicate, {\tool} outputs an ordered list of AST nodes based on their possibility to the bug. {\tool} consists parts as shown in ~\ref{fig:workflow}. We will discuss each components next.


%\subsection{Example}
The key idea underlying our fault localization approach is to analyze the differences between \emph{counterexamples} (instances of the model that do not satisfy the assertion) and instances that do satisfy the assertion to find suspicious expressions in the input model.
%We use the model in Figure~\ref{fig:ex} to show how {\tool} works.
{\tool} first checks the assertion \code{NoStopTransition} in the model using the Alloy Analyzer, which returns the cex in Figure~\ref{fig:cex1}.
Next, {\tool} generates a satisfying (sat) instance that is as minimal and similar to the cex as possible.
%The idea is that 
Their differences promise effective localization of the issue.
%\tvn{talk about difficulties in just using Alloy to generate sat instances}

\paragraph{Generating SAT instances} To obtain an instance similar to the cex, {\tool} transforms the input model into a logical formula representing \emph{hard constraints} and the information from cex into a formula representing \emph{soft constraints}.
Essentially, {\tool} converts the instance finding problem into a \emph{Partial-Max SAT} problem~\cite{pmaxsat} and then uses the Pardinus~\cite{pardinus} solver to find a solution that satisfies all the hard constraints and as many soft constraints as possible.
Thus, the result is an instance of the model that is similar to the cex but satisfies the assertion.
Figure~\ref{fig:expected1} shows an instance produced by Pardinus, considering the cex shown in Figure~\ref{fig:cex1}.
Notice that this instance is similar to the given cex, except for the edge from \texttt{State3} to \texttt{State1}, which represents the main difference between the two instances.

\begin{figure}
  \centering  
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=1\linewidth]{cex1.png}
    \caption{Counterexample}
    \label{fig:cex1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=1\linewidth]{expt1.png}
    \caption{(PMAX) Sat instance}
    \label{fig:expected1}
  \end{subfigure}
  \caption{Instance Pair. Notice that these instances are very similar.}
  \label{fig:pair1}
\end{figure}



%\tvn{STOP HERE FOR NOW}
%To automatically locate errors, \tool generates a minimal sat instance based on the cex, and using the difference to locate the bug.


%% \begin{figure}
%% \centering
%%     \begin{subfigure}{0.25\textwidth}
%%     \centering
%%         \includegraphics[width=0.9\linewidth]{res/images/cex1.png}
%%         \caption{Counter Example}
%%         \label{fig:cex2}
%%     \end{subfigure}%
%%     \begin{subfigure}{0.25\textwidth}
%%     \centering
%%         \includegraphics[width=0.9\linewidth]{res/images/expectedins1.png}
%%         \caption{Expected Instance}
%%         \label{fig:expected2}
%%     \end{subfigure}
%%     \caption{Instance Pair 2}
%%     \label{fig:pair2}
%% \end{figure}

%\lstinputlisting[language=Alloy, label=model2, caption=Sliced Model]{res/fsm_sliced.als}

%% \paragraph{Obtaining cexs} To check whether this property holds for certain bounds, we run the command \code{check NoStopTransition for 5}. Alloy then generates a cex as shown in ~\ref{fig:cex1}, indicating the model doesn't always satisfying the expected property. Manually inspect cex, we could find the violation is cause by that the stop state \code{State1} in the cex has a transition to \code{State2}, which violates the stated property in assertion that stop state shouldn't have any outgoing transitions. 

%% \paragraph{Obtaining minimal sat instances} To automatically find the cause to the violation in cex, we change the assert at line~\ref{assert} to a predicate \code{pred NoStopTransition \{ no FSM.stop.transition \}} and run command \code{run NoStopTransition for 5}. Alloy then generates an instance that satisfies the no outoging transition for stop state proeprty as shown in ~\ref{fig:expected2}. Due to the randomness of Alloy model finding, this instance is very different from the cex shown at ~\ref{fig:cex1}. The expected instance contains one more sig and the transitions between them are very different from the cex. Many information that not related the error will misslead the localization result. 

%For the cex in Fig ~\ref{fig:cex1}, the best expected instance is the instance shown at Fig ~\ref{fig:expected1}, where the difference between these two is exactly the cause of the violation. However due to the randomness of Alloy's model finding, to get one sat instance that is closest to the counterxample as shown in Fig ~\ref{fig:expected1}, we may need to ask Alloy many times and we may not get the right one needed. For example, the instances in ~\ref{fig:randoms} are instances getting by asking Alloy to generate next instance 2 times, none of them is that useful for locating bug. 

%% \begin{figure}
%%     \centering
%%         \begin{subfigure}{0.25\textwidth}
%%         \centering
%%             \includegraphics[width=0.9\linewidth]{res/images/random1.png}
%%             %\caption{Counter Example}
%%             \label{fig:random1}
%%         \end{subfigure}%
%%         \begin{subfigure}{0.25\textwidth}
%%         \centering
%%             \includegraphics[width=0.9\linewidth]{res/images/random2.png}
%%             %\caption{Expected Instance}
%%             \label{fig:random2}
%%         \end{subfigure}
%%         \caption{Random Alloy Instances}
%%         \label{fig:randoms}
%%     \end{figure}

%This search for most similar instance depends on pure luck due to the randomness model finding of Alloy. To address this problem, {\tool} modifies Alloy such that it is able to generate an instance that is as similar as a target instance. We reduce this problem to a partial max sat problem, where the original Alloy model is hard constraints and the cex is soft constraints, and use an existing tool Pardinus ~\cite{pardinus} to solve this PMAXSAT problem\tvn{{\tool} modifies Alloy or {{\tool}} uses some existing work to do this?}\gz{add reference}. When the sovler solves this formula, all hard constraints must be satisfied and as many as soft constraints should be satisfied. The result is an instance the most simialr as the cex.Another advantage of using PMAXSAT is that we don't need to mapping name of sigs in cex with that in expected instance. 

%Applying this approach, given the cex at fig ~\ref{fig:cex1}, {\tool} could directly generate the corresponding instance at fig ~\ref{fig:expected1}, where the difference is the cause of the violation. The causes for this difference in Alloy model are potential bug locations. 

%Each sentence in Alloy model ~\ref{fig:ex} affects different relations. For example, 
%To capture different scenarios of how cexs violates the assertion, {\tool} generates 2 pairs of counterxample and expected instances as shown in Fig ~\ref{fig:pair1} and ~ref{fig:pair2} respectively.\tvn{how do you know you need a different scenario?  How do you know the pair in Figure 4 is good enough and stop there? how many different scenarios do you need to do? Does the algorithm generate a pair, analyze it, if it doesn't work, then try to generate another one ? and so on ?  or does it generate some fixed number of pairs and analyze them ?  What if it doesn't find what it wants (how do you know what you want?),  then what does it do? }

% \begin{figure}
%   \small
% \begin{verbatim}
% FSM={FSM}
% start={FSM->State0}
% stop={FSM->State3}
% State={State0, State1, State2, State3}
% transition={State0->State1, State0->State3, 
%     State1->State2, State2->State3, State3->State1}  
% \end{verbatim}
% \caption{Textual representation of the cex in Figure~\ref{fig:cex1}.}
% \label{fig:textrepr}
% \end{figure}

\paragraph{Finding Suspicious Expressions} {\tool} analyzes the differences between cexs and the sat instances---e.g., here the transition from \texttt{State3} to \texttt{State1}, which only appears in the cex but not the sat instance---to identify Alloy relations causing the issue.
As shown in Table~\ref{fig:textrepr}, that demonstrates the Alloy text representation of the cex in Figure~\ref{fig:cex1}, the \texttt{transition} relation involves the tuple \texttt{State3 -> State1} and the \texttt{stop} relation involves \texttt{State3}.
Thus, {\tool} hypothesizes that two relations of \texttt{transition} and \texttt{stop} may cause the difference in the two models.
Note that while we present one cex and one sat instance in this example for the sake of simplicity, {\tool} supports analyzing multiple pairs of cex and sat instances in tandem. %by focusing on shared differences.


\begin{table}[h]
  \caption{Text Representation of the cex in Figure~\ref{fig:cex1}}
  \label{fig:textrepr}
  \begin{tabular}{|c|c|}
    \hline
    Relation  &  Tuples \\ 
    \hline
    FSM       &  FSM0  \\
    \hline
    start     &  FSM0-$>$State0 \\
    \hline
    stop      &  FSM0-$>$State3 \\
    \hline
    State     &  State0, State1, State2, State3 \\
    \hline
    \multirow{2}{4em}{transition} & State0-$>$State1, State0-$>$State3, State1-$>$State2, \\
                             & State2-$>$State3, State3-$>$State1 \\ 
    \hline
  \end{tabular}
\end{table}



%To locate bug, {\tool} first infers affected relations based on difference between cex and expected instance. For the first pair in Fig ~\ref{fig:pair1}, the relation with different tuples is \code{transition}, where the tuple \code{State3->State1} is present in cex and not in expected instance. This means that if we removing this tuple in cex, then it no longer a cex. \tvn{what about the first pair?  why not use it?}\gz{change to the first pair, but after adding one more step, there is no need to use the second pair. add below for the reason why need another pair.}

%Why this tuple is different from other tuples in the same relation? So we try to analysis each atom and infer how these atoms different from other atoms. Based on the text representation ~\ref{text1} of cex1, we check all appearance of \code{State1} and \code{State3} in relations other than its original type \code{State} and the different relation \code{transition}. \code{State3} appears in \code{FSM.stop} and \code{State1} doesn't appear in any other relations. We infer that \code{FSM.stop} is also a possible relations that affects the cex. \gz{add one sentence to explain the neccessary of using another pair of instances}. To ensure that all keywords are general across other cex, for example, \code{FSM.stop} is applied to other cexs, \tool generates multiple pairs of counterexmaple and expected instace, and use the summary of all pairs for keywrods extraction. For example, another pair of instances is shown as in ~\ref{fig:pair2}.

After determining the relations \texttt{transition} and \texttt{FSM.stop}, {\tool} \emph{slices} the input model to contain only expressions affecting both relations.
This results in two expressions:

%\begin{centering}
\noindent
  \texttt{all s: State | FSM.stop in s.*transition} (line~\ref{line:sexp1})\\
  %and\\
\noindent 
  \texttt{all s: State | s.transition = none => s in FSM.stop} (line ~\ref{line:bug})
%\end{centering}

At this point, {\tool} could stop and return these two expressions, one of which is the buggy expression on line~\ref{line:bug}.
Indeed, this level of ``statement'' granularity is often used in fault localization techniques, like Tarantula~\cite{tarantula} or Ochiai~\cite{spfl1}.
However, {\tool} aims to achieve a finer-grained granularity level by also considering the \emph{boolean} and \emph{relational} subexpressions, detailed below.

\paragraph{Ranking Boolean Nodes} The expressions on lines~\ref{line:sexp1} and~\ref{line:bug} have four boolean nodes: (a) \texttt{FSM.stop in s.*transition}, (b) \texttt{s.transition = none}, (c) \texttt{s in FSM.stop}, and (d) \texttt {s.transition = none => s in FSM.stop}.
{\tool} instantiates each of these with \texttt{State1} and \texttt{State3}, the values that differentiate the cex and sat instance.
For example, (a) becomes \texttt{FSM.stop in S1.*transition} and \texttt{FSM.stop in S3.*transition}. Next, {\tool} evaluates these instantiations using the cex and sat instance and assigns a higher suspicious score to those with inconsistent evaluation results.
For example, the instantiations \texttt{FSM.stop in S1.*transition} and \texttt{FSM.stop in S3.*transition} of node (a) evaluate to \texttt{true} in both cex and sat instance, so we give (a) the score 0 (i.e., no changes).
We assign score 1 to (b) because \texttt{State3.transition = none} evaluates to \texttt{false} in the cex but \texttt{true} in the sat instance (thus 1 change) and \texttt{State1.transition = none} evaluates to false in both (no change).

Overall, {\tool} obtains the scores 0, 1, 0, 1 for nodes (a), (b), (c), (d), respectively.
%Note that the score of (d) is essentially the sum of the scores of (b) and (c) as these are subexpressions of (d).
Thus, {\tool} determines that nodes (b) \texttt{s.transition = none} and (d) \texttt {s.transition = none => s in FSM.stop} are the two most suspicious boolean subexpressions within the expression on line~\ref{line:bug}.


%Similarly, (c) gets a score 0 and (d) gets a score of 0. Also as (b) and (c) is a node of (d), (d) also gets a score of sum of (b) and (c). Overall (d) get a score of 1.


%Also for, \texttt{s.transition = none => s in FSM.stop} gets a priority 1 based on its own evaluation 0 and the sum of all its child nodes 1. 

%First, we instantiate each sentence using values involved in the difference. For example, given the difference \texttt{transition:\{State3->State1\}}, \texttt{all s: State | FSM.stop in s.*transiton} is instantiated to \texttt{FSM.stop in State1.*transtion} and \texttt{FSM.stop in State3.*transiton}; \texttt{all s : State | s.transition = none => s in FSM.stop} to \texttt{State1.transition = none => State1 in FSM.stop} and \texttt{State3.transition = none => State3 in FSM.stop}.

%% Second, we try to calculate the priority at the boolean formula level by evaluating each boolean formula in the context of couterexample and expected instance, if the value changes we assign that formula a high score. 

%% In this example, there are total 4 boolean formulas: \texttt{FSM.stop in s.*transition}, \texttt{s.transition = none}, \texttt{s in FSM.stop} and \texttt{s.transition = none => s in FSM.stop}
\paragraph{Ranking Relational Nodes}  While subexpression (d) indeed contains the error, it receives the same score as subexpression (a).
To achieve more accurate results\footnote{While this example has only two expressions with similar scores,  we obtain many expressions with similar scores in more complex and real-world models. Thus, this step is crucial to distinguish the buggy expressions from the rest.}, {\tool} further analyzes the involving relations.
{\tool} instantiates these relations with \texttt{State1} and \texttt{State3}, assesses them in the context of the cex and sat instances, and assigns scores based on the evaluations.
For example, node (d) \texttt{s.transition = none => s in FSM.stop} contains 3 relations:
(1) \texttt{s.transition},
(2) \texttt{s}, and
(3) \texttt{FSM.stop}.
Instantiating these relations with \texttt{State3} and evaluating them using the cex is as follows:
(1) becomes \{\texttt{State1}\},
(2) \{\texttt{State3}\}, and
(3) \{\texttt{State3}\}.
Thus, for the cex, (d) involves both \texttt{\texttt{State1}} and \texttt{\texttt{State3}}, and {\tool} gives it a score of 1.
Next, it evaluates the instantiations using the sat instance as follows:
(1) becomes \{\},
(2) \{\texttt{State3}\}, and
(3) \{\texttt{State3}\}.
(d) does not involve \texttt{State1} and thus has a score 0.
{\tool} assigns (d) the average score of 0.5 (for the instantiations of \texttt{State3}).
Performing a similar computation for the instantiation of \texttt{State1}, we obtain a score of 2/3 for (d) as the evaluation for the cex and sat instances involves both \texttt{State1} and \texttt{State3} (differentiated values) and \texttt{State2} (regular value). %which is not in the differentiated values.
Thus, (d) has a score of 0.58 as an average of 0.5 and 2/3.

Overall, {\tool} obtains the scores 0.5, 0.25, 0.5,  0.58 for (a), (b), (c), and (d), respectively.
Note that the node (d) is now ranked higher than (a) as desired.

\paragraph{Suspicious Scores}
{\tool} computes the final suspicious score of a node as the sum of the boolean and relational scores of that node, as shown above.
For example, the node (d) \texttt{s.transition = none => s in FSM.stop} in the expression on line~\ref{line:bug} has the highest suspicious score of 1.58.
Table~\ref{table:model1} shows suspicious scores of the expressions in the ranked list returned by {\tool}.


In addition, %as a ``bonus'' heuristics, 
{\tool} analyzes (non-atomic) nodes containing (boolean) connectors and reports connectors that connect subnodes with different scores.
For example, {\tool} suggests that the operator \texttt{=>} is likely responsible for the error in (d) because the two subexpressions \texttt{s.transition = none} and \texttt{s in FSM.stop} have different scores as shown in Table~\ref{table:model1}.
Indeed, in this example, the assertion violation is entirely due to this operator (a potential fix would be strengthening the model to \texttt{<=>} or switching the two subexpressions as Alloy does not have the operator \texttt{<=}).

%% {\tool} further analyzes the boolean connectors among the resulting suspicious nodes.
%% Third, we calculate the priority for boolean formula at AST node level based on its potential impact to other values. This priority is trying to capture the following impacts: The evaluated value should contain other values in difference and should contain less values that are not in the difference. 

%% Given the value State3, in counterexample,
%% (1) evaluates to \{State1\},
%% (2) to \{State3\} and
%% (3) to \{State3\},
%% (d) gets a score 1 for value State3 in counterexample;
%% in sat instance, (1) to \{\},
%% (2) to \{State3\} and (3) to
%% \{State3\},
%% (d) gets a score 0 for value State3 in sat instance as it doesn't contain value State1.
%% (d) then gets a score of 0.5 as the average of score for State3.
%% Similarly, for value State1, (1) to \{State2\}, (2) to \{State1\} and (3) to \{State3\} in both counter and sat instances, (A) then gets a score of 2 / 3. Overall, expression (d) get a score of 0.58 as an average of value State1 and State3. 

%% Similarly (a) gets a score 0.5(2/3 for State1 and 1/3 for State3), (b) gets a score 0.25(0 for State1 and 0.5 for State3), (c) gets a score of 0.5(1 for State1 and 0 for State3). 

%% The overall score for an experssion is the sum of step 2 and step 3, as shown in table ~\ref{table:model1}. Then for the ''large'' expression (d), we apply the following heuristic to further narrow down the error: if the left subexpression and right subexpression has a different score, then we report the operator as a most suspicious location.




% \code{State1.transition = none => State1 in FSM.stop} where \code{State1.transition} $\equiv$ \{State2\}; \code{none} $\equiv$ \{\}; FSM.stop $\equiv$ \{State3\}. So every AST node in \code{s.transtion = none} gets a score 0 as it doesn't contain \code{State3}, \code{State1 in FSM.stop} gets a score of 1 and \code{s.transition = none => s in FSM.stop} gets a score of 1. 
% \code{State3.transition = none => State3 in FSM.stop} where \code{State3.transition} $\equiv$ \{State1\}; \code{none} $\equiv$ \{\}; FSM.stop $\equiv$ \{State3\}. So every AST node in \code{s.transtion = none} gets a score 1, \code{s in FSM.stop} gets a score of 0 and \code{s.transition = none => s in FSM.stop} gets another score of 1.

% For example, \code{FSM.stop in State1.*transition} contains two expressions: \code{FSM.stop} and \code{State1.*transition}. \code{FSM.stop} evaluates to \code{\{State3\}} and \code{State1.*transition} to \code{\{State1, State2, State3\}}. The union of result is \code{\{State1, State2, State3\}}. It contains all different values \code{\{State1, State2\}} and one extra value \code{\{State3\}}, so we give a score 2/3 to \code{FSM.stop in s.*transition}. Similarly \code{FSM.stop in State3.*transition} gives another score of 2/3. Overall, \code{FSM.stop in s.*transtion} get a score of 4/3.
% %Similarly, \code{State1.transition = none} contains expression \code{State1.transition} evaluates to \code{State2} and gets a priority 1/1 and its total priority is calculated to 2 by adding the priority calculated in the second step; \code{State1 in FSM.stop} contains expression \code{FSM.stop} evaluates to \code{State1}, doesn't contain the different value \code{State2} and gets a priority 0. \code{State1.transtion = none => State1 in FSM.stop} then intotal gets a priority of 2. 

% Overall, \code{s.transition = none => s in FSM.stop} gets the highest score 3 and ranked first in the output list. Among them the operator \code{=>} with a score of 3 is most suspicious. The operator is reported when the left node and right node has imbalanced score\tvn{Meaning what?}. As shown in table ~\ref{table:ranklist1}. The fix would be changing \code{=>} to \code{<=>}.
% %\tvn{what are ranked second, third, etc ?  can you create a table showing this ranked list}.\gz{added below:}


%TODO: put this in alg
%\tvn{Also, here is where we should say something interesting about the algorithm,  e.g., could you create several scenarios and show what the result would be ? e.g., instead of the bug on line X that we are having,  if the bug is something else,  then what would the algorithm do ?  These kind of things.  Also may give a scenario where you cannot find anything useful}\gz{add below:}
%% \tool is also able to locate another kind of bug, where Alloy couldn't find any expected instance given a cex. For example, if we change line 17 to \code{all s : State | s.transtion !in FSM.start}, Alloy generates same cex when checking the assertion but outputs \textbf{No instance found} when running the predicate. This is caused by that if there is no transition for stop state, then stop state's transition is empty and is a subset of \code{FSM.start}, inconsistent with line 17. Alloy provides UNSAT cores as commented by \/\/1 in the buggy model. \tool then locate bug by identify causes to the inconsistency in UNSAT core. This is done by removing all constraints involved in UNSAT cores, then run predicate to generating the minimal difference sat instance, then evaluate the difference in the context of sat instance and check which constarint(s) is evaluated to false and this constraint(s) is the bug location. 

%% \tool couldn't work well when constraint related to the assertion is completely missing in the model. For example, if we delete line 18, then \tool locates to line 17 which is correct and not related to the bug.



%Build an abstract representation graph for Alloy model.

%For each sentence, {\tool} calculate a priority based on its suspicious level. The score is calcualted as: for boolean expressions, if its value changed between expected instance and cex, it got a higher priority. for expressions return a set of values, the priority is calculated as the ratio to the number of values in difference.

% \begin{comment}
% To check that property, we run $check NoStopTransition$ to tell Alloy check the assertion. Alloy then produces a cex as shown in ~\ref{fig:cex1}, indicating an inconsistency between specification and assertion. As this counter example is simple, it is easy to see what causes the assertion to fail: there is a transition to state1 which is the stop state\tvn{briefly explain why, which expressions in the from the code cause this}. But when the counter example becomes more complicated, it would be hard to manually identify the cause of the problem\tvn{Why do I want to know this?}. Alloy provide a way to automatically generate such an instance\tvn{what instance ?  Did you miss something here? Did you want to talk about correct instances?}.  We change the assert to pred { no FSM.stop.transition } and run Alloy. 

% However, this time Alloy couldn't generate any sat instance, indicating an overconstraint bug in the specification preventing any instance having such a property\tvn{what's overconstraint bug? why mention it here? How is that no sat indicates for a pred indicate a ``bug'' ?}. To locate the error, one common method is to check the UNSAT core, highlighted yellow in Listing ~\ref{fig:ex}. In this example, the UNSAT core contains 6 formulas. Assume the property expressed in the definition for sigs are correct, there are still 4 formulas in the UNSAT core. It is still not easy to identify which one or ones cause this overconstraint problem. 

% To better locate the bug, we remove all UNSAT cores(other than sig declaration), then re-run predicate on this sliced model as shown in ~\ref{model2}, from which we get an instance shown as ~\ref{fig:expected2}\tvn{Is it Fig 2b or 3b?} due to the randomness of Alloy search, this instance is very different from the counter example. But it has the expected property that no outgoing transition from stop state and we know that this instance is definitely inconsistent with the unsat cores. So we evaluate all these 4 expressions in unsat core in the context of this instance. 

% For example, $all start1, start2 : FSM.start | start1 = start2$ would be instantiated to $ all start1, start2 : {state0} | start1 = start2 $; $ some FSM.stop $ to $some {state1}$; $ FSM.start !in FSM.stop$ to $state0 != state1$ and $all s: State | s.transition !in FSM.start$ to $ {state0, stat1, state2} !in {state0}$. Among these 4 formulas, the 4th one is evaluated to false and is the constraint preventing the presence of expected instance. We locate the overconstraint bug to this sentence.\tvn{How do we know this is correct? What if there are multiple sentences that are false?}

% \tvn{Not sure if this is the story we want to tell.  Why do we require the developer to fix this to continue?}
% The developer then use this information and fix this bug by changing the bug line to $all s: State | FSM.start !in s.transition$\tvn{why change to this?}. Rerun the check command, Alloy still gives the same cexs ~\ref{fig:counter1}, but this time Alloy also provides the expected instance ~\ref{fig:expected2}. Due to the randomness of Alloy search, these two instances are very different from each other. Comparing between these two couldn't lead to a clear understanding of why the cex presents.  

% To get a better understanding, we would like to generate an expected instance as similar as the cex, so that the difference between these two removes all unnecessary information about the bug. Thus, we generate multiple cex and expected instance pairs, as shown in Fig ~\ref{fig:pair1} and Fig ~\ref{fig:pair2}. 

% We then extract the differences between counter example and expected instance. For Fig ~\ref{fig:pair1}, the difference is $transition: State1->State2$, for Fig~\ref{fig:pair2}, the difference is $transition: State1->State1$. 

% Then we try to find the most 'specified' name for each atom. Here most 'specified' name is the relation name, either sig name or field name or the combination of them, that when evaluate that name in an instance, the value will always be the same atom. For example, in the both examples, evaluating $FSM.start$ will always gives $State0$, and $FSM.stop$ $State1$, thus we could use $FSM.start$ to represent $State0$ and $FSM.stop$ $State1$. To find out such an name, we would search all relations in an instance and check if the number of values in that relation is 1 and if atom appears in the right-most location along the arrow. In second example, there will be two 'specified' names for $State1$, $FSM.stop$ and $State.transition$. However, if we look at the other instances pairs generated in the first example, $State.transition$ is evaluated to ${State1, State2}$, and thus is not the most specified name for $State1$. Considering all instance pairs, the most 'specified' name for $State1$ is $FSM.stop$. If such an name couldn't be found, we would use the most specified sig name for that atom, for example, $State2$ in the first example. After finding such name, difference becomes $transition:FSM.stop -> State$ for the first pair and $transition:FSM.stop -> FSM.stop$ for the second pair. 

% We slice the Alloy model to find sentences that contains the relation transition and FSM.stop. This leads our search to $all s : State | FSM.stop !in s.*transition$ and $all s:State | s.transition = none => s in FSM.stop$. Then we evaluate all expressions in these two sentences and check their distance to the difference. The instantiated value for each expression are from the skolemized variables provided by Alloy, if no skolem variable provided, we use the set of atoms that involved in the difference between these two. In this example, no skolem vairable provided, so we pick State1 and State2 for pair one and State1 for pair 2. The intuition is to evaluate the expression and check how close their returns values to the different relations. The atomic expressions are FSM.stop, s.*transition and s.transition. In pair1, FSM.stop = {State1}, State1.*transition = {State2, State1},  State2.*transition = {State2, State1}, State2.transition = {state1}, State1.transition = {State2} s.transition = {state1}. 


% However, the differences between these two still provides some insight of the bug. First thing we learn from the difference is that the bug has to contains the relation transition. However, there are still 4 sentences has relation transition. Modifying any of these will potentially change the value for transition. To further narrow down the range, we apply the following heuristics. (1) Extract the difference between counterexample and expected instance, in this example, it is $State0 -> State0$; (2) try to find the most 'specified' name for each atom. Here most 'specified' name is the relation name, either sig name or field name or the combination of them, that when evaluate that name in an instance, the value will always be the same atom. For example, in this example, evaluating $FSM.start$ will always gives $State0$, and $FSM.stop$ $State1$. To find out such an name, we would search all relations in an instance and check if the number of values in that relation is 1 and if atom appears in the right-most location along the arrow. In this example, there will be two 'specified' names for $State0$, $FSM.stop$ and $State.transition$. However, if we look at the other instances pairs generated, $State.transition$ is removed. Considering all instance pairs, the most 'specified' name for $State0$ is $FSM.stop$. The difference becomes $FSM.stop -> FSM.stop$ in relation 'transition'. From which we get another keywords FSM.stop. This further reduce the range to two: $ all s: State | s.transition = none => s in FSM.stop$ and $ all s: State | FSM.stop in s.*transition$. (3) To further narrow down the range between these two sentences, we apply the following steps:
% \begin{itemize}
%     \item Remove the suspicious sentences from original specification, get the sliced model shown in Listing~\ref{fig:maxmodel1}
%     \item Then maximize the counterexample, which generates an instances MaxIns with suspicious constraints removed. 
%     \item Fore each suspicious sentences S, do the following:
%         \begin{itemize}
%             \item Add two pred S and not S back to specification, for example, add the following two pred for $ all s : State | FSM.stop in s.*transition $ : pred1 $ run { not (all s : State | FSM.stop in s.*transition) }$ and pred2 $ run { all s : State | FSM.stop in s.*transition} $;
%             \item Run the sliced Alloy model with the two new pred and generate closest instances to MaxIns. pred1 generates an instance INS1 as shown in ~\ref{fig:maxpred1} and pred2 generates INS2 ~\ref{fig:maxmodel1}(the same as MaxIns);
%             \item Compare INS1 with INS2 and check the difference, calculate the possibility based on this difference. For example, in this example, the difference is $transition: State0 -> State2$. The possibility is calculated by the number of common difference: number of common difference / total number of difference. In this one the possibility is 0/1 = 0
%             %to find an instance NewIns that is closest to MaxIns, the heuristic is that if S is related to bug, then the difference between NewIns and MaxIns would contain the difference between countereeample and expected instance;
%         \end{itemize}
%         \begin{itemize}
%             \item Similarly, for $ all s: State | s.transition = none => s in FSM.stop$, we generate the model in Figure ~\ref{fig:maxpred2} and the difference is $transition: State2->State0$ and $State0->State0$. The possibility is 1/2 = 0.5
%         \end{itemize}
% \end{itemize}

% \end{comment}
%(2) For each sentences calculate its possibility using the following methods:
%   1. Add it back to the sliced model;
%   2. Generates an instance S that is closest to max;
%   3. If the difference doesn't include any of the 'first' difference, then this sentence has a low chance to relate to bug;
   
   
%   A more complicated way: Generate instance S1 that is closest to counter, S2 closest to expected. Compare the difference between S1 and S2, the more similar this difference is closest to the difference of original c/e pair, the more likely this sentence is contributed to bug.

%Then we use the differences and go back to these two expressions to find out which one is more like to be related to the bug. If we apply a minimum change steps to the difference would be: $State2->State0$ is added and $State0->State1$ is deleted. Which relations has been changed and which hasn't. We would then evaluate all atomic expressions. For boolean expression, if the value changed, from true to false or vice versa, then this expression has the most high possibility to the bug. For formulas, we evaluate it and find out the set of values it returns, we define the possibility of an expression by the number of different values. Instead of all values, we use the value of the difference. 

%Then we evaluate the expression against these difference, the difference between these two is that $s.transition = none$ is evaluated to true for expected example while false for counterexample, so we locate the bug to this location. 







==> pldi21/relatedwork.tex <==
\vspace{0.1cm}
\section{Related Work}
\label{sec:related}
\vspace{0.1cm}

{\tool} is closely related to AlloyFL~\cite{alloyfl}, which 
adopts spectrum-based fault localization~\cite{spfl1, spfl2, spfl3} and mutation-based techniques~\cite{mut1, mut2} from imperative languages.
Given a set of AUnit tests~\cite{aunit} labeled with should-pass or should-fail, AlloyFL computes a suspicious score for expression by mutating and giving it a higher score if the mutation increases the number of should-pass tests pass and the number of should-fail tests fail.
%While AlloyFL shows an accurate localization result, it relies on having quality test cases.
AlloyFL uses MuAlloy~\cite{mualloy} to automatically generate tests.
However, MuAlloy requires the correct Alloy model to generate these tests.
{\tool} does not require tests and instead uses assertions, which are commonly used in Alloy.

The Amalgam project~\cite{whyandwhynot} explains why some tuples of a relation do or do not appear in certain instances.
In Amalgam, the user manually selects a tuple to add or delete, and when trying to explain why or why not literal presents in counterexample or instance, the provenances are assertion or predicate inserted.
{\tool} adopts Amalgam to automatically identify why a counterexample fails and find locations that relate to this violation. 

% The core of {\tool} is generating pairs of closest instances and utilizing their differences to locate errors. The closest instance generation belongs to the area of model finding. Many studies have been conducted to optimize Alloy's random model finding. Kodkod~\cite{kodkod} uses symmetry-breaking to eliminate isomorphic instances to speed up Alloy's model finding. Platinum~\cite{platinum} improves Alloy's performance on finding new models by reusing previous solutions. Pardinus~\cite{pardinus} extends Kodkod with the ability of target-oriented model finding. Aluminum~\cite{aluminum} extends Alloy to present minimal instances and provides users the ability to guide instances exploration by adding to an existing instance. 

Many fault localization techniques have been developed for imperative languages.
Spectrum-based technique~\cite{spfl1,spfl2,spfl3,spfl4,spfl5,tarantula,spfl6,spfl7} identify faulty statements by comparing passing and failing test executions.
SAT-based techniques~\cite{sat1, sat2} convert the fault location problem into an SAT problem.
Statistic-based methods~\cite{stat1, stat2} collect statistical information from test executions to locate errors. Feedback-based techniques~\cite{feed1, feed2} interactively locates error by getting feedback from the user.
Delta debugging~\cite{delta1, delta2} identifies code changes responsible for test failure.
There are also works on minimizing differences in inputs based on the assumption that similar inputs would lead to similar runs~\cite{diff1, diff2, diff3}.
Program slicing~\cite{slice1, slice2, slice3} has also been used to aid debugging.

% Many works in imperative programs also locate bug by minimizing differences in inputs~\cite{diff1, diff2, diff3}. \cite{diff4} further improves this by expanding the similarity of input to the similarity of executions. Another similar idea is delta debugging~\cite{delta1, delta2}, which also utilizes differences. However, delta debugging is used in regression, and the deltas are referred to as source code changes. Given a set of test cases and a list of changes of a program, delta debugging locates the causes of test failure to one or a combination of changes.

Model-based diagnosis (MBD) approaches identify faulty components of a system based on abnormal behaviors.
%The main difference is that in MDB, the behaviors of each components are modeled while there is no components or behavior given in Alloy.
Griesmayer~\cite{mdb3} applied MBD to localizing fault in imperative programs using model checker. Marques-Silva~\cite{mdb2} converted the MBD problem into a MAXSAT problem to find the minimal diagnosis, where the system description is encoded as the hard clauses and the not abnormal predicates as the soft clauses.
There has also been another similar line work in pinpointing axioms in description logic~\cite{axoimpinpoint, dl}.
%\paragraph{Model-based Diagnosis}
%Similar technique has been developed in the Artificial Intellegence community, called model-based diagnosis(MDB)~\cite{mdb1}. Given a set of components and system description, MDB .
% Description logic~\cite{descriptionlogic} is also a modelling language. 

%computing all the minimal subsets of a given knowledge base that havea given consequence.


==> pldi21/result_table.tex <==
\begin{table*}[]
  \centering
  \caption{Results for models collected from AlloyFL~\cite{alloyfl}.}
  \label{table:res}
  \begin{tabular}{c|ccccc|cc|cc||c|ccccc|cc|cc}
  \hline
  model    & loc & \#rel & \#val & sliced & total & flack & time & afl & time  & model    & loc & \#rel & \#val & sliced & total & flack & time & afl & time  \\ \hline
  addr     & 21  & 1      & 3      & 10     & 74    & 1     & 0.6  & 1   & 9.2   & dll16    & 36  & 1      & 3      & 68     & 82    & 1     & 0.1  & 1   & 7.4   \\
  arr3     & 24  & 1      & 3      & 9      & 48    & 1     & 0.1  & 1   & 6.1   & dll17\_1 & 36  & 1      & 3      & 63     & 77    & 1     & 0.1  & 1   & 7.3   \\
  arr4     & 24  & 0      & 0      & 61     & 64    & 1     & 0.2  & 1   & 8.7   & dll17\_2 & 36  & 2      & 1      & 57     & 82    & 2     & 0.0  & 1   & 7.8   \\
  arr5     & 24  & 0      & 0      & 59     & 62    & 1     & 0.2  & 1   & 5.8   & dll18    & 36  & 3      & 2      & 84     & 102   & 1     & 0.0  & 3   & 14.2  \\
  arr6     & 25  & 1      & 3      & 30     & 56    & 1     & 0.3  & 2   & 4.4   & dll18\_1 & 36  & 2      & 3      & 67     & 101   & 1     & 0.1  & 3   & 103.8 \\
  arr7     & 25  & 0      & 0      & 50     & 63    & 1     & 0.1  & 1   & 6.9   & dll18\_2 & 36  & 1      & 3      & 71     & 107   & 3     & 0.6  & 1   & 44.2  \\
  arr7\_1  & 24  & 2      & 9      & 9      & 46    & 2     & 0.9  & 1   & 5.7   & dll18\_3 & 36  & 2      & 1      & 78     & 103   & 2     & 0.0  & 1   & 29.5  \\
  arr8     & 25  & 2      & 6      & 15     & 80    & 4     & 0.5  & 1   & 8.8   & dll19    & 36  & 1      & 3      & 63     & 83    & 2     & 0.1  & 1   & 7.7   \\
  arr9     & 27  & 1      & 3      & 43     & 83    & 2     & 0.2  & 2   & 8     & dll20    & 36  & 4      & 4      & 64     & 90    & 1     & 0.0  & 4   & 8.3   \\
  arr11    & 24  & 2      & 3      & 41     & 83    & 5     & 0.1  & 1   & 7     & dll20\_1 & 36  & 1      & 3      & 68     & 88    & 2     & 0.1  & 1   & 8.3   \\
  bst2     & 56  & 3      & 2      & 56     & 134   & 1     & 0.4  & 12  & 68.3  & dll20\_2 & 36  & 2      & 1      & 47     & 88    & 2     & 0.0  & 1   & 7.6   \\
  bst2\_1  & 56  & 1      & 3      & 95     & 134   & 1     & 0.3  & 13  & 68.5  & fsm1\_1  & 30  & 2      & 1      & 19     & 90    & 1     & 0.0  & 1   & 2.9   \\
  bst2\_2  & 47  & 7      & 5      & 92     & 147   & 4     & 0.1  & 2   & 95.2  & fsm2     & 29  & 2      & 1      & 14     & 70    & 4     & 0.0  & 1   & 2.8   \\
  bst2\_3  & 52  & 5      & 3      & 68     & 133   & 2     & 0.1  & 2   & 68.1  & fsm4     & 31  & 2      & 3      & 39     & 141   & 3     & 0.0  & 3   & 4.7   \\
  bst3     & 57  & 1      & 3      & 97     & 137   & 4     & 0.1  & 8   & 70    & fsm5\_2  & 29  & 2      & 2      & 17     & 69    & 3     & 0.0  & 9   & 2.1   \\
  bst3\_1  & 57  & 3      & 2      & 58     & 137   & 6     & 0.2  & 7   & 71.2  & fsm6     & 29  & 2      & 2      & 17     & 98    & 2     & 0.0  & 16  & 3     \\
  bst3\_2  & 55  & 5      & 3      & 68     & 141   & 1     & 0.2  & 1   & 68.6  & fsm7     & 29  & 2      & 2      & 14     & 64    & 6     & 0.1  & 13  & 2.6   \\
  bst4     & 46  & 5      & 3      & 95     & 145   & -     & 0.1  & 4   & 70.4  & fsm7\_1  & 29  & 2      & 2      & 14     & 59    & 1     & 0.0  & 9   & 2.6   \\
  bst4\_2  & 51  & 7      & 5      & 61     & 154   & 11    & 0.3  & 1   & 84.8  & fsm8     & 29  & 3      & 1      & 14     & 71    & 4     & 0.1  & 14  & 2.7   \\
  bst6     & 51  & 7      & 5      & 61     & 140   & 8     & 0.2  & 1   & 69.4  & fsm9\_1  & 29  & 2      & 1      & 18     & 91    & 5     & 0.1  & 1   & 3.1   \\
  bst8     & 59  & 3      & 2      & 57     & 134   & 3     & 0.3  & 8   & 62.8  & fsm9\_2  & 29  & 2      & 2      & 18     & 90    & 2     & 0.1  & 1   & 2.9   \\
  bst8\_1  & 59  & 3      & 2      & 57     & 134   & 3     & 0.2  & 8   & 62.7  & fsm9\_4  & 30  & 0      & 0      & 78     & 91    & 1     & 0.1  & 1   & 1.5   \\
  bst10\_3 & 55  & 7      & 5      & 75     & 162   & 5     & 0.3  & 4   & 91.7  & grade    & 33  & 2      & 3      & 7      & 22    & 1     & 0.0  & 1   & 4.1   \\
  bst11    & 54  & 5      & 3      & 135    & 196   & -     & 0.2  & 31  & 77    & other    & 34  & 1      & 2      & 19     & 26    & -     & 0.0  & 11  & 1.4   \\
  bst12    & 47  & 5      & 3      & 94     & 146   & 2     & 0.2  & -   & 0.6   & ssl1     & 40  & 2      & 2      & 126    & 168   & 1     & 0.1  & 3   & 25.7  \\
  bst12\_1 & 56  & 5      & 3      & 68     & 164   & 8     & 0.2  & 6   & 62.9  & ssl2     & 40  & 1      & 2      & 122    & 150   & 1     & 0.1  & 3   & 26.5  \\
  bst16    & 64  & 7      & 5      & 79     & 181   & 12    & 0.3  & 3   & 76.9  & ssl2\_1  & 44  & 2      & 2      & 72     & 156   & 3     & 0.1  & 2   & 46.9  \\
  bst17    & 48  & 5      & 3      & 113    & 186   & 12    & 0.2  & 1   & 113.7 & ssl3     & 45  & 1      & 1      & 135    & 188   & 1     & 0.0  & 1   & 81.1  \\
  bst17\_2 & 55  & 7      & 5      & 79     & 177   & 9     & 0.2  & 1   & 83.9  & ssl3\_1  & 44  & 3      & 2      & 121    & 184   & 1     & 0.2  & 1   & 65.4  \\
  bst18    & 51  & 3      & 2      & 115    & 187   & 2     & 1.4  & -   & 0.7   & ssl4     & 40  & 1      & 2      & 118    & 146   & 1     & 0.1  & 3   & 25.8  \\
  bst19    & 47  & 5      & 3      & 112    & 158   & 2     & 0.1  & 1   & 93.6  & ssl5     & 42  & 1      & 2      & 160    & 188   & 1     & 0.6  & 3   & 26.5  \\
  bst19\_1 & 52  & 6      & 3      & 112    & 175   & 2     & 0.1  & 10  & 88.7  & ssl6     & 42  & 0      & 0      & 148    & 157   & 1     & 0.7  & 1   & 30.2  \\
  bst19\_2 & 55  & 5      & 3      & 86     & 154   & 8     & 0.2  & 2   & 50.1  & ssl6\_1  & 42  & 0      & 0      & 148    & 157   & 1     & 0.5  & 1   & 31.7  \\
  bst20\_1 & 55  & 7      & 5      & 61     & 152   & 6     & 0.2  & 2   & 83.3  & ssl6\_2  & 41  & 2      & 1      & 119    & 152   & 1     & 0.1  & 1   & 29.1  \\
  bst22\_1 & 49  & 3      & 2      & 124    & 199   & 3     & 0.1  & 12  & 47.1  & ssl6\_3  & 42  & 2      & 1      & 107    & 152   & 1     & 0.1  & 3   & 31.2  \\
  bst22\_2 & 54  & 6      & 3      & 118    & 209   & 10    & 0.1  & 1   & 98    & ssl7     & 41  & 2      & 1      & 95     & 136   & 1     & 0.1  & 1   & 58.7  \\
  bst22\_3 & 57  & 5      & 5      & 74     & 199   & 16    & 0.5  & 4   & 75.7  & ssl7\_1  & 40  & 1      & 1      & 110    & 135   & 1     & 0.1  & 1   & 34.1  \\
  bempl    & 51  & 1      & 2      & 7      & 14    & -     & 0.0  & -   & 1.9   & ssl8     & 43  & 1      & 1      & 119    & 166   & 1     & 0.1  & 1   & 35    \\
  cd1      & 27  & 1      & 1      & 33     & 44    & 1     & 0.0  & 2   & 0.8   & ssl9     & 44  & 2      & 2      & 72     & 153   & 13    & 0.1  & 1   & 47.4  \\
  cd1\_1   & 27  & 1      & 2      & 31     & 44    & 1     & 0.0  & 1   & 1.8   & ssl10    & 43  & 2      & 1      & 110    & 155   & 1     & 0.1  & 3   & 31.2  \\
  cd2      & 27  & 1      & 1      & 25     & 35    & 1     & 0.0  & 1   & 0.5   & ssl11    & 42  & 2      & 1      & 127    & 177   & 2     & 0.1  & 4   & 33.5  \\
  cd3      & 26  & 1      & 1      & 32     & 43    & 1     & 0.0  & 2   & 0.7   & ssl12    & 40  & 2      & 2      & 114    & 157   & 1     & 0.1  & 3   & 70.2  \\
  cd3\_1   & 26  & 1      & 1      & 31     & 46    & 1     & 0.0  & 4   & 1     & ssl12\_1 & 44  & 3      & 3      & 78     & 161   & 12    & 0.4  & 1   & 53.5  \\
  ctree    & 30  & 1      & 1      & 5      & 49    & -     & 0.0  & -   & 4.2   & ssl13    & 43  & 1      & 1      & 123    & 174   & 3     & 0.1  & 1   & 67.8  \\
  dll1     & 37  & 1      & 3      & 63     & 77    & 1     & 0.1  & 1   & 7.3   & ssl14    & 44  & 0      & 0      & 149    & 158   & 1     & 0.5  & 1   & 31.3  \\
  dll1\_1  & 38  & 2      & 1      & 57     & 86    & 3     & 0.1  & -   & 0.2   & ssl14\_1 & 44  & 0      & 0      & 149    & 158   & 1     & 0.5  & 1   & 32    \\
  dll2     & 42  & 1      & 3      & 63     & 77    & 1     & 0.1  & 1   & 7.3   & ssl14\_2 & 43  & 2      & 1      & 120    & 153   & 1     & 0.0  & 1   & 30.6  \\
  dll2\_1  & 42  & 2      & 1      & 57     & 82    & 2     & 0.0  & 1   & 7.8   & ssl14\_3 & 44  & 2      & 2      & 108    & 153   & 1     & 0.1  & 3   & 31.6  \\
  dll3     & 37  & 5      & 4      & 59     & 80    & 1     & 0.0  & 1   & 7.4   & ssl15    & 41  & 2      & 1      & 106    & 161   & 5     & 0.1  & 3   & 35.5  \\
  dll3\_1  & 37  & 2      & 1      & 49     & 75    & 1     & 0.1  & 3   & 14.9  & ssl16    & 39  & 2      & 2      & 119    & 137   & -     & 0.0  & 1   & 53.1  \\
  dll3\_2  & 36  & 2      & 1      & 67     & 75    & -     & 0.0  & 1   & 13.2  & ssl16\_1 & 39  & 2      & 2      & 115    & 133   & -     & 0.0  & 1   & 16.3  \\
  dll4     & 37  & 1      & 3      & 67     & 81    & 1     & 0.1  & 1   & 8.3   & ssl16\_2 & 47  & 2      & 4      & 74     & 136   & -     & 0.3  & 1   & 16.9  \\
  dll5\_1  & 39  & 1      & 3      & 80     & 102   & 1     & 0.1  & 1   & 9.2   & ssl16\_3 & 43  & 2      & 2      & 71     & 133   & -     & 0.2  & 1   & 40.6  \\
  dll6     & 36  & 1      & 3      & 94     & 113   & 1     & 0.1  & 3   & 9.3   & ssl17    & 41  & 2      & 1      & 119    & 151   & 1     & 0.0  & 1   & 29.5  \\
  dll7\_1  & 36  & 1      & 3      & 59     & 73    & 1     & 0.1  & 1   & 7.1   & ssl17\_1 & 42  & 2      & 1      & 106    & 151   & 1     & 0.1  & 3   & 32.2  \\
  dll8     & 36  & 1      & 3      & 76     & 96    & 1     & 0.1  & 3   & 9.8   & ssl18    & 40  & 1      & 2      & 131    & 162   & 3     & 0.0  & -   & 0.4   \\
  dll9     & 38  & 2      & 1      & 91     & 100   & 1     & 0.1  & 2   & 10.8  & ssl18\_1 & 40  & 2      & 2      & 118    & 160   & 1     & 0.1  & 3   & 30.9  \\
  dll11    & 36  & 1      & 3      & 68     & 87    & 1     & 0.1  & 3   & 8.9   & ssl18\_2 & 49  & 1      & 3      & 85     & 160   & 1     & 0.3  & 2   & 54.9  \\
  dll12    & 36  & 1      & 3      & 63     & 77    & 1     & 0.1  & 1   & 7.3   & ssl19    & 40  & 1      & 2      & 141    & 169   & 1     & 0.1  & 3   & 29.1  \\
  dll13    & 36  & 2      & 3      & 51     & 60    & 1     & 0.0  & 1   & 11.6  & ssl19\_1 & 50  & 2      & 3      & 106    & 175   & 7     & 0.6  & 1   & 28    \\
  dll14\_1 & 37  & 1      & 3      & 71     & 85    & 1     & 0.1  & 1   & 7.3   & ssl19\_2 & 44  & 1      & 3      & 81     & 174   & 8     & 0.3  & -   & 0.5   \\
  dll15    & 40  & 1      & 3      & 107    & 126   & 1     & 0.1  & 3   & 13.6  &          &     &        &        &        &       &       &      &     &      \\
  \hline
  \end{tabular}
  \end{table*}

==> result_table.tex <==
\begin{table*}[]
  \centering
  \caption{Results for models collected from AlloyFL~\cite{alloyfl}.}
  \label{table:res}
  \begin{tabular}{c|ccccc|cc|cc||c|ccccc|cc|cc}
  \hline
  model    & loc & \#rel & \#val & sliced & total & flack & time & afl & time  & model    & loc & \#rel & \#val & sliced & total & flack & time & afl & time  \\ \hline
  addr     & 21  & 1      & 3      & 10     & 74    & 1     & 0.6  & 1   & 9.2   & dll16    & 36  & 1      & 3      & 68     & 82    & 1     & 0.1  & 1   & 7.4   \\
  arr3     & 24  & 1      & 3      & 9      & 48    & 1     & 0.1  & 1   & 6.1   & dll17\_1 & 36  & 1      & 3      & 63     & 77    & 1     & 0.1  & 1   & 7.3   \\
  arr4     & 24  & 0      & 0      & 61     & 64    & 1     & 0.2  & 1   & 8.7   & dll17\_2 & 36  & 2      & 1      & 57     & 82    & 2     & 0.0  & 1   & 7.8   \\
  arr5     & 24  & 0      & 0      & 59     & 62    & 1     & 0.2  & 1   & 5.8   & dll18    & 36  & 3      & 2      & 84     & 102   & 1     & 0.0  & 3   & 14.2  \\
  arr6     & 25  & 1      & 3      & 30     & 56    & 1     & 0.3  & 2   & 4.4   & dll18\_1 & 36  & 2      & 3      & 67     & 101   & 1     & 0.1  & 3   & 103.8 \\
  arr7     & 25  & 0      & 0      & 50     & 63    & 1     & 0.1  & 1   & 6.9   & dll18\_2 & 36  & 1      & 3      & 71     & 107   & 3     & 0.6  & 1   & 44.2  \\
  arr7\_1  & 24  & 2      & 9      & 9      & 46    & 2     & 0.9  & 1   & 5.7   & dll18\_3 & 36  & 2      & 1      & 78     & 103   & 2     & 0.0  & 1   & 29.5  \\
  arr8     & 25  & 2      & 6      & 15     & 80    & 4     & 0.5  & 1   & 8.8   & dll19    & 36  & 1      & 3      & 63     & 83    & 2     & 0.1  & 1   & 7.7   \\
  arr9     & 27  & 1      & 3      & 43     & 83    & 2     & 0.2  & 2   & 8     & dll20    & 36  & 4      & 4      & 64     & 90    & 1     & 0.0  & 4   & 8.3   \\
  arr11    & 24  & 2      & 3      & 41     & 83    & 5     & 0.1  & 1   & 7     & dll20\_1 & 36  & 1      & 3      & 68     & 88    & 2     & 0.1  & 1   & 8.3   \\
  bst2     & 56  & 3      & 2      & 56     & 134   & 1     & 0.4  & 12  & 68.3  & dll20\_2 & 36  & 2      & 1      & 47     & 88    & 2     & 0.0  & 1   & 7.6   \\
  bst2\_1  & 56  & 1      & 3      & 95     & 134   & 1     & 0.3  & 13  & 68.5  & fsm1\_1  & 30  & 2      & 1      & 19     & 90    & 1     & 0.0  & 1   & 2.9   \\
  bst2\_2  & 47  & 7      & 5      & 92     & 147   & 4     & 0.1  & 2   & 95.2  & fsm2     & 29  & 2      & 1      & 14     & 70    & 4     & 0.0  & 1   & 2.8   \\
  bst2\_3  & 52  & 5      & 3      & 68     & 133   & 2     & 0.1  & 2   & 68.1  & fsm4     & 31  & 2      & 3      & 39     & 141   & 3     & 0.0  & 3   & 4.7   \\
  bst3     & 57  & 1      & 3      & 97     & 137   & 4     & 0.1  & 8   & 70    & fsm5\_2  & 29  & 2      & 2      & 17     & 69    & 3     & 0.0  & 9   & 2.1   \\
  bst3\_1  & 57  & 3      & 2      & 58     & 137   & 6     & 0.2  & 7   & 71.2  & fsm6     & 29  & 2      & 2      & 17     & 98    & 2     & 0.0  & 16  & 3     \\
  bst3\_2  & 55  & 5      & 3      & 68     & 141   & 1     & 0.2  & 1   & 68.6  & fsm7     & 29  & 2      & 2      & 14     & 64    & 6     & 0.1  & 13  & 2.6   \\
  bst4     & 46  & 5      & 3      & 95     & 145   & -     & 0.1  & 4   & 70.4  & fsm7\_1  & 29  & 2      & 2      & 14     & 59    & 1     & 0.0  & 9   & 2.6   \\
  bst4\_2  & 51  & 7      & 5      & 61     & 154   & 11    & 0.3  & 1   & 84.8  & fsm8     & 29  & 3      & 1      & 14     & 71    & 4     & 0.1  & 14  & 2.7   \\
  bst6     & 51  & 7      & 5      & 61     & 140   & 8     & 0.2  & 1   & 69.4  & fsm9\_1  & 29  & 2      & 1      & 18     & 91    & 5     & 0.1  & 1   & 3.1   \\
  bst8     & 59  & 3      & 2      & 57     & 134   & 3     & 0.3  & 8   & 62.8  & fsm9\_2  & 29  & 2      & 2      & 18     & 90    & 2     & 0.1  & 1   & 2.9   \\
  bst8\_1  & 59  & 3      & 2      & 57     & 134   & 3     & 0.2  & 8   & 62.7  & fsm9\_4  & 30  & 0      & 0      & 78     & 91    & 1     & 0.1  & 1   & 1.5   \\
  bst10\_3 & 55  & 7      & 5      & 75     & 162   & 5     & 0.3  & 4   & 91.7  & grade    & 33  & 2      & 3      & 7      & 22    & 1     & 0.0  & 1   & 4.1   \\
  bst11    & 54  & 5      & 3      & 135    & 196   & -     & 0.2  & 31  & 77    & other    & 34  & 1      & 2      & 19     & 26    & -     & 0.0  & 11  & 1.4   \\
  bst12    & 47  & 5      & 3      & 94     & 146   & 2     & 0.2  & -   & 0.6   & ssl1     & 40  & 2      & 2      & 126    & 168   & 1     & 0.1  & 3   & 25.7  \\
  bst12\_1 & 56  & 5      & 3      & 68     & 164   & 8     & 0.2  & 6   & 62.9  & ssl2     & 40  & 1      & 2      & 122    & 150   & 1     & 0.1  & 3   & 26.5  \\
  bst16    & 64  & 7      & 5      & 79     & 181   & 12    & 0.3  & 3   & 76.9  & ssl2\_1  & 44  & 2      & 2      & 72     & 156   & 3     & 0.1  & 2   & 46.9  \\
  bst17    & 48  & 5      & 3      & 113    & 186   & 12    & 0.2  & 1   & 113.7 & ssl3     & 45  & 1      & 1      & 135    & 188   & 1     & 0.0  & 1   & 81.1  \\
  bst17\_2 & 55  & 7      & 5      & 79     & 177   & 9     & 0.2  & 1   & 83.9  & ssl3\_1  & 44  & 3      & 2      & 121    & 184   & 1     & 0.2  & 1   & 65.4  \\
  bst18    & 51  & 3      & 2      & 115    & 187   & 2     & 1.4  & -   & 0.7   & ssl4     & 40  & 1      & 2      & 118    & 146   & 1     & 0.1  & 3   & 25.8  \\
  bst19    & 47  & 5      & 3      & 112    & 158   & 2     & 0.1  & 1   & 93.6  & ssl5     & 42  & 1      & 2      & 160    & 188   & 1     & 0.6  & 3   & 26.5  \\
  bst19\_1 & 52  & 6      & 3      & 112    & 175   & 2     & 0.1  & 10  & 88.7  & ssl6     & 42  & 0      & 0      & 148    & 157   & 1     & 0.7  & 1   & 30.2  \\
  bst19\_2 & 55  & 5      & 3      & 86     & 154   & 8     & 0.2  & 2   & 50.1  & ssl6\_1  & 42  & 0      & 0      & 148    & 157   & 1     & 0.5  & 1   & 31.7  \\
  bst20\_1 & 55  & 7      & 5      & 61     & 152   & 6     & 0.2  & 2   & 83.3  & ssl6\_2  & 41  & 2      & 1      & 119    & 152   & 1     & 0.1  & 1   & 29.1  \\
  bst22\_1 & 49  & 3      & 2      & 124    & 199   & 3     & 0.1  & 12  & 47.1  & ssl6\_3  & 42  & 2      & 1      & 107    & 152   & 1     & 0.1  & 3   & 31.2  \\
  bst22\_2 & 54  & 6      & 3      & 118    & 209   & 10    & 0.1  & 1   & 98    & ssl7     & 41  & 2      & 1      & 95     & 136   & 1     & 0.1  & 1   & 58.7  \\
  bst22\_3 & 57  & 5      & 5      & 74     & 199   & 16    & 0.5  & 4   & 75.7  & ssl7\_1  & 40  & 1      & 1      & 110    & 135   & 1     & 0.1  & 1   & 34.1  \\
  bempl    & 51  & 1      & 2      & 7      & 14    & -     & 0.0  & -   & 1.9   & ssl8     & 43  & 1      & 1      & 119    & 166   & 1     & 0.1  & 1   & 35    \\
  cd1      & 27  & 1      & 1      & 33     & 44    & 1     & 0.0  & 2   & 0.8   & ssl9     & 44  & 2      & 2      & 72     & 153   & 13    & 0.1  & 1   & 47.4  \\
  cd1\_1   & 27  & 1      & 2      & 31     & 44    & 1     & 0.0  & 1   & 1.8   & ssl10    & 43  & 2      & 1      & 110    & 155   & 1     & 0.1  & 3   & 31.2  \\
  cd2      & 27  & 1      & 1      & 25     & 35    & 1     & 0.0  & 1   & 0.5   & ssl11    & 42  & 2      & 1      & 127    & 177   & 2     & 0.1  & 4   & 33.5  \\
  cd3      & 26  & 1      & 1      & 32     & 43    & 1     & 0.0  & 2   & 0.7   & ssl12    & 40  & 2      & 2      & 114    & 157   & 1     & 0.1  & 3   & 70.2  \\
  cd3\_1   & 26  & 1      & 1      & 31     & 46    & 1     & 0.0  & 4   & 1     & ssl12\_1 & 44  & 3      & 3      & 78     & 161   & 12    & 0.4  & 1   & 53.5  \\
  ctree    & 30  & 1      & 1      & 5      & 49    & -     & 0.0  & -   & 4.2   & ssl13    & 43  & 1      & 1      & 123    & 174   & 3     & 0.1  & 1   & 67.8  \\
  dll1     & 37  & 1      & 3      & 63     & 77    & 1     & 0.1  & 1   & 7.3   & ssl14    & 44  & 0      & 0      & 149    & 158   & 1     & 0.5  & 1   & 31.3  \\
  dll1\_1  & 38  & 2      & 1      & 57     & 86    & 3     & 0.1  & -   & 0.2   & ssl14\_1 & 44  & 0      & 0      & 149    & 158   & 1     & 0.5  & 1   & 32    \\
  dll2     & 42  & 1      & 3      & 63     & 77    & 1     & 0.1  & 1   & 7.3   & ssl14\_2 & 43  & 2      & 1      & 120    & 153   & 1     & 0.0  & 1   & 30.6  \\
  dll2\_1  & 42  & 2      & 1      & 57     & 82    & 2     & 0.0  & 1   & 7.8   & ssl14\_3 & 44  & 2      & 2      & 108    & 153   & 1     & 0.1  & 3   & 31.6  \\
  dll3     & 37  & 5      & 4      & 59     & 80    & 1     & 0.0  & 1   & 7.4   & ssl15    & 41  & 2      & 1      & 106    & 161   & 5     & 0.1  & 3   & 35.5  \\
  dll3\_1  & 37  & 2      & 1      & 49     & 75    & 1     & 0.1  & 3   & 14.9  & ssl16    & 39  & 2      & 2      & 119    & 137   & -     & 0.0  & 1   & 53.1  \\
  dll3\_2  & 36  & 2      & 1      & 67     & 75    & -     & 0.0  & 1   & 13.2  & ssl16\_1 & 39  & 2      & 2      & 115    & 133   & -     & 0.0  & 1   & 16.3  \\
  dll4     & 37  & 1      & 3      & 67     & 81    & 1     & 0.1  & 1   & 8.3   & ssl16\_2 & 47  & 2      & 4      & 74     & 136   & -     & 0.3  & 1   & 16.9  \\
  dll5\_1  & 39  & 1      & 3      & 80     & 102   & 1     & 0.1  & 1   & 9.2   & ssl16\_3 & 43  & 2      & 2      & 71     & 133   & -     & 0.2  & 1   & 40.6  \\
  dll6     & 36  & 1      & 3      & 94     & 113   & 1     & 0.1  & 3   & 9.3   & ssl17    & 41  & 2      & 1      & 119    & 151   & 1     & 0.0  & 1   & 29.5  \\
  dll7\_1  & 36  & 1      & 3      & 59     & 73    & 1     & 0.1  & 1   & 7.1   & ssl17\_1 & 42  & 2      & 1      & 106    & 151   & 1     & 0.1  & 3   & 32.2  \\
  dll8     & 36  & 1      & 3      & 76     & 96    & 1     & 0.1  & 3   & 9.8   & ssl18    & 40  & 1      & 2      & 131    & 162   & 3     & 0.0  & -   & 0.4   \\
  dll9     & 38  & 2      & 1      & 91     & 100   & 1     & 0.1  & 2   & 10.8  & ssl18\_1 & 40  & 2      & 2      & 118    & 160   & 1     & 0.1  & 3   & 30.9  \\
  dll11    & 36  & 1      & 3      & 68     & 87    & 1     & 0.1  & 3   & 8.9   & ssl18\_2 & 49  & 1      & 3      & 85     & 160   & 1     & 0.3  & 2   & 54.9  \\
  dll12    & 36  & 1      & 3      & 63     & 77    & 1     & 0.1  & 1   & 7.3   & ssl19    & 40  & 1      & 2      & 141    & 169   & 1     & 0.1  & 3   & 29.1  \\
  dll13    & 36  & 2      & 3      & 51     & 60    & 1     & 0.0  & 1   & 11.6  & ssl19\_1 & 50  & 2      & 3      & 106    & 175   & 7     & 0.6  & 1   & 28    \\
  dll14\_1 & 37  & 1      & 3      & 71     & 85    & 1     & 0.1  & 1   & 7.3   & ssl19\_2 & 44  & 1      & 3      & 81     & 174   & 8     & 0.3  & -   & 0.5   \\
  dll15    & 40  & 1      & 3      & 107    & 126   & 1     & 0.1  & 3   & 13.6  &          &     &        &        &        &       &       &      &     &      \\
  \hline
  \end{tabular}
  \end{table*}
